Functional Adaptor Signatures: Beyond All-or-Nothing Blockchain-based Payments

In scenarios where a seller holds sensitive data $x$, like patient records, and a buyer seeks to obtain an evaluation of a function $f$ on $x$, solutions in trustless environments like blockchain fall into two categories: (1) Smart contract-powered solutions and (2) cryptographic solutions using tools such as adaptor signatures. The former offers atomic transactions where the buyer learns $f(x)$ upon payment. However, this approach is inefficient, costly, lacks privacy for the seller's data, and is incompatible with blockchains such as bitcoin. In contrast, the adaptor signature-based approach addresses all of the above issues but comes with an "all-or-nothing" guarantee, where the buyer fully extracts $x$ and does not support extracting $f(x)$. In this work, we bridge the gap between these approaches, developing a solution that enables fair functional sales while offering all the above properties like adaptor signatures. Towards this, we propose functional adaptor signatures (FAS), a novel cryptographic primitive and show how it can be used to enable functional sales. We formalize the security properties of FAS, among which is a new notion called witness privacy to capture seller's privacy, which ensures the buyer does not learn anything beyond $f(x)$. We present multiple variants of witness privacy, namely, witness hiding, witness indistinguishability, and zero-knowledge. We introduce two efficient constructions of FAS supporting linear functions based on groups of prime-order and lattices, that satisfy the strongest notion of witness privacy. A central conceptual contribution of our work lies in revealing a surprising connection between functional encryption and adaptor signatures. We implement our FAS construction for Schnorr signatures and show that for reasonably sized seller witnesses, all operations are quite efficient even for commodity hardware.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

#TARGET=main.pdf 
TARGET=functional-adaptors.pdf 
TARGET2=fas-eprint.pdf 

all: $(TARGET)
tcc: $(TARGET2)
eprint:  $(TARGET2)
 
$(TARGET): $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<


$(TARGET2): $(TARGET2:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<) 
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<


full: $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	
quick: $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<

quick2: $(TARGET2:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<

test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) $(TARGET2) *.log *.aux *.bbl *.blg *.toc *.out *.bak .*.xtx.cache parsetab.py \#*\# *~


==> as-construction-alt.tex <==
\subsection{Construction}
Recall the hard relation 
$R_\DLstar := \{ \ (\Delta, (\delta_1, \delta_2)) \ | \ \Delta = g_1^{\delta_1} \cdot g_2^{\delta_2} \ \}$. 
Our Adpator Signature construction with respect to the 
Schnorr signature scheme $\Sch$ and the hard relation $R_\DLstar$ 
is as follows. We construct it at a different abstraction level directly from Schnorr Adaptor Signature Scheme $\AS_{Sch, \DL}$ for the hard relation $R_\DL$. This will potentially help us simplify security proofs.

\paragraph{\underline{
$\KGen(1^\secparam, G, q, g_1)$}:
} 
\begin{itemize}
\item Compute Schnorr Adaptor signature key-pair $(\sk' = \delta_1, \vk' = g_1^{\delta_1}) \gets AS_{Sch, \DL}.\KGen(1^\lambda)$.
\item Sample $a, \overline{a} \getr \Z_q$ such that $a \neq \overline{a}$, compute generators $g_2 := g_1^a, \overline{g}_2 := g_1^{\overline{a}}$, sample $\delta_2, \overline{\delta}_2 \getr \Z_q$. 
Let $\sk_1 = \delta_1 + a \delta_2$ and $\sk_2 = \delta_1 + \overline{a} \overline{\delta}_2$.
Let $\vk_1 = g_1^{\delta_1} \cdot g_2^{\delta_2}$ and $\vk_2 = g_1^{\delta_1} \cdot \overline{g}_2^{\overline{\delta}_2}$. 
Observe that $(\sk_1, \vk_1)$ and $(\sk_2, \vk_2)$ are two valid key-pairs for Schnorr Adaptor signature scheme w.r.t.\ the hard relation $R_\DL$.
\item Output $\sk = (\sk_1, \sk_2)$ and $\vk = (\vk_1, \vk_2, a, \overline{a})$.
\end{itemize}

\paragraph{\underline{
$\PreSign(\sk,m,X, \overline{X})$}:
}
\begin{itemize}
\item 
Compute $\widetilde{\sigma}_1 = AS_{Sch, \DL}.\PreSign(\sk_1, m, X)$ and 
$\widetilde{\sigma}_2 = AS_{Sch, \DL}.\PreSign(\sk_2, m, \overline{X})$, where $X = g_1^{x_1} \cdot g_2^{x_2}, \overline{X} = g_1^{x_1} \cdot \overline{g}_2^{x_2}$. 
% \nikhil{PROBLEM: How to compute $\overline{X}$ from $X$ without knowing $x_2$?}
\item 
Output pre-signature $\widetilde{\sigma} := (\widetilde{\sigma}_1, \widetilde{\sigma}_2)$.  
\end{itemize}

\paragraph{\underline{
$\PreVerify(\vk, m, X, \overline{X}, \widetilde{\sigma})$}: 
}
\begin{itemize}
\item 
Output $1$ iff 
$AS_{Sch, \DL}.\PreVerify(\vk_1, m, X, \widetilde{\sigma}_1) = 1$ 
and 
$AS_{Sch, \DL}.\PreVerify(\vk_2, m, \overline{X}, \widetilde{\sigma}_2) = 1$.
\end{itemize}

\paragraph{\underline{
$\Adapt({\color{blue}\vk}, \widetilde{\sigma}, (x_1, x_2))$}: 
}
\nikhil{do we need to modify definition to allow using $\vk$ here?}
\begin{itemize}
\item 
Parse $\vk = (\vk_1, \vk_2, a, \overline{a})$.
\item 
Suppose $X = g_1^{x_1} \cdot g_2^{x_2} = g_1^{x_1 + a \cdot x_2} = g_1^{x_1} \cdot \overline{g}_2^{}$.
\item 
Compute witnesses $w_1 = x_1 + a \cdot x_2$ and $w_2 = x_1 + \overline{a} \cdot x_2$.
\item 
Compute 
$\sigma_1 = AS_{Sch, \DL}.\Adapt(\widetilde{\sigma}_1, w_1)$ 
and 
$\sigma_2 = AS_{Sch, \DL}.\Adapt(\widetilde{\sigma}_2, w_2)$. 
\item 
Output two Schnorr signatures $\sigma_1$ and $\sigma_2$.
\end{itemize}

\paragraph{\underline{
$\Verify(\vk, m, \sigma_1, \sigma_2)$}: 
}
\begin{itemize}
\item 
Output $1$ iff $\Sch.\Verify(\vk_1, m, \sigma_1) = 1$ and 
$\Sch.\Verify(\vk_2, m, \sigma_2) = 1$.
\end{itemize}

\paragraph{\underline{
$\Ext({\color{blue}\vk}, \widetilde{\sigma}, (\sigma_1, \sigma_2), X)$}: 
}
\nikhil{do we need to modify definition to allow using $\vk$ here?}
\begin{itemize}
\item 
Parse $\widetilde{\sigma} = (\widetilde{\sigma}_1, \widetilde{\sigma}_2)$.
\item 
Recover witnesses $w_1 = AS_{Sch, \DL}.\Ext(\widetilde{\sigma}_1, \sigma_1)$ and 
$w_2 = AS_{Sch, \DL}.\Ext(\widetilde{\sigma}_2, \sigma_2)$.
\item 
Compute  $x'_1 := \frac{a w_2 - \overline{a} w_1}{a - \overline{a}}$ and $x'_2 := \frac{w_1 - w_2}{a - \overline{a}}$.
\item Output $(x'_1, x'_2)$.
\end{itemize}

==> as-construction.tex <==
\section{Adaptor Signatures w.r.t.\ $\Sch$ and hard relation $\DLstar$ }
In this section, we present a construction of adaptor signatures with respect to the Schnorr signature scheme $\Sch$ and the hard relation $\DLstar$.

First, we recall the Schnorr Signature Scheme $\Sch$.

\subsection{Schnorr Signature Scheme $\Sch$}
\paragraph{$\KGen(1^\secparam)$:}
\begin{itemize}
\item Sample a cyclic group $\G$ with generator $g_1$ and prime-order $q$ as $(\G, g_1, q) \gets \GroupGen(1^\secparam)$.
\item Sample $\delta_1 \getr \Z_q$.
\item Output $\sk = \delta_1$ and $\vk = g_1^{\delta_1}$.
\end{itemize}
\paragraph{$\Sign(\sk, m \in \{0,1\}^*)$:}
\begin{itemize}
\item Sample $r_1 \getr \Z_q$.
\item Compute $h = H(g_1^{r_1} || m)$.
\item Compute $s_1 = r_1 + h \delta_1$.
\item Output signature $\sigma = (h, s_1)$.
\end{itemize}
\paragraph{$\verify(\vk, m, \sigma)$:}
\begin{itemize}
\item Compute $g_1^{R_1} := g_1^{s_1} / (g_1^{\delta_1})^h$.
\item Output $1$ iff $h = H(g_1^{R_1} || m)$.
\end{itemize}


\ignore{
	
\subsection{Construction}
Recall the hard relation 
$R_\DLstar := \{ \ (\Delta, (\delta_1, \delta_2)) \ | \ \Delta = g_1^{\delta_1} \cdot g_2^{\delta_2} \ \}$. 
Our Adpator Signature construction with respect to the 
Schnorr signature scheme $\Sch$ and the hard relation $\DLstar$ 
is as follows.

\paragraph{\underline{
$\KGen(1^\secparam, G, q, g_1)$}:
} \nikhil{is it okay to post-process $\Sch$ keys here?}
\begin{itemize}
\item Compute Schnorr signature key-pair $(\sk' = \delta_1, \vk' = g_1^{\delta_1}) \gets \Sch.\Setup(1^\lambda)$.
\item Sample $a, \overline{a} \getr \Z_q$ such that $a \neq \overline{a}$, compute generators $g_2 := g_1^a, \overline{g}_2 := g_1^{\overline{a}}$, sample $\delta_2, \overline{\delta}_2 \getr \Z_q$. Let $\Delta = g_1^{\delta_1} \cdot g_2^{\delta_2}$ and $\overline{\Delta} = g_1^{\delta_1} \cdot \overline{g}_2^{\overline{\delta}_2}$.
\item Output $\sk = (\delta_1, \delta_2, \overline{\delta}_2)$ and $\vk = (\Delta, \overline{\Delta}, a, \overline{a})$.
\end{itemize}

\paragraph{\underline{
$\PreSign(\sk,m,X)$}:
}
\begin{itemize}
\item 
Sample $r_1, \overline{r}_1, r_2, \overline{r}_2 \getr \Z_q$.

\item 
Compute $h = H(X \cdot g_1^{r_1} \cdot g_2^{r_2} || m)$, 
$\widetilde{s}_1 = r_1 + h \cdot \delta_1$, 
$\widetilde{s}_2 = r_2 + h \cdot \delta_2$.

\item 
Compute $\overline{h} = H(X \cdot g_1^{\overline{r}_1} \cdot \overline{g}_2^{\overline{r}_2} || m)$, 
$\overline{\widetilde{s}}_1 = \overline{r}_1 + \overline{h} \cdot \delta_1$, 
$\overline{\widetilde{s}}_2 = \overline{r}_2 + \overline{h} \cdot \overline{\delta}_2$.

\item 
Output pre-signature $\widetilde{\sigma} := (h, \widetilde{s}_1, \widetilde{s}_2, \overline{h}, \overline{\widetilde{s}}_1, \overline{\widetilde{s}}_2)$.  
\end{itemize}

\paragraph{\underline{
$\PreVerify(\vk, m, X, \widetilde{\sigma})$}: 
}
\begin{itemize}
\item
Compute $g_1^R := X \cdot g_1^{\widetilde{s}_1} \cdot g_2^{\widetilde{s}_2} / \Delta^h$.
\item 
Compute $g_1^{\overline{R}} := X \cdot g_1^{\overline{\widetilde{s}}_1} \cdot \overline{g}_2^{\overline{\widetilde{s}}_2} / \overline{\Delta}^{\overline{h}}$.
\item 
Output $1$ iff $h = H(g_1^R || m)$ and $\overline{h} = H(g_1^{\overline{R}} || m)$.
\end{itemize}

\paragraph{\underline{
$\Adapt({\color{blue}\vk}, \widetilde{\sigma}, (x_1, x_2))$}: 
}
\nikhil{do we need to modify definition to allow using $\vk$ here?}
\begin{itemize}
\item 
Compute $s_1 = \widetilde{s}_1 + x_1$, $s_2 = \widetilde{s}_2 + x_2$, and $s = s_1 + a \cdot s_2$.
\item 
Compute $\overline{s}_1 = \overline{\widetilde{s}}_1 + x_1$, $\overline{s}_2 = \overline{\widetilde{s}}_2 + x_2$, and $\overline{s} = \overline{s}_1 + \overline{a} \cdot \overline{s}_2$.
\item 
Output two Schnorr signatures $\sigma = (h, s)$ and $\overline{\sigma} = (\overline{h}, \overline{s})$.

\end{itemize}

\paragraph{\underline{
$\Verify(\vk, m, (\sigma, \overline{\sigma}))$}: 
}
\begin{itemize}
\item 
Output $1$ iff $\Sch.\Verify(\Delta, m, \sigma) = 1$ and 
$\Sch.\Verify(\overline{\Delta}, m, \overline{\sigma}) = 1$.
\end{itemize}

\paragraph{\underline{
$\Ext({\color{blue}\vk}, \widetilde{\sigma}, (\sigma, \overline{\sigma}), X)$}: 
}
\nikhil{do we need to modify definition to allow using $\vk$ here?}
\begin{itemize}
\item 
Parse $\widetilde{\sigma} = (h, \widetilde{s}_1, \widetilde{s}_2, \overline{h}, \overline{\widetilde{s}}_1, \overline{\widetilde{s}}_2)$,
$\sigma = (h, s)$ and $\overline{\sigma} = (\overline{h}, \overline{s})$.
\item 
Compute $\widetilde{s} = \widetilde{s}_1 + a \cdot \widetilde{s}_2$ and 
$\overline{\widetilde{s}} = \overline{\widetilde{s}}_1 + a \cdot \overline{\widetilde{s}}_2$.
\item Compute $x'_1 := \frac{\overline{a} (s - \widetilde{s}) - a (\overline{s} - \overline{\widetilde{s}})}{\overline{a} - a}$, $x'_2 := \frac{(\overline{s} - \overline{\widetilde{s}}) - (s - \widetilde{s})}{\overline{a} - a}$.
\item Output $(x'_1, x'_2)$.
\end{itemize}

}

\input{as-construction-alt}










==> complex-fas-construction.tex <==
\section{Construction: Functional Adaptor Signature}
\label{sec:fas-construction}

Assume the following building blocks:
\begin{itemize}
\item 
A secure adaptor signature scheme $\as$ w.r.t.\ the Schnorr signature scheme $\Sch$ and the discrete log hard relation $R_{DL}$, where $\Sch$ is defined w.r.t.\ a cyclic group $\G$ of prime order $q$ and with generator $g$.
\item 
A selective, IND-secure inner product functional encryption scheme $\ipe$ 
with an additional public keygen algorithm that outputs $\pk_\bfy$ satisfying $(\pk_\bfy, \sk_\bfy) \in R_{DL}$:
\begin{itemize} 
\item 
$\pk_\bfy \leftarrow \PubKGen(\mpk, \bfy \in \Z_q^n)$:
it is a {\em deterministic} algorithm that 
takes in the master public key $\mpk$, and 
a vector $\bfy \in \Z_q^n$,
outputs a functional public key $\pk_\bfy$.
\end{itemize}
The IPE scheme by Abdalla et al.~\cite{ipe} based on the DDH assumption satisfies our requirements. Specifically, in their construction, $\msk = \bfs \getr \Z_q^n$, $\mpk = g^\bfs$, and $\sk_\bfy = \bfs^T \bfy$. Then, given $\mpk$ and $\bfy$, we can efficiently compute $\pk_\bfy = g^{ \bfs^T \bfy} := \Pi_{i \in [m]} (g^{s_i})^{y_i}$. This natural choice meets our requirement that $(\pk_\bfy, \sk_\bfy) \in R_{DL}$.
\item 
A non-interactive zero-knowledge proof system $\nizk$ in the common reference string model for the NP language $L_{NIZK}$ defined as\nikhil{blah relation}. 
\end{itemize}
Then, our functional adaptor signature scheme w.r.t.\ signature scheme $\Sch$, any hard relation $R$ with statement/witness pairs $(X, \bfx)$ such that $\bfx \in \Z_q^n$, and family of inner product functions $\mcal{F}_{IP, \Z_q^n} = \{y \in \Z_q^n\}$ on vectors in $\Z_q^n$ is as follows. 

\subsection{Construction}
\label{sec:construction}

\paragraph{$\Setup(1^\secparam, 1^n)$:}
\begin{itemize}[itemsep=0.1em]
\item Compute $\crs' \gets \nizk.\Setup(1^\secparam)$.
\nikhil{does the nizk setup need to take $1^n$ as input too?}
\item Compute $(G, q, g_1) \gets \GroupGen(1^\secparam)$ and sample generators $g_2, \overline{g}_2 \gets G$.
\item Output $\crs = (\crs', G, q, g_1, g_2, \overline{g}_2)$.
\end{itemize}

\paragraph{$\AdvertisementGen(1^n, \crs, X, \bfx)$:}
\begin{itemize}[itemsep=0.1em]
\item 
$(\mpk, \msk) \gets \ipe.\Setup(1^\secparam, 1^n, G, q, g_1, g_2)$. \nikhil{Here, $\msk = (\bfs, \bft), \mpk = g_1^\bfs g_2^\bft$.}
\item 
$\overline{\mpk} \gets \ipe.\AuxSetup(\msk, G, q, g_1, \overline{g}_2)$. \nikhil{New algorithm! Here, $\mpk_2 = g_1^\bfs \overline{g}_2^\bft$.}
\item 
Sample random coins $r$ and compute $\ct = \ipe.\Enc(\mpk, \bfx; r)$.
\item 
$\pi \gets \nizk.\Prove(\crs', (X, \mpk, \ct), (\bfx, r))$.
\item 
Output $\advt = (\mpk, \ct, \pi, \overline{\mpk})$, and $\state = \msk$.
\end{itemize}

\paragraph{$\AdvertisementVerify(\crs, X, \advt)$:}
output $\nizk.\Verify(\crs', (X, \mpk, \ct), \pi)$.

\paragraph{$\KGen(1^\secparam, \crs)$:} \nikhil{added crs as input}
output $(\vk, \sk) \gets \as.\KGen(1^\secparam, G, q, g_1)$. \nikhil{this keygen samples different $g_2, \overline{g}_2$ from that used by \ipe. need to make it the same! how?}

\paragraph{$\FPreSign(\advt, \sk, m, X, \bfy \in \mcal{F}^n_{IP})$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $Z = \ipe.\Commit(\mpk, \bfy)$. 
\nikhil{New algorithm! here $Z = \mpk^\bfy = g_1^{\bfs^T \bfy} g_2^{\bft^T \bfy}$.}
\item 
Compute $\overline{Z} = \ipe.\Commit(\overline{\mpk}, \bfy)$.
\nikhil{New algorithm! here $\overline{Z} = \overline{\mpk}^\bfy = g_1^{\bfs^T \bfy} \overline{g}_2^{\bft^T \bfy}$.}
\item 
Output $\widetilde{\sigma} \gets \as.\PreSign(\sk, m, Z, \overline{Z})$.
\nikhil{Note: pre-sign with respect to two statements.}

\end{itemize}

\paragraph{$\FPreVerify(\advt, \vk, m, X, \bfy, \widetilde{\sigma})$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $Z = \ipe.\Commit(\mpk, \bfy)$.
\item 
Compute $\overline{Z} = \ipe.\Commit(\overline{\mpk}, \bfy)$.
\item 
Output $\as.\PreVerify(\vk, m, Z, \overline{Z}, \widetilde{\sigma})$. 
\nikhil{Note: pre-verify with respect to two statements.}
\end{itemize}

\paragraph{$\Adapt(\advt, \vk, \state, \widetilde{\sigma}, \bfy, \bfx)$:}
\nikhil{added $\vk$ as input to the function}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$, and $\state = \msk$.
\item 
Compute $z = \ipe.\KGen(\msk, \bfy)$.
\item
Output $\sigma = \as.\Adapt(\vk, \widetilde{\sigma}, z)$.
\end{itemize}

\paragraph{$\Verify(\vk, m, \sigma)$:}
output $\as.\Verify(\vk, m, \sigma)$.

\paragraph{$\FExt(\advt, \vk, \widetilde{\sigma}, \sigma, X, \bfy)$:} 
\nikhil{added $\vk$ as input to the function}
\begin{itemize}[itemsep=0.1em]
\item
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $Z = \ipe.\Commit(\mpk, \bfy)$.
\item 
Compute $z = \as.\Ext(\vk, \widetilde{\sigma}, \sigma, Z)$.
\item 
Output $\bfx^T \bfy \gets \ipe.\Dec(z, \ct)$.

\end{itemize}

\subsection{Correctness}

\nikhil{todo}

\input{fas-proof}

==> conclusion.tex <==
\section{Conclusions}
In this work, we have presented a novel and practical approach to enable fair functional sales of information while offering improved efficiency, privacy, and compatibility similar to adaptor signatures.
Towards this, we presented functional adaptor signatures (FAS), a novel cryptographic primitive.
We formalized the security properties of FAS, among which is a new notion called witness privacy to capture seller’s privacy, which ensures the buyer does not learn anything beyond $f(x)$.
We presented a generic construction of FAS from AS, IPFE and NIZKs. We showed two ways to instantiate it from prime-order groups and lattices. 
We implemented the prime-order groups instantiation on ${\sf Secp256k1}$ elliptic curve and benchmarked our scheme for a wide range of parameter settings to demostrate practical efficiency.
Future work and open problems include exploring constructions for richer classes of functionality such as quadratic functions and attribute-based access control.

==> definitions.tex <==
\section{FAS Definition}\label{sec:FAS}

A functional adaptor signature scheme shares similar syntax to an adaptor signature scheme with few additional interfaces and parameters. 
Specifically, 
a functional adaptor signature scheme
$\FAS := (\Setup, \AdvertisementGen, \AdvertisementVerify, \AuxGen, \AuxVerify, \FPreSign, \FPreVerify, \allowbreak \Adapt, \FExt)$ 
is defined with respect to a signature scheme $\DS = (\KGen, \Sign, \Verify)$, a hard relation $R$, and a family of functions $\mcal{F}$. 
We recall that $(\AuxGen, \AuxVerify, \allowbreak \FPreSign)$ essentially denote the 3-round interactive pre-signing process. 
We defer formal description of syntax 
\ifcameraready
to the full version
\else
to~\Cref{def:fas-syntax} 
\fi
due to space constraints. 
% We describe the formal definition below.
 
%(a) the pre-signatures are computed not only w.r.t.\ an NP statement $X$ and a message $m$, but also w.r.t.\ some function $f$ and some auxiliary value $\aux_f$,
%(b) the auxiliary value $\aux_f$ is computed using an additional algorithm $\AuxGen$ and can be verified using $\AuxVerify$, 
%(c) the extract algorithm $\FExt$ extracts a function $f(x)$ of the witness from a valid pair of a pre-signature (w.r.t.\ $f, X$) and an adapted signature. The formal definition is given below.
%\nikhil{redo the above para based on final syntax}


% \begin{remark}
% We want the algorithm $\AuxGen$ to be \emph{consistent} in the sense that multiple calls to it on the same inputs produce the same outputs, for instance, in a stateful manner. 
% Looking ahead, this \emph{consistency} is used in the witness privacy security property against a malicious buyer. 
% In particular, before adapting a pre-signature $\widetilde{\sigma}$ obtained from the malicious buyer, the seller will run $\FPreVerify$ against the locally computed $\aux_f$.  
% %\nikhil{is this remark? Typically, this can be achieved if the algorithm is deterministice or stateful. In our constructions, it is achieved via statefulness, but there seems no reason to restrict the defintion that way.} 
% % \nikhil{Note that consistency is used in the ZK experiment. the Adapt oracle over there samples $(\aux_f, \_) \gets \AuxGen(\pp, \advt, f)$ on its own and runs $\FPreVerify$ of $\widetilde{\sigma}$ against this $\aux_f$.}
% % \anote{I would not say this line here. Rather I will add a remark after the definition and clarify we want this algorithm to be stateful.}

% \end{remark}

% \pnote{Where is $\Sign$?}
% \nikhil{done, added.}
% \nikhil{change $\FAS$ to $\FAS$ and same for DS.}


\smallskip\noindent\textbf{Correctness.} 
If everything is run honestly, then, $\FExt$ must return $f(x)$. We defer the formal details 
\ifcameraready
to the full version.
\else
to~\Cref{def:fas-correctness}.
\fi

\ifacm
\smallskip\noindent\textbf{Security.} 
% In terms of security, we want
% \emph{advertisement soundness},
% \emph{pre-signature validity},
% \emph{unforgeability}, 
% and \emph{witness extractability} 
% against an adversarial seller and 
% \emph{pre-signature adaptability} and 
% \emph{witness privacy} against an adversarial buyer as discussed in~\Cref{sec:overview-fas-security}.
Due to space constraints, we defer all properties (mentioned in~\Cref{sec:overview-fas-security}) except 
unforgeability and 
zero-knowledge witness privacy 
\ifcameraready
to the full version.
\else
to~\cref{sec:defs-appendix}.
\fi

% \begin{enumerate}[leftmargin=*]
% 	\item {\bf Advertisement soundness:} The property requires that given $\pp$, it should be infeasible for a \ppt malicious seller to find statement $X \notin L_R$ and advertisement $\advt$ such that $\advt$ is accepted by $\AdvertisementVerify$.
	
% 	\item {\bf Pre-signature validity:} This property says that given a valid auxiliary value, one can always compute a valid pre-signature using it. Intuitively, this tries to capture that it should be impossible for a malicious seller to give out a malformed auxiliary value for the function $f$ and yet learn an honestly generated pre-signature for $f$ that is valid.
	
% 	\item {\bf Unforgeability:} This is similar to the unforgeability typically defined for adaptor signatures~\cite{asig}.
% The property requires that even when the adversary (malicious seller) is given access to pre-signatures with respect to functions $f$ of its choice, it should not be able to forge signatures if it does not know the witness $x^*$ for the challenge statement $X^*$ in the first place.

% 	\item {\bf Witness extractability:} We require that for any function $f\in\mcal{F}$, for any honestly generated pre-signature w.r.t.\ $f$ and a valid signature, one should be able to extract the function evaluation $f$ on a witness. Intuitively, it tries to capture the interaction between an honest buyer (i.e., generates valid pre-signature) and a malicious seller trying to get paid (i.e., adapt pre-signature into a signature) without revealing evaluation of $f$ on witness (i.e., extraction failure) should be unlikely to occur.
% %This is similar to the witness extractability security property of adaptor signatures (See~\Cref{def:as-wit-ext}) except that in the formal witness extractability experiment~\Cref{fig:fasig-wit-ext-exp}, in step~\ref{step:z-inefficient}, computing the set $Z$ is inefficient.

% 	\item {\bf Pre-signature adaptability:} This property says that given a valid pre-signature and a witness for the instance, 
% one can always adapt the pre-signature into a valid signature.
% Intuitively, this tries to capture that it should be impossible for a malicious buyer to learn a function evaluation on a witness without making the payment. 
% This is similar to the pre-signature adaptability security property of adaptor signatures (See~\Cref{def:as-pre-sig-adaptability}).

% 	\item {\bf Witness Privacy:} Here we want that in an interaction between a malicious buyer wanting to learn function evaluation $f$ on the witness and an honest seller using witness $x$ to adapt the pre-signature into a valid signature, at the end the buyer should not be able to learn any information about $x$ beyond $f(x)$. There are different ways to capture this formally as described below. 
% %We consider various notions of witness privacy akin to those in functional encryption literature and zero-knowledge proofs literature as follows.
% \begin{itemize}[leftmargin=*]
% \item {\bf Zero-Knowledge:}
% for every $(X, x) \in R$, there exists a \ppt simulator $\Sim$ such that the adversary should not be able to guess whether it is interacting with a real-world challenger that is allowed to use the witness $x$ or the simulator $\Sim$ that is only allowed access to $f(x)$. 
% \item {\bf Witness Indistinguishability:}
% given two valid witnesses $x_0$ and $x_1$ for a statement $X \in L_R$, the adversary should not be able to guess which witness was used to adapt a pre-signature as long as $f(x_0) = f(x_1)$. This notion is meaningful only for languages that have at least two witnesses. 
% \item {\bf Witness Hiding:}
% for every $X \in L_R$, given valid pre-signature w.r.t.\ function $f$ and valid signature adapted from it, the adversary should not be able to guess a witness $x$ s.t. $(X, x) \in R$.
% \end{itemize}

% \end{enumerate}

\begin{figure}[t]
\ifhldiff
{\color{hldiffcolor}
\fi
\centering
\captionsetup{justification=centering}
% \fbox{
\begin{pcvstack}[boxed,space=1em]
\procedure[linenumbering, mode=text]{Experiment $\faSigForge_{\A,\FAS}(1^\secparam)$}{
$\mcal{Q} := \emptyset$, 
% \\ 
$\pp \gets \Setup(1^\secparam)$, 
% \\ 
$(\sk, \vk) \gets \KGen(1^\secparam)$ 
\\ 
$(X^*, x^*) \gets \GenR(1^\secparam)$
\\ 
% $\advt = \bot$ 
% \\ 
% $(\advt, m^*, f^*) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot)}(\pp, \vk, X^*)$ 
$(\advt, m^*, f^*, \aux_f^*, \pi_f^*) \gets \A^{\mcal{O}_S(\cdot)}(\pp, \vk, X^*) $ \\
% $(\advt, m^*, f^*, \aux_f^*, \pi_f^*)  $ \pcskipln \\
% $\qquad \qquad  \gets \A^{\mcal{O}_S(\cdot)}(\pp, \vk, X^*)$ 
% \\ 
\label{step:adverify}
If $\AdvertisementVerify(\pp, X^*, \advt) =0 \ \vee \ f^* \notin \mcal{F} $ 
\pcskipln \\
$\vee \ \AuxVerify(\advt, f^*, \aux_f^*, \pi_f^*)=0$ : 
\ret $0$ 
\\ 
$\widetilde{\sigma}^* \gets \FPreSign(\advt, \sk, m^*, X^*, f^*, \aux_f^*)$ 
\\ 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot, \cdot, \cdot)}(\widetilde{\sigma}^*)$ \\
\ret $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_S(m)$}{
$\sigma \gets \Sign(\sk, m)$,
% \\
$\mcal{Q} := \mcal{Q} \vee \{m\}$, 
% \\ 
\ret $ \sigma$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{\fpS}(m, X, f, \aux_f, \pi_f)$}{
If $\AuxVerify(\advt, f, \aux_f, \pi_f) = 0$: \ret $\bot$ \\
$\widetilde{\sigma} \gets \FPreSign(\advt, \sk, m, X, f, \aux_f)$, 
% \\ 
$\mcal{Q} := \mcal{Q} \vee \{m\}$, 
% \\ 
\ret $\widetilde{\sigma}$
}

\end{pcvstack}
% }
\caption{
\ifhldiff
{\color{hldiffcolor}
\fi
Unforgeability of functional adaptor signatures 
\ifhldiff
}
\fi
% \pnote{please see my comment on slack on the kind of access A is given to Pre-sign.}
% \nikhil{done}
}
\label{fig:fasig-unf-exp}
\ifhldiff
}
\fi
\end{figure}
\ifhldiff
{\color{hldiffcolor}
\fi
\smallskip\noindent\textbf{Unforgeability.} 
% This is similar to the unforgeability security property typically defined for adaptor signatures~\cite{asig}.
The property requires that even when the adversary (malicious seller) is given access to pre-signatures with respect to functions $f$ of its choice, it should not be able to forge signatures if it does not know the witness $x^*$ for the challenge statement $X^*$ in the first place. To capture this essence, the experiment (See~\Cref{fig:fasig-unf-exp}) samples $(X^*, x^*)$ at random. Beyond this, the adversary has all the powers of a (malicious) seller starting with generating $\advt$. A curious reader might ask if the adversary doesn't know $x^*$, then, wouldn't it typically fail to pass the $\AdvertisementVerify$ check in step~\ref{step:adverify} in~\Cref{fig:fasig-unf-exp} and thus rendering the experiment after that pointless? The answer is no, because \emph{advertisement soundness} is for statements not in the language $L_R$, but here $X^* \in L_R$ as the experiment chooses it.
% \anote{We do not seem to explain the subtlety about the $\advt$ verifying. }
\begin{definition}[Unforgeability]
A $\FAS$ scheme is $\faSigForge$-secure or simply unforgeable, if 
for every stateful \ppt adversary \A there exists a negligible function $\negl$ such that
for all $\secparam \in \N$,
$\Pr[ \faSigForge_{\A,\FAS}(1^\secparam) = 1] \leq \negl(\secparam)$,
where the experiment $\faSigForge_{\A,\FAS}$ 
is defined as in~\Cref{fig:fasig-unf-exp}.
% \nikhil{change $\faSigForge$ to something more readable}
% \nikhil{discuss why we use the weaker pre-sign oracle and not the stronger one proposed in the indocrypt'22 paper. }
% \anote{Something is wrong in the experiment. The oracle $\fpS$ will return $\bot$ always because $\advt = \bot$. It only becomes non-bot after step 6. That means the oracle access in step 6 is useless. Also, the adversary is required to output $\advt$ without knowing $x^*$. Isn't this already some form of a security violation? }
\end{definition}
\ifhldiff
}
\fi

\smallskip\noindent\textbf{Witness Privacy.}  We want that in an interaction between a malicious buyer wanting to learn function evaluation $f$ on the witness and an honest seller using witness $x$ to adapt the pre-signature into a valid signature, at the end the buyer learns no information beyond $f(x)$. The strongest way to capture this is via a simulation-style definition which we define as zero-knowledge.
Informally, zero-knowledge requires that there exists a \ppt simulator $\Sim$ such that the adversary's can't guess whether it is interacting with a real-world challenger that uses witness $x$ or an ideal-world challenger that only uses $f(x)$ via simulator $\Sim$. Formal details follow.

\begin{definition}[Zero-Knowledge]
\label{def:fas-zk}
% \pnote{this terminology makes no sense to me, perhaps just use ZK.}\nikhil{done}
A $\FAS$ scheme satisfies zero-knowledge if 
for every \ppt adversary \A, 
there exists a stateful \ppt simulator $\Sim = (\Setup^*, \AdGen^*, \AuxGen^*, \Adapt^*)$,
there exists a negligible function $\negl$ s.t.
for all \ppt distinguishers \D, 
for all $\secparam \in \N$, 
for all $(X, x) \in R$,
$| \Pr[\D(\faZKReal_{\A, \FAS}(1^\secparam, X, x)) = 1] - \Pr[ \D(\faZKIdeal_{\A, \FAS}^\Sim(1^\secparam, X, x)) = 1] | \leq  \negl(\secparam)$,
% \begin{align*}
% & | \Pr[\D(\faZKReal_{\A, \FAS}(1^\secparam, X, x)) = 1] \\ 
% & \quad - \Pr[ \D(\faZKIdeal_{\A, \FAS}^\Sim(1^\secparam, X, x)) = 1] | \leq  \negl(\secparam),
% \end{align*}
% \[
% | \Pr[ \faZKReal_{\A, \FAS}(1^\secparam) = 1] - \Pr[ \faZKIdeal_{\A, \FAS}^\Sim(1^\secparam) = 1] | \leq  \negl(\secparam),
% \]
where experiments $\faZKReal_{\A, \FAS}$ and $\faZKIdeal^\Sim_{\A, \FAS}$ are defined in~\Cref{fig:fas-zk-real,fig:fas-zk-ideal}.
% \pnote{I think we should standardize how we write advantages for decisional games: here it written as a difference of probabilities of $A$ whereas previously it the $1/2$ - negl version.} 
% \nikhil{done}
% \pnote{I think this definition needs to be refined to make it look similar to ZK -- e.g., for ZK there are two adversaries: the verifier who participates in the experiment, and the distinguisher who is given the \emph{view} (all messages including the output) of the verifier from the experiment.}
% \nikhil{done}

\end{definition}

% \anote{Split the below figure and put them into boxes}
\begin{figure}[t]
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed, space=1em]
\procedure[linenumbering, mode=text]{Experiment $\faZKReal_{\A,\FAS}(1^\secparam, X, x)$; $\pcbox{\faZKIdeal^\Sim_{\A,\FAS}(1^\secparam, X, x)}$}{
$\pp \gets \Setup(1^\secparam)$ $\pcbox{\Setup^*(1^\secparam)}$ 
\\ 
$(\advt, \state) \gets \AdvertisementGen(\pp, X, x)$ $\pcbox{\AdGen^*(\pp, X)}$ 
\\
% ;\   \pcbox{\AdvertisementGen^*(\pp, X)}$ 
% \\ 
$\vk := \bot$
\\ 
$\vk \gets \A^{\mcal{O}_{\AuxGen}(\cdot), \mcal{O}_{\Adapt}(\cdot, \cdot, \cdot)}(\pp, \advt, X)$;  \pcskipln \\
$\pcbox{\vk \gets \A^{\mcal{O}^*_{\AuxGen}(\cdot, \cdot), \mcal{O}^*_{\Adapt}(\cdot, \cdot, \cdot, \cdot)}(\pp, \advt, X)}$
\\ 
\ret view of $\A$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{\AuxGen}(f);\ \pcbox{\mcal{O}^*_{\AuxGen}(f, f(x))}$.}{
\ret $(\aux_f, \pi_f) \gets \AuxGen(\advt, \state, f);\ \pcbox{\AuxGen^*(\advt, f, f(x))}$  
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{\Adapt}(m, f, \widetilde{\sigma});\ \pcbox{\mcal{O}^*_{\Adapt}(m, f, \widetilde{\sigma}, f(x))}$.}{
If $\vk = \bot$: \ret $\bot$
\\ 
$(\aux_f, \pi_f) \gets \AuxGen(\advt, \state, f);\ \pcbox{\AuxGen^*(\advt, f, f(x))}$ 
\\ 
If $\FPreVerify(\advt, \vk, m, X, f, \aux_f, \pi_f, \widetilde{\sigma}) = 0$: \ret $\bot$
\\ 
\ret $\sigma := \Adapt(\advt, \state, \vk, m, X, x, f, \aux_f, \widetilde{\sigma})$  \pcskipln \\
$\pcbox{\ret \ \sigma :=  \Adapt^*(\advt, \vk, m, X, f, \aux_f, \widetilde{\sigma}, f(x))}$
}

\end{pcvstack}

\caption{Zero-Knowledge experiments of FAS
% , with real-world experiment in plain while the changes for the ideal-world experiment are in a $\pcbox{\text{box}}$.
}
\label{fig:fas-zk-real}
\label{fig:fas-zk-ideal}
\end{figure}
\iffalse
\begin{figure}[t]
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed, space=1em]
\procedure[linenumbering, mode=text]{Experiment $\faZKIdeal^\Sim_{\A,\FAS}(1^\secparam, X, x)$.}{
$\pp \gets \Setup^*(1^\secparam)$
\\ 
$\advt \gets \AdvertisementGen^*(\pp, X)$
% \nikhil{ZK is never defined wrt random X, so don't sample $X$ randomly. But quantify over all possilbe $X \in L_R$, this will result in non-adaptive ZK, but let's live with it for the moment and try to argue if its achievable or not. If it is not achievable (maybe it contradicts unforgeability?), then, we are done here and this acts as motivation for WI and WH. If it is achievable, then, we can think of strengthening it.}
\\ 
% \pnote{Why is the simulator choosing $X$, this is like letting the ZK simulator choose the statement it want to simulate proofs for. This is incorrect.}
% \nikhil{fixed}
$\vk := \bot$ 
\\ 
$\vk \gets \A^{\mcal{O}^*_{\AuxGen}(\cdot, \cdot), \mcal{O}^*_{\Adapt}(\cdot, \cdot, \cdot, \cdot)}(\pp, \advt, X)$ 
\\ 
\ret view of $\A$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}^*_{\AuxGen}(f, f(x))$.}{
\ret $(\aux_f, \pi_f) \gets \AuxGen^*(\advt, f, f(x))$  
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}^*_{\Adapt}(m, f, \widetilde{\sigma}, f(x))$.}{
If $\vk = \bot$: return $\bot$
\\ 
$(\aux_f, \pi_f) \gets \AuxGen^*(\advt, f, f(x))$ 
\pcskipln \\ \nikhil{note aux}
\\
If $\FPreVerify(\advt, \vk, m, X, f, \aux_f, \pi_f, \widetilde{\sigma}) = 0$: \ret $\bot$
\\ 
\ret $\sigma \gets \Adapt^*(\advt, \vk, m, X, f, \aux_f, \widetilde{\sigma}, f(x))$    
}

\end{pcvstack}

\caption{Zero-Knowledge: ideal world experiment of functional adaptor signatures}
\label{fig:fas-zk-ideal}
\end{figure}
\fi 
\else
% and unlinkability against a malicous observer. 
% \nikhil{Check with Pratik and Aravind: should we also add unlinkability?}
% \pnote{since this is the new contribution, we should discuss this more at length as WI is not the most natural definition of privacy (ZK is)}
% \nikhil{done}
% \anote{These are in the context of adaptor signatures where the adversary receives pre-signatures. The current write-up is not clear as to what additional power the adversary gets apart from the statement $X$. I would also expand the security notions with intuitions for the experiments at the respective security definitions.}
\smallskip\noindent\textbf{Advertisement Soundness.} The property requires that given $\pp$, it should be infeasible for a \ppt malicious seller to find statement $X \notin L_R$ and advertisement $\advt$ such that $\advt$ is accepted by $\AdvertisementVerify$.
% \pnote{is this required? or can we live with a "computational" version?}
% \nikhil{yes, TODO: change}

\begin{definition}[Advertisement Soundness]
\label{def:fas-ad-sound}
A functional adaptor signature scheme $\FAS$ satisfies advertisement soundness if 
for every \ppt adversary \A, there exists a negligible function $\negl$ such that for all 
$\secparam \in \N$, for all NP languages $L_R$, $\pp \gets \Setup(1^\secparam)$, $(X, \advt) \gets \A(\pp)$,
% \nikhil{X is fixed before $crs$ making it non-adaptive soundness. Change quantifiers to get adaptive soundness. Also change to computational version.}
\[
\Pr[X \notin L_R \ \wedge \ \AdvertisementVerify(\pp, X, \advt) = 1 ] \leq \negl(\secparam).
\]
\end{definition}

\smallskip\noindent\textbf{Pre-signature validity.}
This property says that given a valid auxiliary value, one can always compute a valid pre-signature using it. Intuitively, this tries to capture that it should be impossible for a malicious seller to give out a malformed auxiliary value for the function $f$ and yet learn an honestly generated pre-signature for $f$ that is valid.

\begin{definition}[Pre-signature Validity]
A functional adaptor signature scheme $\fas$ satisfies pre-signature validity if for 
any $\secparam \in \N$, 
any $\pp \gets \Setup(1^\secparam)$, 
any $X, \advt$ such that $\AdvertisementVerify(\pp, \advt, $ $X)=1$,
any message $m\in \{0,1\}^*$,
any function class $\mcal{F}$,
any function $f \in \mcal{F}$,
any $(\aux_f, \pi_f)$, 
any key pair $(\sk, \vk) \gets \KGen(1^\secparam)$,
any pre-signature $\widetilde{\sigma} \gets \FPreSign(\advt, \sk, m, X, f, \aux_f)$, 
we have that if $\AuxVerify(\advt, f, \aux_f, \pi_f)=1$, then, 
\[
\Pr[\FPreVerify(\advt, \vk, m, X, f, \aux_f, \pi_f, \widetilde{\sigma})=1]=1.
\]
\end{definition}
% The property requires that an auxiliary value $\aux_f$ should be binding to the function $f$.
% \nikhil{I don't think we need this. I don't think it can even be satisfied. Reason for the latter: in constructions, $\aux_f$ is binding to $\sk_f$ and not $f$. There is no requirement in FE that $\sk_{f_0}$ and $\sk_{f_1}$ can't be the same for different $f_0$ and $f_1$, ie, $\sk_f$ need not be binding to $f$. Further, in our constructions, even if buyer requests for $f_0$ but gets auxiliary information for $f_1$, as long as $\pk_{f_0} = \pk_{f_1}$, it is guaranteed that IPFE decryption will allow buyer to learn $f_0(x)$ because IPFE decryption algorithm implicitly takes $f$ as input in addition to $\sk_f$. So, after extracting $\sk_{f_1}$, the buyer will run $\ipfe.\Dec(f_0, \sk_{f_1}, \ct)$.}

% \begin{definition}[Auxiliary Value Binding]
% A functional adaptor signature scheme $\FAS$ satisfies auxiliary value binding if 
% for all $\secparam \in \N, X \in L_R$, for $\pp \gets \Setup(1^\secparam)$, for any $\advt$ such that $\AdvertisementVerify(\pp, X, \advt)=1$, 
% \[
% \Pr\left[
% \begin{matrix}
% \exists \ f_0, f_1, \pi_0, \pi_1, \aux\ s.t.\\ 
% \AuxVerify(\advt, f_0, \aux, \pi_0) = 1 \ \wedge \\ 
% \AuxVerify(\advt, f_1, \aux, \pi_1) = 1
% \end{matrix}
% \right] \leq \negl(\secparam).
% \]

% \end{definition}

\ignore{
	
			\begin{definition}[Unforgeability (Old)]
			A functional adaptor signature scheme $\FAS$ is faEUF-CMA secure if 
			for every stateful \ppt adversary \A there exists a negligible function $\negl$ such that

			\[
			\Pr[ \faSigForge_{\A,\FAS}(1^\secparam) = 1] \leq \negl(\secparam),
			\]
			where the experiment $\faSigForge_{\A,\FAS}$ 
			is defined as in~\Cref{fig:fasig-unf-exp-old}.

			\end{definition}

			\begin{figure}[H]
			\centering
			\captionsetup{justification=centering}
			\begin{mdframed}
			\begin{multicols}{2}

			\paragraph{Experiment $\faSigForge_{\A,\FAS}$.} 

			\begin{enumerate}
			\item 
			$\mcal{Q} := \emptyset$
			\item 
			$\pp \gets \Setup(1^\secparam)$
			\item 
			$(\sk, \vk) \gets \KGen(1^\secparam)$
			\item 
			$(X, x) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot)}(\pp, \vk)$
			\item 
			$(\advt, \state) \gets \AdvertisementGen(\pp, X, x)$
			\item 
			$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot)}(\advt)$
			\item $f \getr \mcal{F}$
			% \nikhil{\A should not be allowed to choose $f$}
			\item 
			$\widetilde{\sigma} \gets \FPreSign(\advt, \sk, m, X, f)$
			\item 
			$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot)}(\widetilde{\sigma}, f)$
			\item 
			return $((m \notin \mcal{Q}) \wedge \Verify(\vk, m, \sigma))$
			\end{enumerate}

			\vfill\null 
			\columnbreak 

			\paragraph{Oracle $\mcal{O}_S(m)$.}
			\begin{enumerate}
			\item 
			$\sigma \gets \Sign(\sk, m)$
			\item 
			$\mcal{Q} := \mcal{Q} \vee \{m\}$
			\item 
			return $\sigma$
			\end{enumerate}

			\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, f)$.}
			\begin{enumerate}
			\item 
			$\widetilde{\sigma} \gets \FPreSign(\advt, \sk, m, X, f)$
			\item 
			$\mcal{Q} := \mcal{Q} \vee \{m\}$
			\item 
			return $\widetilde{\sigma}$
			\end{enumerate}
			\vfill\null

			\end{multicols}
			\end{mdframed}
			\caption{Unforgeability experiment of adaptor signatures}
			\label{fig:fasig-unf-exp-old}
			\end{figure}

			\nikhil{the previous definition did not seem very meaningful. the following is a better proposal}
}

\smallskip\noindent\textbf{Unforgeability.} 
This is similar to the unforgeability security property typically defined for adaptor signatures~\cite{asig}.
The property requires that even when the adversary (malicious seller) is given access to pre-signatures with respect to functions $f$ of its choice, it should not be able to forge signatures if it does not know the witness $x^*$ for the challenge statement $X^*$ in the first place. To capture this essence, the experiment (See~\Cref{fig:fasig-unf-exp}) samples $(X^*, x^*)$ at random. Beyond this, the adversary has all the powers of a (malicious) seller starting with generating $\advt$. A curious reader might ask if the adversary doesn't know $x^*$, then, wouldn't it typically fail to pass the $\AdvertisementVerify$ check in step~\ref{step:adverify} in~\Cref{fig:fasig-unf-exp} and thus rendering the experiment after that pointless? The answer is no, because \emph{advertisement soundness} is for statements not in the language $L_R$, but here $X^* \in L_R$ as the experiment chooses it.

% \anote{We do not seem to explain the subtlety about the $\advt$ verifying. }

\begin{definition}[Unforgeability]
A functional adaptor signature scheme $\FAS$ is $\faSigForge$-secure or simply unforgeable, if 
for every stateful \ppt adversary \A there exists a negligible function $\negl$ such that
for all $\secparam \in \N$,
\[
\Pr[ \faSigForge_{\A,\FAS}(1^\secparam) = 1] \leq \negl(\secparam),
\]
where the experiment $\faSigForge_{\A,\FAS}$ 
is defined as in~\Cref{fig:fasig-unf-exp}.
% \nikhil{change $\faSigForge$ to something more readable}
\nikhil{discuss why we use the weaker pre-sign oracle and not the stronger one proposed in the indocrypt'22 paper. }
% \anote{Something is wrong in the experiment. The oracle $\fpS$ will return $\bot$ always because $\advt = \bot$. It only becomes non-bot after step 6. That means the oracle access in step 6 is useless. Also, the adversary is required to output $\advt$ without knowing $x^*$. Isn't this already some form of a security violation? }
\end{definition}

\begin{figure}[t]
\centering
\captionsetup{justification=centering}
% \fbox{
\begin{pcvstack}[boxed,space=1em]
\begin{pchstack}
\procedure[linenumbering, mode=text]{Experiment $\faSigForge_{\A,\FAS}(1^\secparam)$}{
$\mcal{Q} := \emptyset$ 
\\ 
$\pp \gets \Setup(1^\secparam)$ 
\\ 
$(\sk, \vk) \gets \KGen(1^\secparam)$ 
\\ 
$(X^*, x^*) \gets \GenR(1^\secparam)$ 
\\ 
% $\advt = \bot$ 
% \\ 
% $(\advt, m^*, f^*) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot)}(\pp, \vk, X^*)$ 
$(\advt, m^*, f^*, \aux_f^*, \pi_f^*) $ \pcskipln \\
$\qquad \qquad  \gets \A^{\mcal{O}_S(\cdot)}(\pp, \vk, X^*)$ 
\\ 
\label{step:adverify}
If $\AdvertisementVerify(\pp, X^*, \advt) =0 \ \vee \ f^* \notin \mcal{F} $ 
\pcskipln \\
$\vee \ \AuxVerify(\advt, f^*, \aux_f^*, \pi_f^*)=0$ : 
\pcskipln \\
$\pcind$ \ret $0$ 
\\ 
$\widetilde{\sigma}^* \gets \FPreSign(\advt, \sk, m^*, X^*, f^*, \aux_f^*)$ 
\\ 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot, \cdot, \cdot)}(\widetilde{\sigma}^*)$ \\
\ret $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_S(m)$}{
$\sigma \gets \Sign(\sk, m)$
\\
$\mcal{Q} := \mcal{Q} \vee \{m\}$ 
\\ 
\ret $ \sigma$
}

\end{pchstack}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{\fpS}(m, X, f, \aux_f, \pi_f)$}{
If $\AuxVerify(\advt, f, \aux_f, \pi_f) = 0$: \ret $\bot$ \\
$\widetilde{\sigma} \gets \FPreSign(\advt, \sk, m, X, f, \aux_f)$ 
\\ 
$\mcal{Q} := \mcal{Q} \vee \{m\}$ 
\\ 
\ret $\widetilde{\sigma}$
}

\end{pcvstack}
% }
\caption{Unforgeability of functional adaptor signatures 
% \pnote{please see my comment on slack on the kind of access A is given to Pre-sign.}
% \nikhil{done}
}
\label{fig:fasig-unf-exp}
\end{figure}
% We also require that, given a pre-signature and a witness for the instance, 
% one can always adapt the pre-signature into a valid signature (pre-signature adaptability).
% \nikhil{comment on it being private and need for $\state$}
% Finally, we require that, given a valid pre-signature and a signature with respect to the same instance, one can efficiently {\color{blue}extract the function evaluation on the corresponding witness} (witness extractability).
% \nikhil{is the definition assuming unique-witness languages?}
\smallskip\noindent\textbf{Witness extractability.}
Here we require that for any function $f\in\mcal{F}$, for any honestly generated pre-signature w.r.t.\ $f$ and a valid signature, one should be able to extract the function evaluation $f$ on a witness. Intuitively, it tries to capture the interaction between an honest buyer (i.e., generates valid pre-signature) and a malicious seller trying to get paid (i.e., adapt pre-signature into a valid signature) without revealing function evaluation $f$ on a witness (i.e., extraction failure) should be unlikely to occur.
This is similar to the witness extractability security property of adaptor signatures (See~\Cref{def:as-wit-ext}) except that in the formal witness extractability experiment~\Cref{fig:fasig-wit-ext-exp}, in step~\ref{step:z-inefficient}, computing the set $Z$ is inefficient.

% \nikhil{is the definition assuming unique-witness languages?}

\begin{definition}[Witness Extractability]
A functional adaptor signature scheme $\FAS$ is $\faWitExt$-secure or simply witness extractable, if 
for every stateful \ppt adversary \A, there exists a negligible function $\negl$ such that 
for all $\secparam \in \N$,
\[
\Pr[ \faWitExt_{\A, \FAS}(1^\secparam) = 1] \leq \negl(\secparam),
\]
where the experiment $\faWitExt_{\A, \FAS}$ is defined as in~\Cref{fig:fasig-wit-ext-exp}.
\end{definition}

% \anote{The check with $\advt = \bot$. The adversary has to somehow set it before the oracle query.}

\begin{figure}[t]
\centering
\captionsetup{justification=centering}
% \fbox{
\begin{pcvstack}[boxed, space=1em]
\begin{pchstack}
\procedure[linenumbering, mode=text]{Experiment $\faWitExt_{\A,\FAS}(1^\secparam)$}{
$\mcal{Q} := \emptyset$ 
\\ 
$\pp \gets \Setup(1^\secparam)$ 
\\ 
$(\sk, \vk) \gets \KGen(1^\secparam)$ 
\\ 
% $\advt = \bot$ 
% \\ 
$(X^*, \advt, m^*, f^*, \aux_f^*, \pi_f^*)$ \pcskipln \\
$\qquad \qquad \gets \A^{\mcal{O}_S(\cdot)}(\pp, \vk)$ 
\\ 
If $\AdvertisementVerify(\pp, X^*, \advt) =0 \ \vee \ f^* \notin \mcal{F}$
\pcskipln \\
$\vee \ \AuxVerify(\advt, f^*, \aux_f^*, \pi_f^*)=0$ 
\pcskipln \\
$\pcind$ \ret $0$ 
\\ 
$\widetilde{\sigma}^* \gets \FPreSign(\advt, \sk, m^*, X^*, f^*, \aux_f^*)$ 
\\ 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot, \cdot, \cdot)}(\widetilde{\sigma}^*)$ 
\\
$z := \FExt(\advt, \widetilde{\sigma}^*, \sigma^*, X^*, f^*, \aux_f^*)$ \\
\label{step:z-inefficient}
Let $Z = \{ f^*(x) : \exists \ x\ s.t.\ (X^*, x) \in R\}$ \\
% \nikhil{computing set $W$ requires to find all witnesses $x$ for the statement $X$ which is going to be inefficient.}
$b := ((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*) \wedge (z \notin Z))$ \\
\ret $b$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_S(m)$}{
$\sigma \gets \Sign(\sk, m)$
\\
$\mcal{Q} := \mcal{Q} \vee \{m\}$ 
\\ 
\ret $\sigma$
}

\end{pchstack}



\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{\fpS}(m, X, f, \aux_f, \pi_f)$}{
% If $\advt = \bot$: return $\bot$ 
% \\ 
If $\AuxVerify(\advt, f, \aux_f, \pi_f) = 0$: \ret $\bot$
\\
$\widetilde{\sigma} \gets \FPreSign(\advt, \sk, m, X, f)$ 
\\ 
$\mcal{Q} := \mcal{Q} \vee \{m\}$ 
\\ 
\ret $\widetilde{\sigma}$
}
\end{pcvstack}
% }
\caption{Witness Extractability of functional adaptor signatures}
\label{fig:fasig-wit-ext-exp}

\end{figure}
\smallskip\noindent\textbf{Pre-signature adaptability.} 
This property says that given a valid pre-signature and a witness for the instance, 
one can always adapt the pre-signature into a valid signature.
Intuitively, this tries to capture that it should be impossible for a malicious buyer to learn a function evaluation on a witness without making the payment. 
This is similar to the pre-signature adaptability security property of adaptor signatures (See~\Cref{def:as-pre-sig-adaptability}).
% \nikhil{comment on it being private and need for $\state$}

\begin{definition}[Pre-signature Adaptability]
\label{def:fas-pre-sig-adaptability}
A functional adaptor signature scheme $\FAS$ satisfies pre-signature adaptability 
if for any $\secparam \in \N$,
any $\pp \gets \Setup(1^\secparam)$, 
any statement/witness pair $(X, x) \in R$, 
any $(\advt, \state) \gets \AdvertisementGen(\pp, X, x)$,
any message $m \in \{0,1\}^*$, 
any function class $\mcal{F}$, 
any function $f \in \mcal{F}$,
any $(\aux_f, \pi_f) $ $\gets \AuxGen(\advt, \state, f)$,
any key pair $(\sk, \vk) \gets \KGen(1^\secparam)$, 
and any pre-signature $\widetilde{\sigma} \in \{0,1\}^*$ 
with $\FPreVerify(\advt, $ $\vk, m, X, f, \aux_f, \pi_f,\allowbreak \widetilde{\sigma}) = 1$, we have:
\[
\Pr[\Verify(\vk, m, \Adapt(\advt, \state, \vk, m, X, x, f, \aux_f, \widetilde{\sigma})) = 1] = 1.
\]
\end{definition}

\smallskip\noindent\textbf{Witness privacy.} 
Here we want that in an interaction between a malicious buyer wanting to learn function evaluation $f$ on the witness and an honest seller using witness $x$ to adapt the pre-signature into a valid signature, at the end the buyer should not be able to extract any information about $x$ beyond $f(x)$. There are different ways to capture this formally. 
We consider various notions of witness privacy akin to those in functional encryption literature and zero-knowledge proofs literature as follows.
\begin{itemize}[leftmargin=*]
\item {\bf Zero-Knowledge:}
for every $(X, x) \in R$, there exists a \ppt simulator $\Sim$ such that the adversary should not be able to guess whether it is interacting with a real-world challenger that is allowed to use the witness $x$ or the simulator $\Sim$ that is only allowed access to $f(x)$. 
\item {\bf Witness Indistinguishability:}
given two valid witnesses $x_0$ and $x_1$ for a statement $X \in L_R$, the adversary should not be able to guess which witness was used to adapt a pre-signature as long as $f(x_0) = f(x_1)$. This notion is meaningful only for languages that have at least two witnesses. 
\item {\bf Witness Hiding:}
for every $X \in L_R$, given valid pre-signature w.r.t.\ function $f$ and valid signature adapted from it, the adversary should not be able to guess a witness $x$ s.t. $(X, x) \in R$.
\end{itemize}

Zero-Knowledge is the strongest among the three and we describe it next. Witness Indistinguishability and Witness Hiding are defined in~\Cref{sec:defs-appendix}.

\begin{definition}[Zero-Knowledge]
\label{def:fas-zk}
% \pnote{this terminology makes no sense to me, perhaps just use ZK.}\nikhil{done}
A functional adaptor signature scheme $\FAS$ satisfies zero-knowledge if 
for every stateful \ppt adversary \A, 
there exists a stateful \ppt simulator $\Sim = (\Setup^*, $ $\AdvertisementGen^*, \AuxGen^*, \Adapt^*)$ and 
there exists a negligible function $\negl$ such that
for all \ppt distinguishers \D, 
for all $\secparam \in \N$, 
for all $(X, x) \in R$,
$| \Pr[\D(\faZKReal_{\A, \FAS}(1^\secparam, X, x)) = 1] - \Pr[ \D(\faZKIdeal_{\A, \FAS}^\Sim(1^\secparam, X, x)) = 1] | \leq  \negl(\secparam)$,
% \begin{align*}
% & | \Pr[\D(\faZKReal_{\A, \FAS}(1^\secparam, X, x)) = 1] \\ 
% & \quad - \Pr[ \D(\faZKIdeal_{\A, \FAS}^\Sim(1^\secparam, X, x)) = 1] | \leq  \negl(\secparam),
% \end{align*}
% \[
% | \Pr[ \faZKReal_{\A, \FAS}(1^\secparam) = 1] - \Pr[ \faZKIdeal_{\A, \FAS}^\Sim(1^\secparam) = 1] | \leq  \negl(\secparam),
% \]
where the real-world experiment $\faZKReal_{\A, \FAS}$ and the ideal-world experiment $\faZKIdeal^\Sim_{\A, \FAS}$ are defined as in~\Cref{fig:fas-zk-real,fig:fas-zk-ideal}.
% \pnote{I think we should standardize how we write advantages for decisional games: here it written as a difference of probabilities of $A$ whereas previously it the $1/2$ - negl version.} 
% \nikhil{done}
% \pnote{I think this definition needs to be refined to make it look similar to ZK -- e.g., for ZK there are two adversaries: the verifier who participates in the experiment, and the distinguisher who is given the \emph{view} (all messages including the output) of the verifier from the experiment.}
% \nikhil{done}

\end{definition}

% \anote{Split the below figure and put them into boxes}
\begin{figure}[t]
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed, space=1em]
\procedure[linenumbering, mode=text]{Experiment $\faZKReal_{\A,\FAS}(1^\secparam, X, x)$.}{
$\pp \gets \Setup(1^\secparam)$ 
\\ 
$(\advt, \state) \gets \AdvertisementGen(\pp, X, x)$ 
\\ 
$\vk := \bot$
\\ 
$\vk \gets \A^{\mcal{O}_{\AuxGen}(\cdot), \mcal{O}_{\Adapt}(\cdot, \cdot, \cdot)}(\pp, \advt, X)$ 
\\ 
\ret view of $\A$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{\AuxGen}(f)$.}{
\ret $(\aux_f, \pi_f) \gets \AuxGen(\advt, \state, f)$  
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{\Adapt}(m, f, \widetilde{\sigma})$.}{
If $\vk = \bot$: \ret $\bot$
\\ 
$(\aux_f, \pi_f) \gets \AuxGen(\advt, \state, f)$ 
\pcskipln \\ \nikhil{note aux}
\\ 
If $\FPreVerify(\advt, \vk, m, X, f, \aux_f, \pi_f, \widetilde{\sigma}) = 0$: \ret $\bot$
\\ 
\ret $\sigma := \Adapt(\advt, \state, \vk, m, X, x, f, \aux_f, \widetilde{\sigma})$  
}

\end{pcvstack}

\caption{Zero-Knowledge: real world experiment of functional adaptor signatures}
\label{fig:fas-zk-real}
\end{figure}
\begin{figure}[t]
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed, space=1em]
\procedure[linenumbering, mode=text]{Experiment $\faZKIdeal^\Sim_{\A,\FAS}(1^\secparam, X, x)$.}{
$\pp \gets \Setup^*(1^\secparam)$
\\ 
$\advt \gets \AdvertisementGen^*(\pp, X)$
% \nikhil{ZK is never defined wrt random X, so don't sample $X$ randomly. But quantify over all possilbe $X \in L_R$, this will result in non-adaptive ZK, but let's live with it for the moment and try to argue if its achievable or not. If it is not achievable (maybe it contradicts unforgeability?), then, we are done here and this acts as motivation for WI and WH. If it is achievable, then, we can think of strengthening it.}
\\ 
% \pnote{Why is the simulator choosing $X$, this is like letting the ZK simulator choose the statement it want to simulate proofs for. This is incorrect.}
% \nikhil{fixed}
$\vk := \bot$ 
\\ 
$\vk \gets \A^{\mcal{O}^*_{\AuxGen}(\cdot, \cdot), \mcal{O}^*_{\Adapt}(\cdot, \cdot, \cdot, \cdot)}(\pp, \advt, X)$ 
\\ 
\ret view of $\A$
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}^*_{\AuxGen}(f, f(x))$.}{
\ret $(\aux_f, \pi_f) \gets \AuxGen^*(\advt, f, f(x))$  
}

\procedure[linenumbering, mode=text]{Oracle $\mcal{O}^*_{\Adapt}(m, f, \widetilde{\sigma}, f(x))$.}{
If $\vk = \bot$: \ret $\bot$
\\ 
$(\aux_f, \pi_f) \gets \AuxGen^*(\advt, f, f(x))$ 
\pcskipln \\ \nikhil{note aux}
\\
If $\FPreVerify(\advt, \vk, m, X, f, \aux_f, \pi_f, \widetilde{\sigma}) = 0$: \ret $\bot$
\\ 
\ret $\sigma \gets \Adapt^*(\advt, \vk, m, X, f, \aux_f, \widetilde{\sigma}, f(x))$    
}

\end{pcvstack}

\caption{Zero-Knowledge: ideal world experiment of functional adaptor signatures}
\label{fig:fas-zk-ideal}
\end{figure}
% 
% \pnote{Do we achieve this notion for our construction? How does the simulator simulate? Naive thought would be that since simulator has signing key, then it can compute a valid sigma without knowing the witness. But since Ext is a public algorithm (is it?), A can also compute the witness by extracting -- note that adapted signature must be at least indistinguishable from valid pre-signatures.}
% \nikhil{we can achieve this notion if we are given Adaptor Signatures for NP. To achieve this, we need simulation-secure IPFE [Wee16]. In [Wee16], public and private functional keys satisfy $\DLstar$ relation, hence we need Adaptor Signatures for NP. The simulator is as follows: $\AdvertisementGen^*$ output $\advt = (\mpk, \ct^*, \pi^*)$ as follows: use IPFE in simulation mode to generate $(\mpk, \msk^*) \gets \ipe.\widetilde{\Setup}(\pp)$, $\ct^* \gets \ipe.\widetilde{\Enc}(\msk^*)$, the NIZK proof $\pi^*$ comes from the NIZK simulator. $\AuxGen^*$ computes $\sigma$ by running adapt algorithm. Adapt algorithm needs as input $\sk_f$ which it obtains from IPFE simulator as $\sk_f = \ipe.\widetilde{\KGen}(\msk^*, f, f(x))$.}
% \pnote{Why is A allowed to choose vk?}
% \nikhil{Intuitively, in witness-privacy we are trying to protect against adversarial buyer. The buyer controls $(\sk, \vk)$, hence, I allowed \A to choose it.}
% 
% \ignore{
% 
% \section{Construction}
% 
% We will construct a functional adaptor signature scheme
% $\FAS := (\KGen, \FPreSign, \FPreVerify, \Adapt, \Verify, \FExt)$ 
% with respect to a signature scheme $\DS$, a hard relation $R$, and {\color{blue}a family of inner product functions $\mcal{F}$}. 
% 
% Let $\ipe = (\ipe.\Setup, \ipe.\KGen, \ipe.\Enc, \ipe.\Dec)$ be an inner product functional encryption scheme.
% Let $(\KGen', \PreSign', \PreVerify', \Adapt', \Verify', \Ext')$ be an adaptor signature scheme defined with respect to a signature scheme $\DS$ 
% and a hard relation $R'$.
% \nikhil{define the relation $R'$.}
% Then, the construction is as follows.
% 
% \paragraph{\underline{
% $\KGen(1^\secparam)$
% }:}
% \begin{itemize}
% \item 
% Compute $(\sk, \vk) \gets \KGen'(1^\secparam)$.
% \item 
% Compute $(\ipe.\msk, \ipe.\mpk) \gets \ipe.\Setup(1^\secparam)$.
% Output $(\sk, \vk, \advt)$.
% \end{itemize}
% 
% \paragraph{\underline{
% ${\FPreSign}(\advt, \sk, m, X, f)$
% }:}
% \begin{itemize}
% \item 
% Output $\widetilde{\sigma}$.
% \end{itemize}
% 
% \paragraph{\underline{
% ${\FPreVerify}(\advt, \vk, m, X, f, \widetilde{\sigma})$
% }:}
% \begin{itemize}
% \item 
% Output .
% \end{itemize}
% 
% \paragraph{\underline{
% $\Adapt(\widetilde{\sigma}, x)$ 
% }:}
% \begin{itemize}
% \item 
% Output $\sigma$.
% \end{itemize}
% 
% \paragraph{\underline{
% $\Verify(\vk, m, \sigma)$
% }:}
% \begin{itemize}
% \item 
% Output.
% \end{itemize}
% 
% \paragraph{\underline{
% ${\FExt}(\widetilde{\sigma}, \sigma, X)$ 
% }:}
% \begin{itemize}
% \item 
% Output $f(x)$.
% \end{itemize}
% 
% }
\fi 
\begin{definition}[Strongly-secure Functional Adaptor Signature Scheme]
A $\FAS$ scheme is strongly-secure if it is 
advertisement sound, pre-signature valid, witness extractable, $\faSigForge$ secure, pre-signature adaptable and zero-knowledge. 
% \anote{Let's use mathsf for experiment names.}
\label{def:fas-strongly-secure}
\end{definition}



==> fas-from-lattices.tex <==
\ifhldiff
{\color{hldiffcolor}
\fi
\section{$\fas$ from lattices}
\label{sec:fas-from-lattices}

In this section, we provide instantiations of the FAS construction in~\Cref{sec:construction} from lattices.
For this, it suffices to instantiate the building blocks IPFE and AS from lattices, while ensuring the two are compatible with each other. We describe these next.

More specifically, we instantiate the $\as$ as the lattice-based adaptor signature scheme by Esgin et al.~\cite{pq-as}. This scheme was built using cyclotomic ring $\Ring = \Z[x]/(x^d+1)$ of degree $d=256$ under Module-SIS and Module-LWE assumptions. Here, we set the degree to be $d=1$, thus giving us the ring of integers $\mcal{R} = \Z$. Consequently, security follows from plain SIS and LWE assumptions. One can look at the resulting $\as$ to be w.r.t.\ a digital scheme $\Lyu$ that is somewhere in between Lyubashevsky's signature scheme~\cite{lyu12lattice-sig} and Dilithium~\cite{dilithium} instantiated with unstructured lattices. 
% \nikhil{is there a closer match? Lyu12 is over unstructured lattices but uses gaussian sampling. If there is some work that does Lyu12 but does not do gaussian sampling, that would be the closest to our digital signature.}
Further, $\as$ is w.r.t.\ hard relations $R_\isis$ and $R'_\isis$ such that $R_\isis \subset R'_\isis$.

Further, we show that the IND-secure IPFE scheme by Agrawal et al.~\cite[Section 4.2]{ipe01} satisfies $R_\isis$-compliance and $R'_\isis$-robustness when appropriately augmented with a $\PubKGen$ algorithm. 
We describe the instantiations of these two building blocks in the subsequent sections.



		% \nikhil{redo this after stabilizing IPFE construction and correponding AS}
		% \begin{itemize}
		% \item 
		% We build an inner product functional encryption scheme from LWE that is selective, SIM secure and additionally has the two special properties that we need. 
		% The construction is obtained by applying the compiler by Agrawal et al.~\cite{ad-sim-ipfe} (Section 5 of~\cite{ad-sim-ipfe}) to the IPFE scheme by Agrawal et al.~\cite{ad-ind-ipfe} for computing integer inner products of short integer vectors (Section 4.1 of~\cite{ad-ind-ipfe}). The compiler works here because we only aim for selective, SIM security and not adaptive, SIM security. We augment this construction with the additional algorithm $\PubKGen$. Once this is specified, we obtain the relation $R_\isis$ that the functinoal public and secret keys readily satisify. Next, based on the choice of the adaptor signature construction described below, we obtain the extended relation $R'_\isis$ such that $R_\isis \subset R'_\isis$. The second special property of IPFE requires that correctness holds even w.r.t.\ a functional secret key satisfying $R'_\isis$. This property is not readily satisfied by the construction and we need to set some of the parameters \nikhil{make this specific} more restrictively in order for it to also satisfy this. 

		% \item 
		% We build an adaptor signature construction w.r.t. Lyubashevsky's~\cite{lyu09lattice-sig,lyu12lattice-sig} digital siganture scheme $\Lyu$ \nikhil{clarify which of the two} and hard relations $R_\rsis$ and $R'_\rsis$. Our construction is secure in the random oracle model and under the Ring-SIS ($\rsis$) and Ring-LWE ($\rlwe$) assumptions. Esgin et al.~\cite{pq-as} constructed adaptor signatures from Module-SIS and Module-LWE assumptions. Their construction has module rank $4$. Our construction can be seen as their construction but with module rank $1$.
		% \end{itemize}


% \nikhil{describe TrapdoorGen}









\smallskip\noindent\textbf{IPFE from lattices.}
\label{sec:ipfe-lwe}
We first recall the IPFE scheme by Agrawal et al.~\cite{ipe01}. Then, we show that it satisfies the additional compliance and robustness properties needed by our FAS construction.

Suppose $p$ is a 
% $\secparam$-bit 
prime number and suppose we want to compute inner products of vectors of length $\ell$.
Let the set of messages be $\mcal{M} = \Z_p^\ell$ and 
the function class be $\mcal{F}_{{\sf IP}, \ell, p} = \{ f_\bfy : \bfy \in \Z_p^\ell\}$, where $f_\bfy: \Z_p^\ell \to \Z_p$ is defined as $f_\bfy(\bfx) = \bfx^T \bfy \bmod{p}$.
Our IPFE scheme augmented with $\PubKGen$ algorithm is as in~\Cref{fig:ipfe-als}.

\begin{remark}
\label{remark:linear-independence}
\ifcameraready
We note that the original construction requires $\KGen$ to be stateful to support key generation queries that are linearly dependent modulo $p$, which is problematic since $\PubKGen$ would also need to be stateful, undermining the algorithm's public nature. To address this, we assume that all $\KGen$ queries to $\ipfe$ are linearly independent. While this restriction is acceptable for a single buyer, it limits support for multiple buyers. 
\ifcameraready
In the full version,
\else
In~\Cref{sec:fas-from-lattices-modified},
\fi 
we show how to assign unique IDs to each buyer and make the underlying $\ipfe$ key generation queries linearly independent.
\else
We note that the original construction needs $\KGen$ to be stateful in order to support key generation queries that are linearly dependent modulo $p$. This is problematic for us as the corresponding $\PubKGen$ will also have to be stateful then, but that defeats the purpose of this algorithm being public. So, in order to remedy the situation, we assume that all $\KGen$ queries to $\ipfe$ are going to be linearly independent. 
Naively instantiating our $\fas$ construction (\Cref{fig:fas-construction}) will result in $\fas$ only supporting linearly independent functions, which is acceptable if it involves a single buyer but in the most general case we would want to support multiple buyers who are agnostic of each other. Specifically, a buyer may engage in $\fas$ protocol to learn a function evaluation of the secret that is linearly dependent on something learnt by other some other buyers. To handle such a scenario, we show 
\ifcameraready
in the full version
\else 
in~\Cref{sec:fas-from-lattices-modified}
\fi
how to assign unique IDs to each buyer and make the underlying $\ipfe$ key generation queries linearly independent.
\fi
\end{remark}

\begin{figure}[t]
\ifhldiff
{\color{hldiffcolor}
\fi
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed]

\procedure[linenumbering, mode=text]{$\ipfe.\Gen(1^\secparam, p)$}{
Let $n=\secparam$, 
integers $m, k$, real $\alpha \in (0,1)$ as explained below
\\ 
Let $q = p^k$,
\ret $\pp = (n, m, p, q, k, \alpha)$
}

\procedure[linenumbering, mode=text]{$\ipfe.\Setup(\pp, 1^\ell)$}{
Sample $\bfA \getr \Z_q^{m \times n}$, $\bfZ \gets \tau$ where
\pcskipln \\ 
distribution $\tau$ over $\Z^{\ell \times m}$ is as explained below
\\ 
Let $\bfU := \bfZ \bfA  \in \Z_q^{\ell \times n}$,
\ret $\mpk := (\bfA, \bfU), \msk := \bfZ$
}

\procedure[linenumbering, mode=text]{$\ipfe.\Enc(\mpk, \bfx \in \Z_p^\ell)$}{
Sample $\bfs \getr \Z_q^n$, $\bfe_0 \gets D_{\Z, \alpha q}^m$, $\bfe_1 \gets D_{\Z, \alpha q}^\ell$ 
\\ 
Let $\ct_0 := \bfA \bfs + \bfe_0 \in \Z_q^m$,
$\ct_1 := \bfU \bfs + \bfe_1 + p^{k-1} \bfx \in \Z_q^\ell$
\\ 
\ret $\ct := (\ct_0, \ct_1)$
}

\begin{pchstack}
\procedure[linenumbering, mode=text]{$\ipfe.\KGen(\msk, \bfy \in \Z_p^\ell)$}{
\ret $\sk_\bfy := \bfZ^T \bfy \in \Z^m$
% Let internal state be $\state = \{ (\bfy_i, \overline{\bfy}_i, \sk_{\bfy_i}, pk_{\bfy_i})\}$
% \\ 
% If $\bfy$ is linearly independent of $\bfy_i$'s modulo $p$, 
% \pcskipln \\ 
% set $\overline{\bfy} := \bfy \in \Z^\ell$, $\sk_\bfy := \bfZ^T \overline{\bfy} \in \Z^m$, add $(\bfy, \overline{\bfy}, \sk_\bfy)$ to $\state$
% \\ 
% Else let $\bfy = \sum_i k_i \bfy_i \bmod{p}$ for $k_i$'s in $[0, p)$, 
% \pcskipln \\ 
% set $\overline{\bfy} := \sum_i k_i \overline{\bfy}_i \in \Z^\ell$, 
% $\sk_\bfy := \sum_i k_i \bfz_i \in \Z^m$
% \\ 
% \ret $(\overline{\bfy}, \sk_\bfy)$
}

\procedure[linenumbering, mode=text]{$\ipfe.\PubKGen(\mpk, \bfy \in \Z_p^\ell)$}{
\ret $\pk_\bfy := \bfU^T \bfy \in \Z_q^n$
}
\end{pchstack}

\procedure[linenumbering, mode=text]{$\ipfe.\Dec(\sk_\bfy, \ct)$}{
Let $d := \ct_1^T\bfy - \ct_0^T \sk_\bfy \bmod{q}$
\\
\ret $v \in \Z_p$ that minimizes $\mid p^{k-1} v - d \mid$
% \pcskipln \\ \nikhil{specify rounding how}
}

\end{pcvstack}
\caption{
\ifhldiff
{\color{hldiffcolor}
\fi
Agrawal et al.~\cite{ipe01} IPFE scheme augmented with $\PubKGen$ algorithm. Note that $\KGen$ here is stateless.
\ifhldiff
}
\fi
}
\label{fig:ipfe-als}
\ifhldiff
}
\fi
\end{figure}

\noindent\textbf{Parameter choices.}
Let $B_\tau$ be such that with probability at most $n^{-\omega(1)}$, each row of sample from $\tau$ has $\ell_2$-norm at least $B_\tau$. Then, the parameter constraints for correctness and security are as follows.
\begin{itemize}[leftmargin=*]
\item 
$\alpha^{-1} \geq \ell^2 p^3 B_\tau \omega(\sqrt{\log n})$, 
% \item 
$q \geq \alpha^{-1} \omega(\sqrt{\log n})$,
\item 
$ \tau = D^{\ell \times m/2}_{\Z,\sigma_1} \times (D_{\Z^{m/2},\sigma_2, \delta_1} \times \ldots \times D_{\Z^{m/2},\sigma_2, \delta_\ell})$, where $\delta_i \in Z^\ell$ denotes the $i$-th canonical vector, and the
standard deviation parameters satisfy $\sigma_1 = \Theta(\sqrt{n \log m} \max(\sqrt{m}, K'))$ and $\sigma_2 = \Theta(n^{7/2} m{1/2} \max(m, K'^2) \log^{5/2} m)$, with $K' = (\sqrt{\ell}p)^\ell$.
% \item 
% To ensure security based on LWEq,α0,m in dimension ≥ c · n for some c ∈ (0, 1) via Theorems 2 and 4 below, one may further impose that ` ≤ (1 c) · n and m = Θ(n log q), to obtain α0 = Ω(α/(n6K0 log2 q log5/2 n)).
\end{itemize}
Further, $R'_\isis$-robustness (~\Cref{lemma:ipfe-als-robust}) will require the constraint $\alpha^{-1} \geq 4p \omega(\sqrt{\log n}) (\ell p + m \beta_1)$, where $\beta_1$ is as chosen below.

\begin{lemma}[~\cite{ipe01}]
\label{lemma:ipfe-als-secure}
Suppose $\ell \leq n^{O(1)}$, $m \geq 4n \log_2(q)$ and $q, \alpha, \tau$ are as described above.
Suppose $\mheLWE_{q,\alpha,m,\ell,\tau}$ 
\ifcameraready
assumption 
\else
assumption (\Cref{def:mhe-lwe}) 
\fi
holds.
Then, the IPFE scheme in~\Cref{fig:ipfe-als} is selective, 
\ifcameraready
IND-secure.
\else
IND-secure (\Cref{def:ipfe-sel-ind-sec}).
\fi
\end{lemma}
% \textcolor{orange}{Aravind: Proof or citation for this lemma?}

Next, we show the IPFE scheme augmented with the above $\PubKGen$ algorithm satisfies $R_\isis$-compliance and $R'_\isis$-robustness, 
where $R_\isis = \isis_{n, m, q, \beta_0}$ and $R'_\isis = \isis_{n, m, q, \beta_1}$, where $\beta_0 = \ell p B_\tau$ and $\beta_1 = 2(\gamma - \kappa) - \beta_0$ s.t. $\beta_1 > \beta_0$ and $\gamma - \kappa - \beta_0 > 0$. 
% \nikhil{review $\beta_0$ and $\beta_1$ bounds after stabilizing IPFE and AS}

\begin{lemma}
\label{lemma:ipfe-als-compliant}
The IPFE scheme in~\Cref{fig:ipfe-als} is $R_\isis$-compliant, 
where $R_\isis = \isis_{n, m, q, \beta_0}$ and $\beta_0 = \ell p B_\tau$.
\end{lemma}
\begin{proof}
For any $\secparam \in \N$,
for any $\pp \gets \ipe.\Gen(1^\secparam)$ as implemented in~\Cref{fig:ipfe-als},
for any $(\mpk, \msk) \gets \ipe.\Setup(\pp, 1^\ell)$ as implemented in~\Cref{fig:ipfe-als}, 
for any $\bfy \in \mcal{F}_{{\sf IP}, \ell, p}$,
let $\pk_\bfy := \PubKGen(\allowbreak \mpk, \bfy)$ as implemented in~\Cref{fig:ipfe-als}, and 
$\sk_\bfy := \KGen(\msk, \bfy)$ as implemented in~\Cref{fig:ipfe-als}. 
Suppose here $\mpk = (\bfA, \bfU)$ and $\msk = \bfZ$. 
Then, $\sk_\bfy = \bfZ^T\bfy \in \Z^m$ and $\pk_\bfy = \bfU^T \bfy \bmod{q} = \bfA^T \sk_\bfy \bmod{q}$.
Further, note that $||\sk_\bfy||_\infty \leq \ell \cdot ||\bfZ||_\infty \cdot ||\bfy||_\infty  \leq \ell \cdot ||\bfZ||_2 \cdot ||\bfy||_\infty \leq \ell \cdot B_\tau \cdot p = \beta_0$. Hence, $(\pk_\bfy, \sk_\bfy) \in R_\isis$.
\end{proof}

\begin{lemma}
\label{lemma:ipfe-als-robust}
If $\alpha^{-1} \geq 4p \omega(\sqrt{\log n}) (\ell p + m \beta_1)$, then, 
the IPFE scheme in~\Cref{fig:ipfe-als} is $R'_\isis$-robust,
where $R'_\isis = \isis_{n, m, q, \beta_1}$ and $\beta_1 = 2 (\gamma - \kappa)-\beta_0$ such that $\beta_1>\beta_0$.
% \nikhil{fix $\beta_1$.}
\end{lemma}

\begin{proof}
For any $\secparam \in \N$ let $\pp \gets \ipfe.\Gen(1^\secparam)$ 
as implemented in~\Cref{fig:ipfe-als},
for any $\ell \in \N$, 
$\bfx \in \Z_p^\ell, \bfy \in \mcal{F}_{{\sf IP}, \ell, p}$, 
let $(\mpk, \msk) \leftarrow  \Setup(\pp, \ell)$
as implemented in~\Cref{fig:ipfe-als},
let $\pk_\bfy = \PubKGen(\msk, \bfy)$
as implemented in~\Cref{fig:ipfe-als},
let $\ct \leftarrow \Enc(\mpk, \bfx)$ 
as implemented in~\Cref{fig:ipfe-als}.
Then, for any 
$\sk'_\bfy$ such that $(\pk_\bfy, \sk'_\bfy) \in R'_\isis$, 
we want that $\Dec(\sk'_\bfy, \ct)$ outputs $\bfx^T\bfy \bmod{q}$.
Observe that the value $d$ computed by $\Dec$ 
implemented in~\Cref{fig:ipfe-als} simplifies to 
$d = p^{k-1} \bfx^T \bfy + (\bfe_1^T \bfy - \bfe_0^T \sk'_\bfy) \bmod{q}$.
% \begin{align*}
% d & := \ct_1^T\bfy - \ct_0^T \sk'_\bfy \bmod{q} \\ 
% & = (\bfU \bfs + \bfe_1 + p^{k-1} \bfx)^T \bfy - (\bfA \bfs + \bfe_0)^T \sk'_\bfy \bmod{q}\\
% % & = (\bfU \bfs + \bfe_1 + p^{k-1} \bfx)^T \bfy - \bfs^T \bfA^T \sk'_\bfy - \bfe_0^T \sk'_\bfy \bmod{q}\\
% % & = (\bfU \bfs + \bfe_1 + p^{k-1} \bfx)^T \bfy - \bfs^T \pk_\bfy - \bfe_0^T \sk'_\bfy \bmod{q}\\
% % & = (\bfU \bfs + \bfe_1 + p^{k-1} \bfx)^T \bfy - \bfs^T \bfU^T \bfy - \bfe_0^T \sk'_\bfy \bmod{q}\\
% & = p^{k-1} \bfx^T \bfy + (\bfe_1^T \bfy - \bfe_0^T \sk'_\bfy) \bmod{q}
% \end{align*}
Observe that 
\begin{align*}
|\bfe_1^T \bfy - \bfe_0^T \sk_\bfy|
% & \leq |\bfe_1^T \bfy| + |\bfe_0^T \sk_\bfy| \\
& \leq \ell p \alpha q \omega(\sqrt{\log n}) + m \alpha q \omega(\sqrt{\log n}) ||\sk'_\bfy||_\infty \\ 
& = \alpha q \omega(\sqrt{\log n}) (\ell p + m \beta_1).
\end{align*}
For decryption correctness to hold, we need that $|\bfe_1^T \bfy - \bfe_0^T \sk_\bfy| \leq q/4p$. Hence it suffices to have $\alpha^{-1} \geq 4p \omega(\sqrt{\log n}) (\ell p + m \beta_1)$.
\end{proof}

% Observe that while computing functional secret key for $\overline{\bfy}$ in $\KGen$ algorithm, it is not necessary that $\overline{\bfy} = \bfy$, but it is the case that $\overline{\bfy} = \bfy \bmod{p}$. Hence, it follows that $\sk_\bfy = \bfZ^T \bfy \bmod{p}$. Recall that $\pk_\bfy = \bfU^T \bfy$. As $\bfU=\bfZ \bfA$, hence, we get that $\pk_\bfy = \bfA^T \sk_\bfy \bmod{p}$.
% \nikhil{but this is not useful as $||\sk_\bfy \bmod{q} ||_\infty$ = p. So, need to consider computations $\bmod{q}$ and there this analysis is not useful. Fix: make $\PubKGen$ stateful as well.}

\ignore{	
		\noindent\textbf{Correctness.}
		Observe that in the $\Dec$ algorithm, $d$ can be written as follows:
		\begin{align*}
		d 
		& = \ct_1^T \bfy - \ct_0^T \sk_\bfy \bmod{q}\\ 
		& = \bfr^T\bfU \bfy + \lfloor q/p \rfloor \bfx^T \bfy - \bfr^T\bfA \bfS\bfy \bmod{q}\\ 
		& = \lfloor q/p \rfloor \bfx^T \bfy + \bfr^T\bfE\bfy \bmod{q}
		\end{align*}
		Therefore, for the correctness to hold, 
		we need that $||\bfr^T\bfE\bfy ||_\infty < \lfloor q/2p \rfloor$, or equivalently $m \ell B(\sigma \sqrt{\secparam}) < \lfloor q/2p \rfloor$.




		\begin{lemma}
		The above IPFE construction is selective, SIM-secure with proper choice of parameters and under the $\lwe$ assumption.
		\label{lemma:ipfe-lwe-sim}
		\end{lemma}
		\begin{proof}
		We describe the IPFE simulator $\Sim = (\Setup^*, \Enc^*, \KGen^*)$ first.

		\begin{figure}[t]
		\centering
		\captionsetup{justification=centering}
		\begin{pcvstack}[boxed, space=1em]

		\procedure[linenumbering, mode=text]{$\Setup^*(\pp)$}{
		Sample $(\bfA, \bfT_\bfA) \gets \TrapdoorGen(1^m, 1^n)$
		\\
		Sample $\bfS \getr \Z_q^{n \times \ell}$, $\bfE \gets \D_{\Z_q, \sigma, 0}^{m \times \ell}$
		\\ 
		Compute $\bfU = \bfA \bfS + \bfE\bmod{q} \in \Z_q^{m \times \ell}$
		\\ 
		Sample $\bfc_0 \getr \Z_q^n$
		\\ 
		Sample $\bfa^\bot \in \Z_q^n$ using $\bfT_\bfA$ such that $\bfA \bfa^\bot = \bfnum{0} \bmod{q}$ 
		\pcskipln \\ and $\bfc_0^T\bfa^\bot = 1 \bmod{q}$.
		\\
		\ret $\mpk^* = (\bfA, \bfU), \msk^* = (\bfS, \bfE, \bfc_0, \bfa^\bot)$
		}

		\procedure[linenumbering, mode=text]{$\Enc^*(\mpk^*, \msk^*)$}{
		Sample $\bfr \getr \{0,1\}^m$ 
		\\ 
		Compute $\ct_0 = \bfc_0 \in \Z_q^n$
		\\ 
		Compute $\ct_1 = \bfS^T\ct_0 + \bfE^T\bfr \bmod{q} \in \Z_q^\ell$
		\\ 
		\ret $\ct = (\ct_0, \ct_1)$
		}

		\procedure[linenumbering, mode=text]{$\KGen^*(\msk, \bfy \in \mcal{M}, z)$}{
		\ret $\sk^*_\bfy = \bfS \bfy - \bfa^\bot \lfloor q/p \rfloor z \bmod{q} \in \Z_q^n$
		}

		\end{pcvstack}
		\caption{IPFE simulator $\Sim$}
		\label{fig:ipfe-als-simulator}
		\end{figure}

		\noindent\textbf{Decryption correctness.}
		First observe that in $\Dec(\sk^*_\bfy, \ct)$, $d$ can be written as follows:
		\begin{align*}
		d 
		& = {\ct_1}^T \bfy - {\ct_0}^T \sk^*_\bfy \bmod{q}\\ 
		& = \bfc_0^T \bfS \bfy + \bfr^T\bfE \bfy - \bfc_0^T \bfS \bfy + \bfc_0^T \bfa^\bot \lfloor q/p \rfloor z \bmod{q}\\ 
		& = \bfr^T\bfE \bfy + \lfloor q/p \rfloor z \bmod{q}\\ 
		\end{align*}
		Here, the last equality follows from the fact that $\bfc_0^T\bfa^\bot = 1 \bmod{q}$.

		\noindent\textbf{Relation between $\pk_\bfy$ and $\sk^*_\bfy$.}
		Note that the adversary can always compute $\pk_\bfy = \bfU\bfy$ on its own, hence, $\sk^*_\bfy$ must satisfy $\bfA \sk^*_\bfy + \bfE\bfy = \pk_\bfy \bmod{q}$.
		One can observe that $\sk^*_\bfy$ satisfies this relation as $\bfA \sk^*_\bfy = \bfA \bfS \bfy - \bfA \bfa^\bot \lfloor q/p \rfloor z = \bfA \bfS \bfy$, where the last equality is due to the fact that $\bfA \bfa^\bot = \bfnum{0} \bmod{q}$.

		Having described the simulator $\Sim$, experiments $\ipfeSimReal$ and $\ipfeSimIdeal$ are as follows.

		\begin{figure*}[t]
		\centering
		\captionsetup{justification=centering}
		\begin{pchstack}[boxed, space=1em]
		\begin{pcvstack}
		\procedure[linenumbering, mode=text]{Experiments $\ipfeSimReal(1^\secparam, 1^\ell, B)$, \pcbox{\ipfeSimIdeal(1^\secparam, 1^\ell, B)}.}{
		$\pp \gets \Gen(1^\secparam)$
		\\ 
		$\bfx \gets \A(\pp)$
		\\ 
		$\bfA \getr \Z_q^{m \times n}$ 
		\pcbox{\text{
		$(\bfA, \bfT_\bfA) \gets \TrapdoorGen(1^m, 1^n)$
		}}
		\\ 
		$\bfS \getr \Z_q^{n \times \ell}$ 
		\\ 
		$\bfE \gets \D_{\Z_q, \sigma, 0}^{m \times \ell}$
		\\ 
		$\bfU := \bfA \bfS + \bfE\bmod{q}$
		\\ 
		\pcbox{\text{
		$\bfc_0 \getr \Z_q^n$
		}}
		\\ 
		\pcbox{\text{
		Sample $\bfa^\bot \in \Z_q^n$ using $\bfT_\bfA$ s.t.\ $\bfA \bfa^\bot = \bfnum{0} \bmod{q}$, $\bfc_0^T\bfa^\bot = 1 \bmod{q}$
		}}
		\\
		$\mpk := (\bfA, \bfU)$
		\\ 
		% $\msk := \bfS$
		% \pcbox{\text{
		% $\msk := (\bfS, \bfE, \bfc_0, \bfa^\bot)$	
		% }}
		% \\ 
		$\bfr \getr \{0,1\}^m$ 
		\\ 
		$\ct_0 := \bfA^T \bfr \bmod{q}$
		\pcbox{\text{
		$\ct_0 := \bfc_0 $
		}}
		\\ 
		$\ct_1 := \bfU^T \bfr + \lfloor q/p \rfloor \bfx \bmod{q}$
		\pcbox{\text{
		$\ct_1 := \bfS^T\ct_0 + \bfE^T\bfr \bmod{q} $
		}}
		\\ 
		$\ct := (\ct_0, \ct_1)$
		\\ 
		$b \gets \A^{\mcal{O}_\KGen(\cdot)}(\mpk, \ct)$ 
		\pcbox{\text{
		$b \gets \A^{\mcal{O}_\KGen^*(\cdot, \cdot)}(\mpk, \ct)$
		}}
		\\ 
		\ret the bit $b \in \{0,1\}$
		}
		\procedure[linenumbering, mode=text]{Oracles $\mcal{O}_\KGen(\bfy)$, \pcbox{\text{$\mcal{O}_\KGen^*(\bfy, z)$}}.}{
		\ret $\sk_\bfy := \bfS \bfy \bmod{q}$
		\pcbox{\text{
		\ret $\sk^*_\bfy := \bfS \bfy - \bfa^\bot \lfloor q/p \rfloor z \bmod{q}$
		}}
		}
		\end{pcvstack}

		\end{pchstack}
		\caption{Selective, SIM-security experiments of Inner Product Functional Encryption
		% \pnote{To be consistent with the literature, I would just call it WI and WH instead of WitInd and WitHid.}
		% \nikhil{done}
		}
		\label{fig:ipfe-sel-sim-end-games}
		\end{figure*}

		To show that \[
		|
		\Pr[\ipfeSimReal(1^\secparam, n) = 1]
		- \Pr[\ipfeSimIdeal(1^\secparam, n) = 1]
		| \leq \negl(\secparam),
		\]
		we consider a sequence of hybrid experiments $G_0, \ldots, G_8$ where $G_0$ is the experiment $\ipfeSimReal$ and $G_8$ is the experiment $\ipfeSimIdeal$.
		The hybrid experiments are as follows:

		\begin{figure*}[t]
		\centering
		\captionsetup{justification=centering}
		\begin{pchstack}[boxed, space=1em]
		\begin{pcvstack}
		\procedure[linenumbering, mode=text]{Experiments $G_0$, 
		{ \color{violet} \pcbox{ \color{black} \text{
		$G_1$
		}}},
		{ \color{blue} \pcbox{ \color{black} \text{
		$G_2$
		}}},
		{ \color{green} \pcbox{ \color{black} \text{
		$G_3$
		}}},
		{ \color{yellow} \pcbox{ \color{black} \text{
		$G_4$
		}}},
		{ \color{orange} \pcbox{ \color{black} \text{
		$G_5$
		}}},
		{ \color{red} \pcbox{ \color{black} \text{
		$G_6$
		}}},
		{ \color{gray} \pcbox{ \color{black} \text{
		$G_7$
		}}},
		\pcbox{\text{
		$G_8$
		}}
		.}{
		$\pp \gets \Gen(1^\secparam)$
		\\ 
		$\bfx \gets \A(\pp)$
		\\ 
		$\bfA \getr \Z_q^{m \times n}$ 
		\pcbox{\text{
		{ \color{violet} \pcbox{ \color{black} \text{
		$(\bfA, \bfT_\bfA) \gets \TrapdoorGen(1^m, 1^n)$
		}}}
		$\ldots$
		}}
		\\ 
		$\bfS \getr \Z_q^{n \times \ell}$ 
		\\ 
		$\bfE \gets \D_{\Z_q, \sigma, 0}^{m \times \ell}$
		\\ 
		$\bfU := \bfA \bfS + \bfE\bmod{q}$
		{ \color{orange} \pcbox{ \color{black} \text{
		{ \color{yellow} \pcbox{ \color{black} \text{
		$\bfU \getr \Z_q^{m \times \ell}$
		}}}
		}}}
		\\ 
		\pcbox{\text{
		{ \color{orange} \pcbox{ \color{black} \text{
		$\bfc_0 \getr \Z_q^n$
		}}}
		$\ldots$
		}}
		\\ 
		\pcbox{\text{
		Sample $\bfa^\bot \in \Z_q^n$ using $\bfT_\bfA$ s.t.\ $\bfA \bfa^\bot = \bfnum{0} \bmod{q}$, $\bfc_0^T\bfa^\bot = 1 \bmod{q}$
		}}
		\\
		$\mpk := (\bfA, \bfU)$
		% \pcbox{\text{
		% $\mpk := (\bfA, \bfU)$	
		% }}
		\\ 
		% $\msk := \bfS$
		% { \color{yellow} \pcbox{ \color{black} \text{
		% { \color{violet} \pcbox{ \color{black} \text{
		% $\msk := (\bfS, \bfE, \bfT_\bfA)$
		% }}}
		% $\ldots$
		% }}}
		% { \color{red} \pcbox{ \color{black} \text{
		% { \color{orange} \pcbox{ \color{black} \text{
		% $\msk := (\bfS, \bfE, \bfT_\bfA, \bfc_0)$
		% }}}
		% }}}
		% \pcskipln
		% \\
		% { \color{gray} \pcbox{ \color{black} \text{
		% $\msk := (\bfS, \bfE, \bfc_0)$
		% }}}
		% \pcbox{\text{
		% $\msk := (\bfS, \bfE, \bfc_0, \bfa^\bot)$	
		% }}
		% \\ 
		$\bfr \getr \{0,1\}^m$ 
		\\ 
		$\ct_0 := \bfA^T \bfr \bmod{q}$
		\pcbox{\text{
		{ \color{orange} \pcbox{ \color{black} \text{
		$\ct_0 := \bfc_0$
		}}}
		$\ldots$
		}}
		\\ 
		$\ct_1 := \bfU^T \bfr + \lfloor q/p \rfloor \bfx \bmod{q}$
		{ \color{gray} \pcbox{ \color{black} \text{
		{ \color{blue} \pcbox{ \color{black} \text{
		$\ct_1 := \bfS^T\ct_0 + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q}$
		}}}
		}}}
		\pcskipln
		\\
		{ \color{red} \pcbox{ \color{black} \text{
		{ \color{green} \pcbox{ \color{black} \text{
		$\ct_1 := (\bfA^{-1}(\bfU-\bfE))^T\ct_0 + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q}$
		}}}
		$\ldots$
		}}}
		\pcbox{\text{
		$\ct_1 := \bfS^T\ct_0 + \bfE^T\bfr \bmod{q}$
		}}
		\\ 
		$\ct := (\ct_0, \ct_1)$
		\\ 
		$b \gets \A^{\mcal{O}_\KGen(\cdot)}(\mpk, \ct)$ 
		\pcbox{\text{
		$b \gets \A^{\mcal{O}_\KGen^*(\cdot, \cdot)}(\mpk, \ct)$
		}}
		\\ 
		\ret the bit $b \in \{0,1\}$
		}
		\procedure[linenumbering, mode=text]{Oracles $\mcal{O}_\KGen(\bfy)$, \pcbox{\text{$\mcal{O}_\KGen^*(\bfy, z)$}}.}{
		\ret $\sk_\bfy := \bfS \bfy \bmod{q}$
		{ \color{red} \pcbox{ \color{black} \text{
		{ \color{green} \pcbox{ \color{black} \text{
		\ret $\sk_\bfy := \bfA^{-1}(\bfU-\bfE) \bfy \bmod{q}$
		}}}
		$\ldots$
		}}}
		\pcbox{\text{
		\ret $\sk^*_\bfy := \bfS \bfy - \bfa^\bot \lfloor q/p \rfloor z \bmod{q}$
		}}
		}
		\end{pcvstack}

		\end{pchstack}
		\caption{Selective, SIM-security experiments of Inner Product Functional Encryption
		% \pnote{To be consistent with the literature, I would just call it WI and WH instead of WitInd and WitHid.}
		% \nikhil{done}
		}
		\label{fig:ipfe-sel-sim-all-games}
		\end{figure*}

		\noindent\textbf{Game $G_0$.}
		This is the real world game $\ipfeSimReal$.

		\noindent\textbf{Game $G_1$.}
		This is same as $G_0$ except that $\bfA$ is sampled along with its trapdoor $\bfT_\bfA$ using $\TrapdoorGen$. Further, $\msk$ contains $\bfT_\bfA$ as well.
		\nikhil{is this statistically close to $G_0$?}

		\noindent\textbf{Game $G_2$.}
		This is same as $G_1$ except that $\ct_1$ is computed as $\ct_1 := \bfS^T\ct_0 + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q}$. One can observe that $G_1$ and $G_2$ are identically distributed as 
		\begin{align*}
		\ct_1 
		& = \bfS^T\ct_0 + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q} \\
		& = \bfS^T\bfA^T\bfr + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q} \\
		& = \bfU^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q}.
		\end{align*}


		\noindent\textbf{Game $G_3$.}
		This is same as $G_2$ except that $\ct_1$ is computed as 
		$\ct_1 := (\bfA^{-1}(\bfU-\bfE))^T\ct_0 + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q}$
		and for any key generation oracle query $\mcal{O}\KGen(\bfy)$, $\sk_\bfy$ is computed as $\sk_\bfy := \bfA^{-1}(\bfU-\bfE) \bfy \bmod{q}$. One can observe that $G_2$ and $G_3$ are identically distributed as the $\bfA^{-1}(\bfU-\bfE) = \bfA^{-1}(\bfA\bfS) = \bfS$.

		\noindent\textbf{Game $G_4$.}
		This is same as $G_3$ except that $\bfU$ is computed as $\bfU \getr \Z_q^{m \times \ell}$. 
		Observe that under the LWE assumption, $G_3$ and $G_4$ are computationally indistinguishable.
		\nikhil{this argument is problematic. The reduction only obtains $(\bfA, \bfU)$ from the LWE challenger, so it does not know $\bfS$ and $\bfE$. But, simulating $\ct_1$ and $\sk_\bfy$ requires knowledge of $\bfE$. How to resolve this? How does ABDP15 handle this? Also, reduction does not have the choice to set $\bfA$ in trapdoor mode. So, when invoking LWE step, $\bfA$ can't be in trapdoor mode.}

		\noindent\textbf{Game $G_5$.}
		This is same as $G_4$ except that $\ct_0$ is computed as $\ct_0 := \bfc_0 \getr \Z_q^n$. Observe that $G_4$ and $G_5$ are statistically indistinguishable due to the Leftover Hash Lemma.
		\nikhil{this argument is problematic. The reduction obtains $(\bfA, \bfc_0)$ from the LHL challenger where $\bfc_0 = \bfA^T\bfr$ or it is uniformly random. Note that the reduction does not have access to $\bfr$. But, simulating $\ct_1$ requires knowledge of $\bfr$. How to resolve this? I think this is fixable. First switch $\bfc_0 = \bfA^T\bfr$ and $\bfc_1 = \bfU^T\bfr$ both to uniformly random via LHL and then, only switch back $\bfc_1$ to $\bfU^T\bfr$ again via LHL.}

		\noindent\textbf{Game $G_6$.}
		This is same as $G_5$ except that $\bfU$ is switched back to $\bfU := \bfA\bfS+\bfE$.
		Observe that under the LWE assumption, $G_5$ and $G_6$ are computationally indistinguishable.
		\nikhil{this argument is problematic. same issue as $G_3$ to $G_4$.}

		\noindent\textbf{Game $G_7$.}
		This is same as $G_6$ except that $\ct_1$ is switched back to 
		$\ct_1 := \bfS^T\ct_0 + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q}$ 
		and 
		for any key generation oracle query $\mcal{O}\KGen(\bfy)$, $\sk_\bfy$ is switched back to being computed as $\sk_\bfy := \bfS \bfy \bmod{q}$.

		\noindent\textbf{Game $G_8$.}
		This is same as $G_7$ except that the $\ct_1$ is computed as 
		$\ct_1 := \bfS^T\ct_0 + \bfE^T\bfr \bmod{q}$ and the simulator answers $\KGen$ queries for $\bfy$ using the oracle $\mcal{O}^*_\KGen(\bfy, z)$ as 
		$\sk^*_\bfy := \bfS \bfy - \bfa^\bot \lfloor q/p \rfloor z \bmod{q}$, 
		where $\bfa^\bot \in \Z_q^n$ is computed using $\bfT_\bfA$ such that \ $\bfA \bfa^\bot = \bfnum{0} \bmod{q}$, $\bfc_0^T\bfa^\bot = 1 \bmod{q}$.

		Observe that $G_8$ is the ideal world experiment $\ipfeSimIdeal$. We show below that $G_7$ and $G_8$ are identically distributed as going from $G_7$ to $G_8$ essentially involves a change of variable $\bfS \to \bfS - \bfa^\bot \lfloor q/p \rfloor \bfx^T$. As $\bfS$ is uniformly random, hence, the two distributions are identical.

		Making the change of variable in $\ct_1$ in game $G_7$, we get that 
		\begin{align*}
		\ct_1
		& = (\bfS - \bfa^\bot \lfloor q/p \rfloor \bfx^T)^T\ct_0 + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q} \\
		& = \bfS^T\ct_0 - \lfloor q/p \rfloor \bfx {\bfa^\bot}^T \bfc_0  + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q} \\
		& = \bfS^T\ct_0 - \lfloor q/p \rfloor \bfx + \bfE^T\bfr + \lfloor q/p \rfloor \bfx \bmod{q} \\
		& = \bfS^T\ct_0 + \bfE^T\bfr \bmod{q},
		\end{align*}
		where the second last equality is due to the fact that ${\bfa^\bot}^T \bfc_0 = 1 \bmod{q}$. Further, making the change of variable in $\sk_\bfy$ in game $G_7$, we get that 
		\begin{align*}
		\sk_\bfy 
		& = (\bfS - \bfa^\bot \lfloor q/p \rfloor \bfx^T)\bfy \bmod{q}\\ 
		& = \bfS\bfy - \bfa^\bot \lfloor q/p \rfloor \bfx^T\bfy \bmod{q}\\ 
		& = \bfS\bfy - \bfa^\bot \lfloor q/p \rfloor z \bmod{q},
		\end{align*}
		where the last equality is due to the fact that $z = \bfx^T\bfy$.

		This completes the proof.
		\end{proof}

}


\smallskip\noindent\textbf{$\fas$ construction.}
Instantiating $\fas$ in~\Cref{sec:fas-construction} with $\ipfe$ as in~\Cref{fig:ipfe-als} and $\as$ 
\ifcameraready
as in the full version, 
\else
as in~\Cref{fig:lyu-as}, 
\fi
we obtain the following informal corollary. Formal details are deferred
\ifcameraready 
to the full version.
\else
to~\Cref{corollary:fas-strongly-secure-lattices}.
\fi

\begin{corollary}[Informal]
\label{corollary:fas-strongly-secure-lattices-informal}
\label{thm:fas-strongly-secure-lattices-informal}
% Let $p$ be a $\secparam$-bit prime number and let $\ell$ be an integer.
% Let $\mcal{M}=\Z_p^\ell$ be an additive group.
% \nikhil{remove additive group from paper everywhere and keep it to $\Z_p^\ell$ everywhere.}
% Let $\mcal{F}_{{\sf IP}, \ell, p}$ be the function family for computing inner products of vectors in $\Z_p^\ell$. 
% Let $R$ be any NP relation 
% with statement/witness pairs $(X, \bfx)$ such that $\bfx \in \Z_p^\ell$.
% Let $R_\isis = \isis_{n, m, q, \beta_0}$ and $R'_\isis = \isis_{n, m, q, \beta_1}$, where $\beta_0 = \ell p B_\tau$ and $\beta_1 = 2(\gamma - \kappa) - \beta_0$ s.t. $\beta_1 > \beta_0$ and $\gamma - \kappa - \beta_0 > 0$. 
% Suppose that 
% \begin{itemize}
% \item 
% All function queries $\bfy$ to $\AuxGen$ are linearly independent modulo $p$,
% \item
% $R$ is $\mcal{F}_{{\sf IP}, \ell, p}$-hard (\Cref{def:f-hard-relation}),
% \item
% $\nizk$ is a secure NIZK argument system (\Cref{def:nizk}),
% \item
% $\as$ construction in~\Cref{fig:lyu-as} is an adaptor signature scheme w.r.t.\ digital signature scheme $\Lyu$ and hard relations  $R_\isis$ and $R'_\isis$ that satisfies weak pre-signature adaptability (\Cref{def:as-pre-sig-adaptability}) and witness extractability (\Cref{def:as-wit-ext}),
% \item
% $\ipfe$ construction in~\Cref{fig:ipfe-abdp} is a selective, IND-secure IPFE scheme (\Cref{def:ipfe-sel-ind-sec}) for function family $\mcal{F}_{{\sf IP}, \ell+1}$ that is $R_\isis$-compliant (\Cref{def:ipfe-compliant}) and $R'_\isis$-robust (\Cref{def:ipfe-robust}). 
% \end{itemize} 
There exists a functional adaptor signature scheme 
w.r.t.\ Lyubashevsky signature scheme $\Lyu$, NP relation $R$, and family of inner product functions $\mcal{F}_{{\sf IP}, \ell, p}$ that is strongly-secure.
\end{corollary}

The proof of corollary is immediate from that of~\cref{thm:fas-strongly-secure} concerning the generic construction, and~\cref{lemma:ipfe-als-secure,lemma:ipfe-als-compliant,lemma:ipfe-als-robust} that show that the $\ipfe$ scheme in~\Cref{fig:ipfe-als} has the required properties.

% \textcolor{orange}{Informally describe why the theorem holds.}
% \begin{remark}
% Note that the linear independence modulo $p$ restriction for all $\AuxGen$ queries in this lattice-based instantiation comes due to the same restriction on the underlying IPFE scheme as discussed in~\Cref{remark:linear-independence}. In practice,  $\AuxGen$ queries can be sent by any buyer to the seller. On one hand it's reasonable to assume that all the queries by a single buyer are going to be linearly independent modulo $p$ because by linearity of the functionality, the buyer can locally compute the function evaluation for some function $\bfy$ that is linear combination of the functions $\bfy_i$'s it previously queried as follows: if $\bfy = \sum_i k_i \bfy_i \bmod{q}$, then, $f_\bfy(\bfx)$ can be computed as $f_\bfy(\bfx) := \sum_i k_i f_{\bfy_i}(\bfx)$. On the other hand, it's unreasonable to assume that all buyers are working in coordination and make sure that their queries are linearly independent. In~\Cref{sec:fas-from-lattices-modified}, we show how to remove this restriction on FAS.
% \end{remark}

\ifhldiff
}
\fi


==> fas-from-prime-groups.tex <==
\ifhldiff
{\color{hldiffcolor}
\fi
\section{FAS from prime-order groups}
\label{sec:fas-from-prime-groups}\label{sec:detailed_instantiation}


% \ifacm
% We discuss the instantiations of the two building blocks namely $\as$ as Schnorr adaptor signature scheme~\cite{PKC:EFHMR21}, and the selective, IND-secure IPFE scheme by Abdalla et al.~\cite{ipe}. These two are the key components of our FAS instantiation.
% \else
We provide instantiations of the FAS construction in~\Cref{sec:construction} from prime order groups. 
For this, it suffices to instantiate the building blocks $\IPFE$ and $\AS$ from prime order groups, while ensuring the two are compatible with each other. We describe these next.
We can instantiate the $\nizk$ for the language $L_\nizk$ depending on the concrete relation $R$. 
That is, given $R$ and the above instantiation of $\IPFE$, we can pick the most efficient $\nizk$ for $L_\nizk$.
Since this is not the main contribution of this work, we will assume $R$ to be a general NP relation and rely on the existence of $\nizk$ for general NP~\cite{nizk-from-ddh,peikert2019noninteractive} and not delve into its details here.
%The asterisk $^*$ in the section title is to note that $\nizk$ for NP are not known from prime order groups, so we do not specify its details here. As the lattice-based $\nizk$ systems support all NP langauges \pnote{which papers to cite?}, we can use those even for the language $L_\nizk$ related to the prime-order groups that the $\ipfe$ instantiation induces here.

More concretely, we instantiate the $\as$ as Schnorr adaptor signature scheme~\cite{asig} and thus, we have $R_\ipfe = R'_\ipfe = R_\DL$ as defined 
\ifcameraready
in the full version. 
\else
in~\Cref{def:dl-relation}. 
\fi
Further, we show that the selective, IND-secure IPFE scheme by Abdalla et al.~\cite{ipe} satisfies $R_\DL$-compliance and $R_\DL$-robustness when appropriately augmented with a $\PubKGen$ algorithm. 
As the $\as$ scheme is not part of our contributions, we defer its details 
\ifcameraready
to the full version
\else
to~\Cref{sec:schnorr-adaptor} 
\fi
and describe the IPFE scheme here.
% \fi 

%\subsection{Preliminaries}
%\noindent\textbf{Decisional Diffie-Hellman (DDH) assumption.}
%Let $\GroupGen$ be a \ppt algorithm that takes as input a security parameter $1^\secparam$ and outputs a triplet $(\G, p, g)$ where $\G$ is a group of order $p$ that is generated by $g \in \G$, and $p$ is a $\secparam$-bit prime number. Then, the DDH assumption states that the tuples $(g, g^a, g^b, g^{ab})$ and $(g, g^a, g^b, g^c)$ are computationally indistinguishable, where $(\G, p, g)\gets \GroupGen(1^\secparam)$, and $a, b, c \in \Z_p$ are chosen independently and uniformly at random. \anote{Why do we need to recall this assumption here? Remove if space constraint}
%
%\noindent\textbf{Additional notation.}
%For $d \in \G$, we denote the algorithm for computing the discrete log of $d$ with respect to base $g \in \G$ by $\DLog_g(d)$. As long as we are promised that the discrete log is bounded by a polynomial $B$, the $\DLog$ algorithm simply enumerates all the possibilities to find the discrete log. The running time is polynomial because of the bound $B$.



\smallskip\noindent\textbf{IPFE from prime-order groups.}
We first recall the IPFE scheme by Abdalla et al.~\cite{ipe}. Then, we show that it satisfies the additional compliance and robustness properties needed by our FAS scheme.

Suppose $p$ is a $\secparam$-bit prime number and suppose we want to compute inner products of vectors of length $\ell$.
The Abdalla et al.~\cite{ipe} IPFE scheme computes inner products with output values polynomially bounded by $B \ll p$. 
Specifically, the message space is $\mcal{M} = \Z_p^\ell$ and the function class is $\mcal{F}_{{\sf IP}, \ell, p, B} = \{ f_\bfy : \bfy \in \Z_p^\ell\} \subseteq \mcal{F}_{{\sf IP}, \ell}$, where $f_\bfy: \Z_p^\ell \to \{0, \ldots, B\}$ is defined as $f_\bfy(\bfx) = \bfx^T \bfy \in \{0, \ldots, B\}$. 
The scheme by Abdalla et al.\cite{ipe} augmented with $\PubKGen$ algorithm is as in~\Cref{fig:ipfe-abdp}.
For $d \in \G$, we denote the algorithm for computing the discrete log of $d$ with respect to base $g \in \G$ by $\DLog_g(d)$. 
\ifcameraready\else
As long as we are promised that the discrete log is bounded by a polynomial $B$, the $\DLog$ algorithm simply enumerates all the possibilities to find the discrete log. The running time is polynomial because of the bound $B$.
\fi 

\begin{figure}[t]
\ifhldiff
{\color{hldiffcolor}
\fi
\centering
\captionsetup{justification=centering}
\begin{pchstack}[boxed, space=0.5em]
\begin{pcvstack}

\procedure[linenumbering, mode=text]{$\ipfe.\Gen(1^\secparam)$}{
$\pp := (\G, p, g) \gets \GroupGen(1^\secparam)$\\
\ret $\pp$
}

\procedure[linenumbering, mode=text]{$\ipfe.\Setup(\pp, 1^\ell)$}{
$\bfs \getr \Z_p^\ell$, 
\ret $\msk:=\bfs, \mpk:=g^\bfs$
}

\procedure[linenumbering, mode=text]{$\ipfe.\Enc(\mpk, \bfx \in \Z_p^\ell)$}{
$r \getr \Z_p$, $\ct_0 := g^r$, $\ct_1 := g^\bfx \cdot \mpk^r$
\\
\ret $\ct := (\ct_0, \ct_1)$
}

\procedure[linenumbering, mode=text]{$\ipfe.\KGen(\msk, \bfy \in \Z_p^\ell)$}{
\ret $\sk_\bfy := \bfs^T\bfy \in \Z_p$
}

\end{pcvstack}
\begin{pcvstack}

\procedure[linenumbering, mode=text]{$\ipfe.\PubKGen(\mpk, \bfy \in \Z_p^\ell)$}{
Parse $\mpk = (k_1, \ldots, k_\ell)$
\\ 
Parse $\bfy = (y_1, \ldots, y_\ell)$
\\
\ret $\pk_\bfy := \prod_{i \in [\ell]} k_i^{y_i} $
}

\procedure[linenumbering, mode=text]{$\ipfe.\Dec(\sk_\bfy, \ct)$}{
Parse $\ct_1 = (c_1, \ldots, c_\ell)$
\\ 
Parse $\bfy = (y_1, \ldots, y_\ell)$
\\
$d := \prod_{i \in [\ell]} c_i^{y_i} / \ct_0^{\sk_\bfy}$
\\
\ret $v := \DLog_g(d)$
}


\end{pcvstack}
\end{pchstack}

\caption{
\ifhldiff
{\color{hldiffcolor}
\fi
Abdalla et al.~\cite{ipe} IPFE scheme augmented with $\PubKGen$ algorithm
\ifhldiff
}
\fi
}
\label{fig:ipfe-abdp}
\ifhldiff
}
\fi
\end{figure}

\begin{lemma}[\cite{ipe}]\label{lemma:1}
Suppose the DDH assumption holds. 
Then, the IPFE scheme in~\Cref{fig:ipfe-abdp} is selective, 
\ifcameraready
IND-secure.
\else
IND-secure (\Cref{def:ipfe-sel-ind-sec}).
\fi
\end{lemma}


Next, we show the IPFE scheme augmented with the above $\PubKGen$ algorithm satisfies $R_\DL$-compliance and $R_\DL$-robustness. 

\begin{lemma}\label{lemma:2}
The IPFE scheme in~\Cref{fig:ipfe-abdp} is $R_\DL$-compliant.
\end{lemma}
\begin{proof}
For any $\secparam \in \N$,
for any $\pp \gets \ipe.\Gen(1^\secparam)$ as implemented in~\Cref{fig:ipfe-abdp},
for any $(\mpk, \msk) \gets \ipe.\Setup(\pp, 1^\ell)$ as implemented in~\Cref{fig:ipfe-abdp}, 
for any $\bfy \in \mcal{F}_{{\sf IP}, \ell, p, B}$,
let $\pk_\bfy :=  \PubKGen(\allowbreak \mpk, \bfy)$ as implemented in~\Cref{fig:ipfe-abdp}, and 
$\sk_\bfy := \KGen(\msk, \bfy)$ as implemented in~\Cref{fig:ipfe-abdp}. Suppose here $\msk=\bfs \in \Z_p^\ell$. Then, $\sk_\bfy = \bfs^T\bfy \in \Z_p$ and $\pk_\bfy = g^{\bfs^T\bfy} \in \G$. Thus, clearly, $(\pk_\bfy, \sk_\bfy) \in R_\DL$.
\end{proof}

\begin{lemma}\label{lemma:3}
The IPFE scheme in~\Cref{fig:ipfe-abdp} is $R_\DL$-robust.
\end{lemma}
\begin{proof}
Observe that in the IPFE scheme in~\Cref{fig:ipfe-abdp}, the base relation $R$ and the extended relation $R'$ are the same: $R = R'=R_\DL$. Further, $R_\DL$ is a unique witness relation. Thus, $R_\DL$-robustness follows trivially from the correctness of the IPFE scheme.  
\end{proof}



\smallskip\noindent\textbf{$\fas$ construction.}
Instantiating $\fas$ in~\Cref{sec:fas-construction} with $\ipfe$ as in~\Cref{fig:ipfe-abdp} and $\as$ 
\ifcameraready
as in the full version, 
\else
as in~\Cref{sec:schnorr-adaptor}, 
\fi 
we obtain the following informal corollary. Formal details are deferred 
\ifcameraready
to the full version.
\else
to~\Cref{corollary:fas-strongly-secure-prime-order-groups}.
\fi

\begin{corollary}[Informal]
\label{corollary:fas-strongly-secure-prime-order-groups-informal}
\label{thm:fas-strongly-secure-prime-order-groups-informal}
% Let $p$ be a $\secparam$-bit prime number and let $\ell$ be an integer.
% Let $\mcal{M}=\Z_p^\ell$ be an additive group.
% let $\mcal{F}_{\sf{IP}, \ell, p, B}$ be the function family for computing inner products of vectors in $\Z_p^\ell$ such that the output value is bounded by some polynomial $B \ll p$. 
% Let $R$ be any NP relation 
% with statement/witness pairs $(X, \bfx)$ such that $\bfx \in \Z_p^\ell$.
% Suppose that 
% \begin{itemize}[leftmargin=*]
% \item
% $R$ is $\mcal{F}_{{\sf IP}, \ell, p, B}$-hard (\Cref{def:f-hard-relation}),
% \item
% $\nizk$ is a secure NIZK argument system (\Cref{def:nizk}),
% \item
% $\as$ construction in~\Cref{sec:schnorr-adaptor} is an adaptor signature scheme w.r.t.\ digital signature scheme $\Sch$ and hard relation $R_\DL$ that satisfies weak pre-signature adaptability (\Cref{def:as-pre-sig-adaptability}) and witness extractability (\Cref{def:as-wit-ext}),
% \item
% $\ipfe$ construction in~\Cref{fig:ipfe-abdp} is a selective, IND-secure IPFE scheme (\Cref{def:ipfe-sel-ind-sec}) for function family $\mcal{F}_{{\sf IP}, \ell+1}$ that is $R_\ipe$-compliant (\Cref{def:ipfe-compliant}). 
% \end{itemize} 
There exists a functional adaptor signature scheme 
w.r.t.\ Schnorr signature scheme $\Sch$, NP relation $R$, and family of inner product functions $\mcal{F}_{{\sf IP}, \ell, p, B}$ that is strongly-secure.
\end{corollary}

The proof of the corollary is immediate from that of~\cref{thm:fas-strongly-secure} concerning the generic construction, and~\cref{lemma:1,lemma:2,lemma:3} that show that the $\ipfe$ scheme in~\Cref{fig:ipfe-abdp} has the required properties.



% \nikhil{move this to DL based instantiation section later}
% The IPFE scheme by Abdalla et al.~\cite{ipe} based on the DDH assumption satisfies our requirements. Specifically, in their construction, $\msk := \bfs \getr \Z_p^\ell$, $\mpk := g^\bfs$, and $\sk_\bfy := \bfs^T \bfy$. Then, given $\mpk$ and $\bfy$, we can efficiently compute $\pk_\bfy := g^{ \bfs^T \bfy} := \Pi_{i \in [m]} (g^{s_i})^{y_i}$. This choice meets our requirements that $(\mpk, \msk) \in R_{DL}$ and for any $\bfy$, $(\pk_\bfy, \sk_\bfy) \in R_{DL}$. \anote{where do we define $R_{DL}$}
\ifhldiff
}
\fi


==> fas-from-structured-lattices.tex <==
\section{$\fas$ from structured lattices}

In this section, we provide instantiations of the functional adaptor signature construction in~\Cref{sec:construction} from structured lattices.
For this, it suffices to instantiate the building blocks IPFE and AS from structured lattices, while ensuring the two are compatible with each other. We describe an overview of these instantiations below.

\begin{itemize}
\item 
We build an inner product functional encryption scheme from Ring-LWE that is secure and additionally has the two special properties that we need. The construction is essentially the same as the one by Mera et al.~\cite{ipfe-rlwe}. We augment the construction with the additional algorithm $\PubKGen$. Once this is specified, we obtain the relation $R_\rsis$ that the functinoal public and secret keys readily satisify. Next, based on the choice of the adaptor signature construction described below, we obtain the extended relation $R'_\rsis$ such that $R_\rsis \subset R'_\rsis$. The second special property of IPFE requires that correctness holds even w.r.t.\ a functional secret key satisfying $R'_\rsis$. This property is not readily satisfied by~\cite{ipfe-rlwe} and we need to set some of the parameters \nikhil{make this specific} more restrictively in order for it to also satisfy this. 

\item 
We build an adaptor signature construction w.r.t. Lyubashevsky's~\cite{lyu09lattice-sig,lyu12lattice-sig} digital siganture scheme $\ds$ \nikhil{clarify which of the two} and hard relations $R_\rsis$ and $R'_\rsis$. Our construction is secure in the random oracle model and under the Ring-SIS ($\rsis$) and Ring-LWE ($\rlwe$) assumptions. Esgin et al.~\cite{pq-as} constructed adaptor signatures from Module-SIS and Module-LWE assumptions. Their construction has module rank $4$. Our construction can be seen as their construction but with module rank $1$.
\end{itemize}

The security assumptins on which our constructions rely are the two well-known lattice problems \rsis and \rlwe \nikhil{add cites}.
As in \nikhil{add cites}, we define below \rsis in the ``Hermite normal form'', which is as hard as \rsis with a completely random vector $\bfa$ \nikhil{double check this claim}.

\subsection{Preliminaries}
We define $\Ring_q = \Z_q[X]/(X^n + 1)$ to be cyclotomic ring of power-of-2 degree $n$ for an odd modulus $q$. 
Let $1_\Ring$ be the identity element of the ring $\Ring_q$.
We denote by $\S_c$ the set of polynomials in $\Ring_q$ whose maximum absolute coefficient is at most $c \in \Z^+$. 
Similarly, $\Ring = \Z[X]/(X^n+1)$. 
For a polynomial $f = f_0 + f_1 X + \ldots + f_{n-1} X^{n-1} \in \Ring$, we define the norms in the typical way: 
$||f|| = \sqrt{\sum_{i=0}^{n-1} f_i^2}$, 
$||f||_\infty = \max_i |f_i|$ and 
$||f||_1 = \sum_{i=0}^{n-1} |f_i|$. 
For a vector $\bfv = (v_0, \ldots, v_{s-1}) \in \Ring^s$ of polynomials with $s \geq 1$, 
we further define 
$||\bfv|| = \sqrt{\sum_{i=0}^{s-1} ||v_i||^2}$, 
$||\bfv||_\infty = \max_i ||\bfv_i||_\infty$ and 
$||\bfv||_1 = \sum_{i=0}^{s-1} ||v_i||_1$. 
$I_n$ denotes the identity matrix of dimension $n \times n$.

\begin{definition}[$\rsis_{m,q,\beta}$]
Let $\bfa' \getr \Ring_q^{m-1}$ and $\bfa = (1 || {\bfa'}^T)^T$.
Given $\bfa$, \rsis problem with parameter $m>1$ and $0 < \beta < q$ asks to find a short non-zero $\bfv \in \Ring^m$ such that $\bfa^T \bfv = \sum_{i=1}^{m} a_i \cdot v_i = 0$ over $\Ring_q$ and $||\bfv||_\infty \leq \beta$.
\end{definition}

\begin{definition}[$\rlwe_{m,q, \Psi}$]
\rlwe problem with parameter $m>0$ and distribution $\Psi$ over $\Ring$ asks to distinguish between the following two cases: 1) $(\bfa, \bfb) \getr \Ring_q^m \times \Ring_q^m$, and 2) $(\bfa, \bfa s + \bfe)$ for $\bfa \getr \Ring_q^m$, a secret $s \gets \Psi$ and an error vector $\bfe \gets \Psi^m$.
\end{definition}

\begin{definition}[$\rpsis_{m, q, \beta}$]
It is the planted version of \rsis. 
Specifically, let $\bfa' \getr \Ring_q^{m-1}$ and $\bfa = (1 || {\bfa'}^T)^T$. Let $\bfu \getr \Ring^m$ s.t. $||\bfu||_\infty \leq \beta$. Let $b = \bfa^T\bfu$ over $\Ring_q$. Given $(\bfa, b)$, the problem with parameters $1 < m \ll \frac{\log{q}}{\log{\beta}}$ \nikhil{check this for unique solution} and $0 < \beta < q$ asks to find a short non-zero $\bfv \in \Ring^m$ such that $\bfa^T \bfv = b$ over $\Ring_q$ and $||\bfv||_\infty \leq \beta$. 
\end{definition}

In the $\rpsis_{m, q, \beta}$ problem, the bound on $m$ ensures that it is very likely that the problem has a unique solution.

\begin{definition}[Hard Relation $R_{\rsis}$]
It is the $\rpsis_{m, q, \beta_0}$ relation for some bound $\beta_0$.
\nikhil{define $\beta_0$}
\end{definition}


\begin{definition}[Hard Relation $R'_\rsis$]
It is the extended relation w.r.t.\ $R_\rsis$. Let $R_\rsis = \rpsis_{m,q,\beta_0}$. Then, $R'_\rsis = \rpsis_{m,q,\beta_1}$ for some bound $\beta_1 > \beta_0$.
\nikhil{define $\beta_1$}
\end{definition}

\begin{definition}[Discrete Gaussian distribution]
A discrete gaussian distribution $D_{\Lambda, \sqrt{\Sigma}, \bfc}$, for $\bfc \in \R^n$, $\Sigma$ a positive semi-definite matrix in $\R^{n \times n}$, and a lattice $\Lambda \subset \Z^n$, is a distribution with values in $\Lambda$ and probabilities
\[
\Pr[X = \bfx] \propto \exp{\left(-\frac12 (\bfx - \bfc)^T\Sigma^+(\bfx-\bfc)\right)}.
\]
\end{definition}
Note that $\Sigma^+$ denotes the pseudoinverse of a matrix. If $\Lambda = \Z^n$, we shall just write $D_{\sqrt{\Sigma}, \bfc}$. Further, if $\bfc = 0$, then we shall just write $D_{\sqrt{\Sigma}}$, and if $\sqrt{\Sigma} = \sigma I_n$ for $\sigma \in \R^+$ and $I_n$ an identity matrix, we shall just write $D_\sigma$.

\subsection{Lattice-based Inner Product Functional Encryption}
\label{sec:ipfe-rlwe}
Let the set of messages be 
$\{\bfx \in \Z^\ell : ||\bfx||_\infty \leq B_x \}$ 
for some bound $B_x$ and 
let the set of functions be 
$\{\bfy \in \Z^\ell : ||\bfy||_\infty \leq B_y \}$ 
for some bound $B_y$.
Let $K$ be greater than the maximal value of the resulting inner product, i.e., $K > \ell B_x B_y$. \nikhil{describe the function class}

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed, space=1em]

\procedure[linenumbering, mode=text]{$\Gen(1^\secparam)$}{
Choose $n$ to be a power-of-2 \nikhil{depends on $\secparam$?}
\\ 
Choose an odd modulus $q$ \nikhil{prime? depends on $\secparam?$}
\\ 
Let $\Ring = \Z[X]/(X^n+1)$, $\Ring_q = \Ring/q\Ring$
\\ 
Choose interger $m$ as described in ??
\\ 
Output $\pp = (q, \Ring, \Ring_q, m)$
}

\procedure[linenumbering, mode=text]{$\Setup(\pp, n)$}{
Sample $\bfa' \getr \Ring_q^m$, let $\bfa = (1||{\bfa'}^T)^T$
% Sample $\bfa  = (a_1, \ldots, a_m)^T \getr \Ring_q^m$
% \\ 
% If no $a_i$ is invertible in $\Ring_q$, resample $\bfa$
\\ 
$\forall i \in [\ell]:$ 
Sample $\bfs \gets D^m_{\sigma_1 I_n}$ over $\Ring^m$
% Let $\bfs_i  = (s_{i,1} , \ldots, s_{i,j})^T \in \Ring^m$, 
% where each $s_{i,j} \in \Ring$ is sampled from $D_{\sigma_1 I_n}$
\\ 
Let $\bfS = (\bfs_1 || \ldots || \bfs_m)^T \in \Ring^{\ell \times m}$
\\ 
Output $\mpk = (\bfa, \bfb = \bfS \bfa), \msk = \bfS$
}

\procedure[linenumbering, mode=text]{$\KGen(\msk, \bfy \in \Z^\ell \ s.t.\ ||\bfy||_\infty \leq B_y)$}{
Output $\sk_\bfy = \bfS^T\bfy = \sum_{i \in [\ell]} \bfs_i y_i \in \Ring^m$
}

\procedure[linenumbering, mode=text]{$\PubKGen(\mpk, \bfy \in \Z^\ell \ s.t.\ ||\bfy||_\infty \leq B_y)$}{
Output $\pk_\bfy = \bfb^T\bfy =  \sum_{i \in [\ell]} b_i y_i\in \Ring$
}

\procedure[linenumbering, mode=text]{$\Enc(\mpk, \bfx \in \Z^\ell \ s.t.\ ||\bfx||_\infty \leq B_x)$}{
Sample $r \gets D_{\sigma_2 I_n}$ over $\Ring_q$
\\ 
Sample $\bfe_0 \gets D^m_{\sigma_2 I_{nm}}$ over $\Ring_q^m$
\\ 
Compute $\ct_0 = \bfa r + \bfe_0$
\\ 
If no element of $\ct_0$ is invertible in $\Ring_q$: resample $r, \bfe_0$
\\ 
Sample $\bfe_1 \gets D^\ell_{\sigma_3 I_{n}}$ over $\Ring_q^\ell$
\\
Compute $\ct_1 = \bfb r + \bfe_1 + \lfloor q/K \rfloor \bfx 1_R$
}

\procedure[linenumbering, mode=text]{$\Dec(\sk_\bfy, \ct)$}{
Compute $d = \ct_1^T\bfy - \ct_0^T \sk_\bfy$
\\
Output $v = {\sf Round}(d)$ \nikhil{specify rounding how}
}

\end{pcvstack}
\caption{Construction: IPFE from \rlwe}
\label{fig:ipfe-rlwe}
\end{figure}

\paragraph{Correctness.}
Observe that in the $\Dec$ algorithm, $d$ can be written as follows:
\begin{align*}
d 
& = \ct_1^T \bfy - \ct_0^T \sk_\bfy \\ 
& = ( \bfb r + \bfe_1 + \lfloor q/K \rfloor \bfx 1_R)^T \bfy - (\bfa r + \bfe_0)^T \sk_\bfy \\
& = \lfloor q/K \rfloor (\bfx^T\bfy) 1_R + (\bfe_1^T\bfy - \bfe_0^T \sk_\bfy) + r(\bfb^T \bfy - \bfa^T \sk_\bfy) \\
& = \lfloor q/K \rfloor (\bfx^T\bfy) 1_R + (\bfe_1^T\bfy - \bfe_0^T \sk_\bfy) + r(\pk_\bfy - \bfa^T \sk_\bfy) \\
& = \lfloor q/K \rfloor (\bfx^T\bfy) 1_R + (\bfe_1^T\bfy - \bfe_0^T \sk_\bfy)
\end{align*}
As $\sk_\bfy$ is honestly generated, hence $\sk_\bfy = \bfS^T\bfy$.
Therefore, for the correctness to hold, 
we need that $||(\bfe_1 - \bfS \bfe_0)^T\bfy ||_\infty < \lfloor q/2K \rfloor$, or equivalently $\ell B_y (\sigma_3 \sqrt{\secparam} + mn \sigma_1 \sigma_2 \secparam) < \lfloor q/2K \rfloor$.

\paragraph{Additional special properties.}
We show that the above construction satisfies the two additional special properties we need of an IPFE scheme.
\begin{itemize}
\item 
{\bf Functional public and secret keys satisfy the hard relation $R_\rsis$.}
Note that for any function $\bfy$ s.t. $||\bfy||_\infty \leq B_y$, we have that $\sk_\bfy = \bfS^T \bfy$ and $\pk_\bfy = \bfb^T\bfy = \bfa^T \bfS^T \bfy = \bfa^T \sk_\bfy$, where each entry of matrix $\bfS$ comes from distribution $D_{\sigma_1 I_n}$ over $\Ring$. Hence, $||\sk_\bfy||_\infty \leq \ell B_y \sigma_1 \sqrt{\secparam}$. Therefore, $(\pk_\bfy, \sk_\bfy) \in \rpsis_{m, q, \beta_0}$ for $\beta_0 = \ell B_y \sigma_1 \sqrt{\secparam}$. Hence, choosing $R_\rsis = \rpsis_{m, q, \beta_0}$ ensures that this special property is satisfied. \nikhil{do we need unique solution setting? in that case we will need an additional constraint on $m$.}

\item 
{\bf IPFE correctness holds even w.r.t.\ a functional secret key satisfying $R'_\rsis$.} Based on the description of the lattice-based adaptor signature construction in~\Cref{sec:las}, we note that $R'_\rsis = \rpsis_{m, q, \beta_1}$, where $\beta_1 = 2(\gamma-\kappa)-\beta_0$. We need to then show that for any $\secparam \in \N$,
let $\pp \gets \Gen(1^\secparam)$, 
then for any 
$ \ell \in \N, \bfx \in \Z^\ell, \bfy \in \Z^\ell$ such that $||\bfx||_\infty \leq B_x$, $||\bfy||_\infty \leq B_y$, 
the following holds:
\[
\Pr\left[
v = \bfx^T \bfy: 
\begin{array}{l}
(\mpk, \msk) \leftarrow  \Setup(\pp, n),\\ 
\pk_\bfy = \PubKGen(\mpk, \bfy),\\ 
\sk_\bfy \ s.t.\ (\pk_\bfy, \sk_\bfy) \in \rpsis_{m, q, \beta_1},\\
\ct \leftarrow \Enc(\mpk, \bfx),\\ 
v = \Dec(\sk_\bfy, \ct)
\end{array}
\right] = 1.
\]
Recall from the correctness calculation in the $\Dec$ algorithm,  
\[d = \lfloor q/K \rfloor (\bfx^T\bfy) 1_R + (\bfe_1^T\bfy - \bfe_0^T \sk_\bfy).
\] 
Therefore, for correctness to hold even w.r.t.\ $\sk_\bfy$ satisfying $\rpsis_{m, q, \beta_1}$, we need that $||\bfe_1^T\bfy - \bfe_0^T \sk_\bfy||_\infty < \lfloor q/2K \rfloor$, or equivalently $(\ell B_y \sigma_3 \sqrt{\lambda} + \ell n \beta_1 \sigma_2 \sqrt{\lambda}) < \lfloor q/2K \rfloor$. 
Substituting $\beta_1 = 2(\gamma-\kappa)-\beta_0$, $\gamma = 2n\kappa$, $\beta_0 = \ell B_y \sigma_1 \sqrt{\lambda}$, we get the constraint $\ell \sqrt{\lambda}(B_y \sigma_3 + 2n(2n-1)\sigma_2\kappa - n\ell B_y \sigma_1 \sigma_2 \sqrt{\lambda}) < \lfloor q/2K \rfloor$. We conclude that, as long as we choose IPFE parameters that satisfy this contraint, the special property is also satisfied. 
\end{itemize}

\begin{lemma}[Theorem 4 of~\cite{ipfe-rlwe}]
The above IPFE construction is adaptive, IND-secure with proper choice of parameters and under the $\rlwe$ assumption.
\label{lemma:ipfe-rlwe-ind}
\end{lemma}
\nikhil{define adaptive, IND-security in prelims}

\begin{lemma}[\nikhil{add cites}]
Any adaptive, IND-secure IPFE scheme is also selective, SIM-secure.
\nikhil{double check this claim}
\label{lemma:ipfe-indtosim}
\end{lemma}

\begin{lemma}
The above IPFE construction is selective, SIM-secure with proper choice of parameters and under the $\rlwe$ assumption.
\label{lemma:ipfe-rlwe-sim}
\end{lemma}
\begin{proof}
Follows from~\Cref{lemma:ipfe-rlwe-ind,lemma:ipfe-indtosim}.
\end{proof}

\paragraph{Parameter choices.}
The constraints on the parameters based on correctness and security requirements are as follows:
\begin{itemize}
\item 
{\bf Correctness.} Requires 
$\ell B_y (\sigma_3 \sqrt{\secparam} + mn \sigma_1 \sigma_2 \secparam) < \lfloor q/2K \rfloor$ and 
$q \gg K > \ell B_x B_y$
\item 
{\bf Additional special properties.} Requires 
% $\beta_0 = \ell B_y \sigma_1 \sqrt{\lambda}$, 
$\ell \sqrt{\lambda}(B_y \sigma_3 + 2n(2n-1)\sigma_2\kappa - n\ell B_y \sigma_1 \sigma_2 \sqrt{\lambda}) < \lfloor q/2K \rfloor$.
\item 
{\bf Adaptor Signature construction in~\Cref{sec:las}.} Requires 
\begin{itemize}
\item 
$\gamma - \kappa > \beta_0$, where $\gamma = 2n\kappa$ and $\beta_0 = \ell B_y \sigma_1 \sqrt{\lambda}$. Equivalently, this requires $(2n-1)\kappa > \ell B_y \sigma_1 \sqrt{\lambda}$.
\item 
modulus $q$ in IPFE and AS constructions should be same.
\end{itemize}
\item 
{\bf Theorem 4 of~\cite{ipfe-rlwe}.} Requires 
\begin{itemize}
\item 
$\sigma_3 = \sqrt{m} \sigma_2$. 
\item $\Gamma_{\sigma_2 I_n, \sigma_2 I_n} \geq \eta_\epsilon(\Z^n)$ with $\epsilon=2^{-\secparam}$. 
\nikhil{what is $\Gamma$?}
\item 
$\sigma \sqrt{1 - \frac{1}{\sigma_2^2} (\sigma n C \sqrt{\ell+2})^2} > \eta_\epsilon(\Z^{n+n\ell})$ where $||\bfs_i||_\infty, ||\bfe_1||_\infty \leq C$ and $\sigma$ is the parameter for the hardness of of \rlwe with $m$ samples. One can set $C=\sqrt{\secparam}\sigma_1$.
\nikhil{what is $\eta$?}
\item 
$\sigma_1 \geq 2\sqrt{\ell}B_x \sigma'$ for non-negatives $\sigma'$ where $\sigma_1, \sigma'$ satisfy $\Gamma_{\Sigma, \sigma'^2 \mathbf{\alpha}^T \mathbf{\alpha}} \geq \eta_\epsilon(\Z^n)$ with $\epsilon' = 2^{-\secparam}/nm$ and $\epsilon = \epsilon'/(2B_x)^{2\ell}$.
\item 
$n$ be a power-of-2 such that $\Phi = x^n + 1$ splits into $n$ linear factors modulo prime $q$, $m\geq 3$, $\delta \in (0,1/2), \epsilon>0, \sigma' \geq \sqrt{n \ln(2mn(1+1/\delta)/\pi)} q^{\frac{2}{m} + \frac{\epsilon}{2}}$ such that $(2\delta + 2^n \frac{1}{q^{\epsilon n}} (\frac{q^{2m}}{(q^m-1)(q^m-q)})^n) \cdot (2B_x)^{2\ell}$ is negligible.
\end{itemize} 

\end{itemize}
\nikhil{add concrete choices of $n, q, K, m, \sigma_1, \sigma_2, \sigma_3$ to fully specify IPFE and $n, q, \kappa$ to fully specify AS?}

\subsection{Lattice-based Adaptor Signatures}
\label{sec:las}

We first describe the digital signature scheme $\ds$ w.r.t.\ which we will build our adaptor signature scheme. \nikhil{cite Lyu09?}

Let $\mcal{H}: \{0,1\}^* \to \C$ be a family of hash functions (modelled as a random oracle), where $\C = \{c \in \Ring: ||c||_1 = \kappa \wedge ||c||_\infty = 1\}$. Let $\gamma$ be the maximum absolute coefficient of the masking randomness $\bfy$ used in the $\Sign$ algorithm below. Then, the digitial signature scheme $\ds$ is as in~\Cref{fig:ds-constr-lattices}

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed, space=1em]

\begin{pcvstack}
\procedure[linenumbering, mode=text]{$\Gen(1^\secparam)$}{
Choose $n$ to be a power-of-2 \nikhil{depends on $\secparam$?}
\\ 
Choose an odd modulus $q$ \nikhil{prime? depends on $\secparam?$}
\\ 
Let $\Ring = \Z[X]/(X^n+1)$, $\Ring_q = \Ring/q\Ring$
\\ 
% Choose interger $m$ as described in ??
% \\ 
% Output $\pp = (q, \Ring, \Ring_q, m)$
Sample $\H \getr \mcal{H}$
\\ 
Output $\pp = (q, \Ring, \Ring_q, \H)$
}

\procedure[linenumbering, mode=text]{$\KGen(1^\secparam, \pp)$}{ 
Sample $a' \getr \Ring_q$, let $\bfa = (1 || a')^T \in \Ring_q^2$
\\ 
Sample $\bfr \getr \S_1^2$, let $t = \bfa^T\bfr$
\\ 
Output $\vk = (\bfa, t), \sk = \bfr$
}
\end{pcvstack}

\begin{pcvstack}
\procedure[linenumbering, mode=text]{$\Sign(\sk, m)$}{ 
Sample $\bfy \getr \S_\gamma^2$, let $w = \bfa^T \bfy$
\\ 
Compute $c = \H(\vk \ ||\  w \ ||\  m)$
\\ 
Compute $\bfz = \bfy + \bfr c$
\\ 
If $||\bfz||_\infty > \gamma - \kappa$: restart 
\\ 
Output $\sigma = (c, \bfz)$
}

\procedure[linenumbering, mode=text]{$\Verify(\vk, m, \sigma)$}{ 
Parse $\sigma = (c, \bfz)$
\\ 
If $||\bfz||_\infty > \gamma - \kappa$: output $0$
\\ 
Compute $w' := \bfa^T\bfz - t c $
\\ 
If $c \neq \H(\vk \ ||\  w' \ ||\ m)$: output $0$
\\ 
Output $1$
}
\end{pcvstack}

\end{pcvstack}
\caption{Digital signature scheme $\ds$ from \rsis and \rlwe}
\label{fig:ds-constr-lattices}
\end{figure}

\nikhil{add correctness and security statement for the above $\ds$ scheme. Based on Lyu09? Lyu12? EEE20?}

Next, we describe our adaptor signature scheme $\las$ w.r.t.\ the digitial signature scheme $\ds$ (\Cref{fig:ds-constr-lattices}) and hard relations $R_\rsis = \rpsis_{m, q, \beta_0}$ and $R'_\rsis = \rpsis_{m, q, \beta_1}$, where $\beta_0 = \ell B_y \sigma_1 \sqrt{\secparam}$ and $\beta_1 = 2(\gamma - \kappa) - \beta_0$ s.t. $\beta_1 > \beta_0$ and $\gamma - \kappa - \beta_0 > 0$. 
\nikhil{note this additional constraint in the summary of constraints and final parameter choices.}
Hence, for $R_\rsis$, statements are of the form $(\bfa, X)$ for $\bfa \in \Ring_q^m$ and $X \in \Ring_q$ (same for $R'_\rsis$), and witnesses are of the form $\bfx \in \Ring^m$ s.t. $||\bfx||_\infty \leq \beta_0$ ($||\bfx||_\infty \leq \beta_1$ for $R'_\rsis$). As $\bfa$ is also part of the verification key $\vk$, henceforth we drop it from the statement.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{pcvstack}[boxed, space=1em]

\begin{pcvstack}
\procedure[linenumbering, mode=text]{$\PreSign(\sk, m, X)$}{ 
Sample $\bfy \getr \S_\gamma^2$, let $w = \bfa^T \bfy$
\\ 
Compute $c = \H(\vk \ ||\  w + X \ ||\  m)$
\\ 
Compute $\widetilde{\bfz} = \bfy + \bfr c$
\\ 
If $||\widetilde{\bfz}||_\infty > \gamma - \kappa - \beta_0$: restart 
\\ 
Output $\widetilde{\sigma} = (c, \widetilde{\bfz})$
}

\procedure[linenumbering, mode=text]{$\Adapt(\vk, m, X, \bfx, \widetilde{\sigma})$}{
If $\PreVerify(\vk, m, X, \widetilde{\sigma})=0$: return $\bot$
\\ 
Parse $\widetilde{\sigma} = (c, \widetilde{\bfz})$
\\ 
Output $\sigma = (c, \bfz = \widetilde{\bfz} + \bfx)$
}

\end{pcvstack}

\begin{pcvstack}
\procedure[linenumbering, mode=text]{$\PreVerify(\vk, m, X, \widetilde{\sigma})$}{ 
Parse $\widetilde{\sigma} = (c, \widetilde{\bfz})$
\\ 
If $||\widetilde{\bfz}||_\infty > \gamma - \kappa - \beta_0$: output $0$
\\ 
Compute $w' = \bfa^T \widetilde{\bfz} - t c $
\\ 
If $c \neq \H(\vk \ ||\ w'+X \ ||\ m)$: output $0$
\\ 
Output $1$
}

\procedure[linenumbering, mode=text]{$\Ext(\widetilde{\sigma}, \sigma, X)$}{ 
Parse $\widetilde{\sigma} = (c, \widetilde{\bfz})$ and $\widetilde{\sigma} = (c, \bfz)$
\\ 
If $X \neq \bfa^T (\bfz - \widetilde{\bfz})$: output $\bot$
\\ 
Output $\bfz - \widetilde{\bfz}$
}
\end{pcvstack}
\end{pcvstack}
\caption{Adaptor signature scheme $\las$ from \rsis and \rlwe}
\label{fig:as-constr-lattices}
\end{figure}

\paragraph{Parameter choices and comparison.}
Our construction can be seen as similar to~\cite{pq-as} but with module rank $1$ instead of $4$. Our costruction is different from~\cite{pq-as} in the following aspects though:~\cite{pq-as} chooses $\beta_0 = 1$, whereas we choose $\beta_0 = \ell B_y \sigma_1 \sqrt{\lambda}$, where parameters $\ell, B_y, \sigma_1$ are chosen based on their specification in the IPFE construction in~\Cref{fig:ipfe-rlwe}. Further,~\cite{pq-as} sets $\beta_1 = 2(\gamma-\kappa)$ whereas we set it a stricter bound on it $\beta_1 = 2(\gamma-\kappa)-\beta_0$ as it is sufficient for correctness and security. Further, note that for the choice of $\beta_1$, the two constraints 
$\beta_1 > \beta_0$ and $\gamma - \kappa - \beta_0 > 0$ are equivalent. Lastly, we note that just like in~\cite{pq-as}, we can set $\gamma = 2 n\kappa$ to ensure that the average number of restarts in $\Sign$ and $\PreSign$ is about $e < 3$, where $n$ is the degree of degree of the cyclotomic ring $\Ring$ and $\kappa$ is the $\ell_1$ norm of values in the range set $\C$ of the hash family $\mcal{H}$.

\paragraph{Correctness.} Follows in a strightforward way.

\paragraph{Security.} All security properties follow from~\cite{pq-as}, but they are based on ring variants of $\sis$ and $\lwe$ instead of module variants. We provide the formal statements below.

\begin{lemma}
If $\rsis_{3, q, \beta}$ for $\beta = 2\gamma\sqrt{2n}$ and $\rlwe_{1, q, \Phi}$ for $\Phi = \S_1$ are hard, then, the adaptor signature construction $\las$ in~\Cref{fig:as-constr-lattices} is secure in the random oracle model.
\end{lemma}
\begin{proof}
Follows from~\Cref{claim:as-unf,claim:as-pre-sig-adaptability,claim:as-wit-ext}.
\end{proof}

\begin{claim}[Weak pre-signature adaptability (Adapted from Lemma 1 of~\cite{pq-as})]
\label{claim:as-pre-sig-adaptability}
$\las$ satisfies weak pre-signature adaptability w.r.t.\ the relation $R_\rsis$.
\end{claim}
% \begin{proof}
% For any $\secparam \in \N$, 
% any message $m \in \{0,1\}^*$, 
% any key pair $(\vk = (\bfa, t), \sk=\bfr) \gets \KGen(1^\secparam)$, 
% any statement/witness pair $(X, \bfx) \in R_\rsis$, 
% and any pre-signature $\widetilde{\sigma} = (c, \widetilde{\bfz})$ 
% with $\PreVerify(\vk, m, X, \widetilde{\sigma}) = 1$, we have:
% \begin{align*}
% \Pr[\Verify(\vk, m, \Adapt(\vk, m, X, \bfx, \widetilde{\sigma})) = 1] 
% & = \Pr[\Verify(\vk, m, (c, \widetilde{\bfz} + \bfx)) = 1] \\ 
% & = \Pr\left[\begin{matrix}||\widetilde{\bfz} + \bfx||_\infty \leq (\gamma - \kappa) \ \wedge \\ c = \H(\vk \ ||\ w' \ || \ m) \end{matrix}: w' = \bfa^T(\widetilde{\bfz} + \bfx) - tc \right] \\
% & = \Pr\left[\begin{matrix}||\widetilde{\bfz} + \bfx||_\infty \leq (\gamma - \kappa) \ \wedge \\ c = \H(\vk \ ||\ w' \ || \ m) \end{matrix}: w' = \bfa^T\widetilde{\bfz} + X - tc \right] \\
% & = \Pr\left[\begin{matrix}||\widetilde{\bfz} + \bfx||_\infty \leq (\gamma - \kappa) \ \wedge \\ c = \H(\vk \ ||\ w'+X \ || \ m) \end{matrix}: w' = \bfa^T\widetilde{\bfz} - tc \right] 
% \end{align*}
% Note that $||\widetilde{\bfz}||_\infty \leq \gamma - \kappa - \beta_0$ as $\PreVerify(\vk, m, X, \widetilde{\sigma}) = 1$. Further, $||\bfx||_\infty \leq \beta_0$ as $(X, \bfx) \in R_\rsis$.
% Then, we get that $||\widetilde{\bfz} + \bfx||_\infty \leq ||\widetilde{\bfz}||_\infty + ||\bfx||_\infty \leq \gamma - \kappa$. Further, we have that $c = \H(\vk \ ||\ w'+X \ || \ m)$, where $w' = \bfa^T\widetilde{\bfz} - tc$ as $\PreVerify(\vk, m, X, \widetilde{\sigma}) = 1$. Thus, we conclude that $\Pr[\Verify(\vk, m, \Adapt(\vk, m, X, \bfx, \widetilde{\sigma})) = 1] = 1$.
% \end{proof}

\begin{claim}[Witness Extractability (Adapted from Lemma 2 of~\cite{pq-as})]
\label{claim:as-wit-ext}
If $\rsis_{3, q, \beta}$ for $\beta = 2\gamma\sqrt{2n}$ and $\rlwe_{1, q, \Phi}$ for $\Phi = \S_1$ are hard, then, $\las$ is witness extractable in the random oracle model.
\end{claim}


\begin{claim}[Unforgeability (Adapted from Lemma 3 of~\cite{pq-as})]
\label{claim:as-unf}
If $\rsis_{3, q, \beta}$ for $\beta = 2\gamma\sqrt{2n}$ and $\rlwe_{1, q, \Phi}$ for $\Phi = \S_1$ are hard, then, $\las$ is aEUF-CMA secure in the random oracle model.
\end{claim}

% \begin{proof}

% We need to show that 
% for every \ppt adversary \A there exists a negligible function $\negl$ such that
% for all $\secparam \in \N$,
% \[
% \Pr[ G_0(1^\secparam) = 1] \leq \negl(\secparam),
% \]
% where the game $G_0$ 
% is defined as in~\Cref{fig:las-unf-exp}.

% \begin{figure}[H]
% \centering
% \captionsetup{justification=centering}
% \begin{pchstack}[boxed, space=1em]
% \begin{pcvstack}[space=1em]
% \procedure[linenumbering, mode=text]{Games $G_0$, \pcbox{G_1}, {\color{blue} \pcbox{ \color{black} G_2}}.}{
% $\mcal{Q} := \emptyset$ \\
% $a' \getr \Ring_q$, $\bfa = (1 || a')^T \in \Ring_q^2$
% \\ 
% $\bfr \getr \S_1^2$, $t = \bfa^T\bfr$
% \\ 
% $\vk = (\bfa, t)$, $\sk = \bfr$
% \\ 
% $m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{pS}(\cdot, \cdot)}(\vk)$ \\ 
% $(X^*, \bfx^*) \gets R_\rsis.\GenR(1^\secparam)$ \\ 
% $\bfy^* \getr \S_\gamma^2$, $w^* = \bfa^T \bfy^*$
% \\ 
% $\widetilde{c^*} = \H(\vk \ ||\  w^* + X^* \ ||\  m^*)$
% \\ 
% $\widetilde{\bfz^*} = \bfy^* + \bfr \widetilde{c^*}$
% \\ 
% If $||\widetilde{\bfz^*}||_\infty > \gamma - \kappa - \beta_0$: restart 
% \\ 
% $\widetilde{\sigma^*} = (\widetilde{c^*}, \widetilde{\bfz^*})$
% \\
% $\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{pS}(\cdot, \cdot)}(\widetilde{\sigma^*}, X^*)$ 
% \\ 
% Parse $\sigma^* = (c^*, \bfz^*)$
% \\ 
% $w'^* = \bfa^T\bfz^* - tc^*$
% \\
% return $((m^* \notin \mcal{Q}) \wedge (||\bfz^*||_\infty \leq \gamma-\kappa) \wedge (c^* = \H(\vk\ ||\ w'^*\ || \ m^*)))$
% } 

% \end{pcvstack}
% \begin{pcvstack}[space=1em]

% \procedure[linenumbering, mode=text]{Oracle $\mcal{O}_S(m)$}{
% $\bfy \getr \S_\gamma^2$, $w = \bfa^T \bfy$
% \\ 
% $c = \H(\vk \ ||\  w \ ||\  m)$
% \\ 
% $\bfz = \bfy + \bfr c$
% \\ 
% If $||\bfz||_\infty > \gamma - \kappa$: restart 
% \\ 
% $\sigma = (c, \bfz)$
% \\ 
% $\mcal{Q} := \mcal{Q} \vee \{m\}$
% \\ 
% return $\sigma$
% }

% \procedure[linenumbering, mode=text]{Oracle $\mcal{O}_{pS}(m, X)$}{
% $\bfy \getr \S_\gamma^2$, $w = \bfa^T \bfy$
% \\ 
% $c = \H(\vk \ ||\  w + X \ ||\  m)$
% \\ 
% $\widetilde{\bfz} = \bfy + \bfr c$
% \\ 
% If $||\widetilde{\bfz}||_\infty > \gamma - \kappa - \beta_0$: restart 
% \\ 
% $\widetilde{\sigma} = (c, \widetilde{\bfz})$
% \\
% $\mcal{Q} := \mcal{Q} \vee \{m\}$ 
% \\ 
% return $\widetilde{\sigma}$
% }
% \end{pcvstack}

% \end{pchstack}
% \caption{Unforgeability experiment of $\las$}
% \label{fig:las-unf-exp}
% \end{figure}

% First, from the assumption $\rsis_{3, q, \beta}$ for $\beta = 2\gamma\sqrt{2n}$, it follows that $R_\rsis = \rpsis_{2,q,\beta_0}$ and $R'_\rsis = \rpsis_{2,q,\beta_1}$ for $\beta_0 =\ell B_y \sigma_1 \sqrt{\secparam} $ and $\beta_1 = 2(\gamma-\kappa)-\beta_0$ are hard as $\beta_0 < \beta_1 < \beta$.

% Next, from the assumption $\rlwe_{1, q, \Phi}$ for $\Phi = \S_1$, it follows that $(a', X)$ is indistinguishable from a uniformly random element in $\Ring_q^2$, where $\bfa = (1||a')^T$ is as sampled in $\KGen$ and and $X$ is as sampled in $R_\rsis.\GenR(1^\secparam)$. This is because $R_\rsis.\GenR(1^\secparam)$ outputs $(X, \bfx)$, where $\bfx = (x_0, x_1) \getr \S_1^2$ and $X = \bfa^T \bfx = x_0 + a'x_1$. Thus, $X$ looks like an $\rlwe$ sample with secret $x_1$ and error $x_0$ coming from distribution $\S_1$.

% Let \A be a \ppt adversary who wins the aEUF-CMA security game with non-neglegible probability. We will build a reduction \B that solves $\rsis_{3,q,\beta}$. 
% Let $\bfb = (1\ || \ a' \ ||\ \alpha)^T \in \Ring_q^3$ for $a' \getr \Ring_q$ and $\alpha \getr \Ring_q$. Assume that \B wants to solve $\rsis$ w.r.t.\ $\bfb$. Let $\bfa = (1\ || \ a')^T$. 
% \end{proof}

\subsection{$\fas$ construction}

Instantiating $\fas$ construction in~\Cref{sec:fas-construction} with $\ipfe$ from~\Cref{sec:ipfe-rlwe} and $\as$ from~\Cref{sec:las}, we obtain the following theorem.

\begin{theorem}
\label{thm:fas-strongly-secure-lattices}
Let $\mcal{F}_{IP, \Z^\ell, B_y} = \{\bfy \in \Z^\ell \ s.t. \ \bfy \neq {\bf 0}\  \wedge \ ||\bfy||_\infty \leq B_y\}$, where $\ell$ is a positive integer and $B_y > 0$.
Let $R$ be any relation 
with statement/witness pairs $(X, \bfx)$ such that $\bfx \in \Z^\ell$ and $||\bfx||_\infty \leq B_x$ for some $B_x >0$.
Suppose that 
\begin{itemize}
\item
$R$ is $\mcal{F}_{IP,\Z^\ell, B_y}$-hard,
\item
$\nizk$ is a secure NIZK argument system,
\item
$\as$ (\Cref{fig:as-constr-lattices}) is a secure adaptor signature scheme w.r.t.\ digital signature scheme $\ds$ (\Cref{fig:ds-constr-lattices}) and hard relations $R_\rsis, R'_\rsis$,
\item
$\ipfe$ (\Cref{fig:ipfe-rlwe}) is a selective, SIM-secure IPFE scheme that satisfies two additional special properties: (i) ``Functional public and secret keys satisfy the hard relation $R_\rsis$'', and (ii) ``IPFE correctness holds even w.r.t.\ a functional secret key satisfying $R'_\rsis$''.
\end{itemize} 
Then, the functional adaptor signature scheme 
w.r.t.\ digital signature scheme $\DS$, hard relation $R$, and family of inner product functions $\mcal{F}_{IP, \Z^\ell, B_y}$  
constructed in~\Cref{sec:construction} is strongly-secure as defined in~\Cref{def:fas-strongly-secure}.
\end{theorem}




==> fas-proof-unforgeability-new.tex <==
\subsubsection{Unforgeability}

To prove unforgeability of our functional adaptor signature construction in~\Cref{sec:construction}, we need to open up the blackbox of Adaptor Signature scheme $\as$. \nikhil{explain why}

We instantiate the Adaptor Signature scheme to be Schnorr-based as constructed in~\cite{asig}. 
In such a case, $\DS = \Sch$. 
Let $G$ be a cyclic group of prime order $q$, with generator $g$. 
Let $H: \{0,1\}^* \to \Z_p$ be a hash function modelled as a random oracle. 
The resulting functional adaptor signature scheme is as follows. 
We implicitly assume henceforth that all algorithms have access to $(G, q, g, H)$.

\paragraph{$\Setup(1^\secparam, 1^\ell)$:}
\begin{itemize}[itemsep=0.1em]
\item Compute $\crs \gets \nizk.\Setup(1^\secparam)$.
\nikhil{does the nizk setup need to take $1^\ell$ as input too?}
\item Compute $\pp' \gets \ipfe.\Gen(1^\secparam)$.
\item Output $\pp = (\crs, \pp')$.
\end{itemize}

\paragraph{$\AdvertisementGen(1^\ell, \pp, X, \bfx)$:}
\begin{itemize}[itemsep=0.1em]
\item 
Compute the master keys for IPE as $(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$. 
\item 
Sample random coins $r \getr \Z_p$ and compute ciphertext $\ct = \ipe.\Enc(\mpk, \bfx; r)$.
\item 
Compute a proof $\pi \gets \nizk.\Prove(\crs, (X, \mpk, \ct), (\bfx, r))$ attesting that $\ct$ is an IPE encryption of $\bfx$ (which is a witness for statement $X$ w.r.t.\ relation $R$) using master public key $\mpk$ and random coins $r$.
\item 
Output $\advt = (\mpk, \ct, \pi)$, and $\state = \msk$.
\end{itemize}

\paragraph{$\AdvertisementVerify(\pp, X, \advt)$:}
output $\nizk.\Verify(\crs, (X, \mpk, \ct), \pi)$.

\paragraph{$\KGen(1^\secparam, \pp)$:} \nikhil{added crs as input. TODO: update FAS defintion to reflect this change.}
output $(\vk, \sk) \gets \Sch.\KGen(\pp')$, where $\vk$ also contains the hash function $H$. 

\paragraph{$\FPreSign(\advt, \sk, m, X, \bfy \in \mcal{F}^\ell_{IP})$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$. 
\item 
Compute $k \getr \Z_p$, 
$r:=H(\vk||g^k \cdot \pk_\bfy||m)$, 
$\widetilde{s}:= k + r \cdot \sk$.
\item 
Output $\widetilde{\sigma} = (r, \widetilde{s})$.
\end{itemize}

\paragraph{$\FPreVerify(\advt, \vk, m, X, \bfy, \widetilde{\sigma})$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$.
\item 
Parse $\widetilde{\sigma} = (r, \widetilde{s})$ and compute $r' := H(\vk || g^{\widetilde{s}} \cdot \vk^{-r} \cdot \pk_\bfy||m)$.
\item 
Output $1$ iff $( r = r' )$, else $0$.
\end{itemize}

\paragraph{$\Adapt(\advt, \state, \widetilde{\sigma}, \bfy, \bfx)$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$, and $\state = \msk$.
\item 
Compute $\sk_\bfy = \ipe.\KGen(\msk, \bfy)$.
\item
Parse $\widetilde{\sigma} = (r, \widetilde{s})$ and compute $s:=\widetilde{s} + \sk_\bfy$.
\item 
Output $\sigma = (r,s)$.
\end{itemize}

\paragraph{$\Verify(\vk, m, \sigma)$:}
output $\Sch.\Verify(\vk, m, \sigma)$.

\paragraph{$\FExt(\advt, \widetilde{\sigma}, \sigma, X, \bfy)$:}
\begin{itemize}[itemsep=0.1em]
\item
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$.
\item 
Parse $\widetilde{\sigma} = (\widetilde{r}, \widetilde{s})$ and 
$\sigma = (r,s)$. Compute $\sk_\bfy := s - \widetilde{s}$. If $(\pk_\bfy, \sk_\bfy)\notin R_{DL}$, output $\bot$. 
\item 
Output $\bfx^T \bfy = \ipe.\Dec(\sk_\bfy, \ct)$.

\end{itemize}



\begin{lemma}
\label{lemma:fas-unf}
Let $R_{\bfy} = \{(X, z) | \exists \bfx \in \Z_p^\ell \ s.t.\ (X, \bfx) \in R \ and \ z=\bfx^T\bfy\}$ be a relation related to the relation $R$ and vector $\bfy \in \Z_p^\ell$.
Suppose $\Sch$ is strongly unforgeable, 
$R_{\bfy}$ is a hard relation, and 
$\nizk$ satisfies adaptive soundness. 
Then, the functional adaptor signature instantiation above is faEUF-CMA secure.
\nikhil{Note that `$R_\bfy$ is a hard relation' seems like a stronger assumption than `$R$ is a hard relation'.}
\end{lemma}

\begin{proof}
We prove the lemma by defining a sequence of games.

\paragraph{Game $G_0$:} This game corresponds to the original game $\faSigForge_{\A, \FAS}$, where the adversary \A has to come up with a valid forgery on a message $m$ of his choice, while having access to functional pre-sign oracle $\mcal{O}_{\fpS}$ and sign oracle $\mcal{O}_S$. Since we are in the random oracle model, the adversary additionally has access to a random oracle $H$.
Game $G_0$ is formally defined in~\Cref{fig:fasig-unf-g0}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_0$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || g^{k^*} \cdot \pk_{\bfy^*}||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_0$}
\label{fig:fasig-unf-g0}
\end{figure}

\paragraph{Game $G_1$:}
same as game $G_0$, except that 
when \A outputs a public advertisement $\advt$, 
the game checks if the NIZK statement $(X^*, \mpk, \ct)$ is in the language $L_{NIZK}$. If no, the game aborts.
\nikhil{note that this check is inefficient. Is that a problem?}
Game $G_1$ is formally defined in~\Cref{fig:fasig-unf-g1}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_1$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
{\color{blue}
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $0$
}
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || g^{k^*} \cdot \pk_{\bfy^*}||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_1$}
\label{fig:fasig-unf-g1}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g1}
Let ${\sf Bad}_1$ be the event that $G_1$ returns $0$ in step 11. 
If the NIZK scheme satisfies adaptive soundness, then, $\Pr[{\sf Bad}_1] \leq \negl(\secparam)$.
\end{claim}

\begin{proof}
We prove the claim using a reduction to the adaptive soundness of the underlying $\nizk$ scheme. More specifically, we show that if the adversary \A causes game $G_1$ to return $0$ in step 11, then, we can use it to construct a reduction \B that breaks the adaptive soundness of $\nizk$. Let \C be the challenger for the NIZK adaptive soundness. Then, the reduction is as follows.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Reduction \B for proof of~\Cref{claim:fasig-unf-g1}.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
{\color{blue}
$\crs \gets \C(1^\secparam)$
}
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: abort the game with $\C$
\item 
{\color{blue}
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $(\stmt = (X^*, \mpk, \ct), \pi)$ to $\C$
}
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Reduction \B for proof of~\Cref{claim:fasig-unf-g1}.}
\label{fig:fasig-unf-g1-proof}
\end{figure}

Observe that if \A causes game $G_1$ to return $0$ in step 11, then, it must be the case that 
$(X^*, \mpk, \ct) \notin L_{NIZK}$. 
Further note that as the reduction did not abort in the previous step, it must be the case the $\pi$ is a valid proof. 
This means that in step 11, the reduction \B successfully returns a valid proof $\pi$ to $\C$ for a statement $\stmt = (X^*, \mpk, \ct)$ not in the language $L_{NIZK}$ and thus breaks the adaptive soundness of the $\nizk$. Thus, $\Pr[{\sf Bad}_1]$ is same as the probability that $\B$ breaks adaptive soundness of the $\nizk$. Hence, we can concolude that $\Pr[{\sf Bad}_1] \leq \negl(\secparam)$.
\end{proof}

\paragraph{Game $G_2$:}
same as game $G_1$, except that 
when \A outputs a forgery $\sigma^*$, 
the game checks if the resulting extracted value $v$ from $\FExt$ is same as ${\bfx^*}^T \bfy^*$. If yes, the game aborts.
Game $G_2$ is formally defined in~\Cref{fig:fasig-unf-g2}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_2$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $0$
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || g^{k^*} \cdot \pk_{\bfy^*}||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
{\color{blue}
Parse $\sigma^* = (\cdot, s^*)$
}
\item 
{\color{blue}
$z := s^* - \widetilde{s}^*$
}
\item 
{\color{blue}
$v := \ipe.\Dec(z, \ct)$
}
\item 
{\color{blue}
If $v = {\bfx^*}^T \bfy^*$: return 0
}

\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_2$}
\label{fig:fasig-unf-g2}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g2}
Let ${\sf Bad}_2$ be the event that $G_2$ returns $0$ in step 22. 
If $R_\bfy$ is a hard relation, then, $\Pr[{\sf Bad}_2] \leq \negl(\secparam)$.
\end{claim}

\begin{proof}
We prove the claim using a reduction to the hardness of the relation $R_{\bfy}$. 
More specifically, 
we show that if an adversary \A causes game $\G_2$ to return $0$ in step 22, then, 
we can use it to construct a reduction \B that breaks 
the hardness of the relation $R_{\bfy}$. 
Let \C be the challenger for 
the hardness of the relation $R_{\bfy}$. 
\C provides a statement $X^* \in R$, and a vector $\bfy^* \in \Z_p^\ell$ to \B and to win the game, \B must return a scalar value $v$ s.t.\ $v = {\bfx^*}^T \bfy^*$ where vector $\bfx^*$ satsifies $(X^*, \bfx^*) \in R$.
The reduction \B is as follows.


\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Reduction \B for proof of~\Cref{claim:fasig-unf-g2}.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
{\color{blue}
$(X^*, \bfy^*) \gets \C(1^\secparam)$
}
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return $v \getr \Z_p$
\item 
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $v \getr Z_p$
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || g^{k^*} \cdot \pk_{\bfy^*}||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
{\color{blue}
Parse $\sigma^* = (\cdot, s^*)$
}
\item 
{\color{blue}
$z := s^* - \widetilde{s}^*$
}
\item 
{\color{blue}
$v := \ipe.\Dec(z, \ct)$
}
\item 
{\color{blue}
return $v$
}
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Reduction \B for proof of~\Cref{claim:fasig-unf-g2}}
\label{fig:fasig-unf-g2-proof}
\end{figure}

Observe that if \A causes game $G_2$ to return $0$ in step 22, then, it must be the case that $v = {\bfx^*}^T \bfy^*$. In such a case, \B wins the game against challenger \C. Formally, we have that
\begin{align*}
\Pr[\B \ \text{wins}] 
& \geq  
\Pr[\nizk.\Verify(\crs, (X^*, \mpk, \ct) = 0] \cdot 1/q \\
& \quad + 
\Pr[\nizk.\Verify(\crs, (X^*, \mpk, \ct) = 1 \wedge (X^*, \mpk, \ct)\notin L_{NIZK}] \cdot 1/q \\
& \quad + 
\Pr[\nizk.\Verify(\crs, (X^*, \mpk, \ct) = 1 \wedge (X^*, \mpk, \ct)\in L_{NIZK}]) \Pr[v = {\bfx^*}^T \bfy^*] \\ 
& \geq 
\Pr[\nizk.\Verify(\crs, (X^*, \mpk, \ct) = 1 \wedge (X^*, \mpk, \ct)\in L_{NIZK}]) \Pr[v = {\bfx^*}^T \bfy^*] \\ 
& = \Pr[{\sf Bad}_2].
\end{align*}

From hardness of the relation $R_{\bfy}$, it follows that $\Pr[\B\ \text{wins}] \leq \negl(\secparam)$. Hence, we conclude that $\Pr[{\sf Bad}_2] \leq \negl(\secparam)$.

\end{proof}

\paragraph{Game $G_3$:}
same as game $G_2$, except that 
the behaviour of $\mcal{O}_{\fpS}$ oracle is different.
In this game, $\mcal{O}_{\fpS}$ makes a copy of the list $H$ 
before executing the algorithm $\FPreSign$. 
Afterwards, it extracts the randomness $K$ used during the 
$\FPreSign$ algorithm, and checks if 
befroe the execution of the signing algorithm 
a query of the form $\vk||K||m$ or $\vk||K \cdot \pk_\bfy || m$ 
was made to $H$ by checking if $H'[\vk||K||m] \neq \bot$ or 
$H'[\vk||K \cdot \pk_\bfy ||m] \neq \bot$. If so, the game aborts.
Game $G_3$ is formally defined in~\Cref{fig:fasig-unf-g3}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_3$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $0$
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || g^{k^*} \cdot \pk_{\bfy^*}||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
Parse $\sigma^* = (\cdot, s^*)$
\item 
$z := s^* - \widetilde{s}^*$
\item 
$v := \ipe.\Dec(z, \ct)$
\item 
If $v = {\bfx^*}^T \bfy^*$: return 0
\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
{\color{blue} $H' = H$}
\item
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
{\color{blue} 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
}
\item 
{\color{blue} 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
}
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_3$}
\label{fig:fasig-unf-g3}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g3}
Let ${\sf Bad}_3$ be the event that game $G_3$ aborts in $\mcal{O}_{\fpS}$. Then, $\Pr[{\sf Bad}_3] \leq \negl(\secparam)$.
\end{claim}
\begin{proof}
\nikhil{same as~\cite{asig}. fill details for completeness.}
\end{proof}

\paragraph{Game $G_4$:}
same as game $G_3$ except the behaviour of $\mcal{O}_{\fpS}$ oracle. 
Upon an $\mcal{O}_{\fpS}$ oracle query, the game produces a 
valid full signature $\widetilde{\sigma}$ and adjusts the global list $H$ as follows: 
It assigns the value stored at position 
$\vk || K || m$ to $H[\vk || K \cdot \pk_\bfy || m]$ and 
samples a fresh random value for $H[pk || K || m]$. 
These changes make the full signature  $\widetilde{\sigma}$ “look like” a pre-signature to the adversary, since upon querying the random oracle on $\vk || K \cdot \pk_\bfy || m$, \A obtains the value $H [\vk || K || m]$. 
Game $G_4$ is formally defined in~\Cref{fig:fasig-unf-g4}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_4$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $0$
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || g^{k^*} \cdot \pk_{\bfy^*}||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
Parse $\sigma^* = (\cdot, s^*)$
\item 
$z := s^* - \widetilde{s}^*$
\item 
$v := \ipe.\Dec(z, \ct)$
\item 
If $v = {\bfx^*}^T \bfy^*$: return 0
\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$H' = H$
\item
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||{\color{blue}g^k}||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
\item 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
% \item 
% {\color{blue} 
% $\alpha = \vk || g^k || m$
% }
% \item 
% {\color{blue} 
% $\alpha' = \vk || g^k \cdot \pk_\bfy || m$
% }
\item 
{\color{blue} 
$H[\vk || K \cdot \pk_\bfy || m] = H[\vk || K || m]$
% $H[\alpha'] = H[\alpha]$
}
\item 
{\color{blue} 
$H[\vk || K || m] \getr \Z_p$
% $H[\alpha] \getr \Z_p$
}
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_4$}
\label{fig:fasig-unf-g4}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g4}
$\Pr[G_3 = 1] = \Pr[G_4 = 1]$.
\end{claim}
\begin{proof}
The adversary can only notice the changes from $G_3$ to $G_4$, in case the random oracle has been previously queried on either $\vk || K || m$ or $\vk || K \cdot \pk_\bfy || m$. This case has been captured in the previous game $G_3$ and hence it holds that $\Pr[G_2 = 1] = \Pr[G_3 = 1]$.
\end{proof}

\paragraph{Game $G_5$:}
same as game $G_4$ except the we apply the exact same changes made in game $G_3$ in oracle $\mcal{O}_{\fpS}$ to the challenge phase of the game. For computing the pre-signature on $m^*$, first a copy of the list $H$ is made. After computing the pre-signature, game extracts the randomness $K^*$ used during pre-signing and checks if before the execution of the pre-signing algorithm a query of the form $\vk||K^*||m^*$ or $\vk||K^* \cdot \pk_{\bfy^*} || m^*$ was made to $H$. This is done by checking if $H'[\vk||K^*||m^*] \neq \bot$ or $H'[\vk||K^* \cdot \pk_{\bfy^*} || m^*] \neq \bot$. If so, the game returns $0$. 
Game $G_5$ is formally defined in~\Cref{fig:fasig-unf-g5}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_5$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $0$
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
{\color{blue}
$H' = H$
}
\item
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || g^{k^*} \cdot \pk_{\bfy^*}||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
{\color{blue} 
$K^* = g^{\widetilde{s}^*} \cdot \vk^{-r^*}$
}
\item 
{\color{blue} 
if $H'[\vk||K^*||m^*] \neq \bot$ or $H'[\vk||K^* \cdot \pk_{\bfy^*} || m^*] \neq \bot$: return 0
}
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
Parse $\sigma^* = (\cdot, s^*)$
\item 
$z := s^* - \widetilde{s}^*$
\item 
$v := \ipe.\Dec(z, \ct)$
\item 
If $v = {\bfx^*}^T \bfy^*$: return 0
\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$H' = H$
\item
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||g^k||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
\item 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
% \item 
% {\color{blue} 
% $\alpha = \vk || g^k || m$
% }
% \item 
% {\color{blue} 
% $\alpha' = \vk || g^k \cdot \pk_\bfy || m$
% }
\item 
$H[\vk || K \cdot \pk_\bfy || m] = H[\vk || K || m]$
% $H[\alpha'] = H[\alpha]$
\item 
$H[\vk || K || m] \getr \Z_p$
% $H[\alpha] \getr \Z_p$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_5$}
\label{fig:fasig-unf-g5}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g5}
Let ${\sf Bad}_5$ be the event that game $G_3$ returns $0$ in step 20. Then, $\Pr[{\sf Bad}_5] \leq \negl(\secparam)$.
\end{claim}
\begin{proof}
\nikhil{similar to proof of~\Cref{claim:fasig-unf-g3}.}
\end{proof}

\paragraph{Game $G_6$:}
same as game $G_6$ except the behaviour of computing the challenge pre-signature. We apply the exact same changes made in game $G_4$ in oracle $\mcal{O}_{\fpS}$.  
The game produces a 
valid full signature $\widetilde{\sigma}^*$ and adjusts the global list $H$ as follows: 
It assigns the value stored at position 
$\vk || K^* || m^*$ to $H[\vk || K^* \cdot \pk_{\bfy^*} || m^*]$ and 
samples a fresh random value for $H[\vk || K^* || m^*]$. 
These changes make the full signature  $\widetilde{\sigma}^*$ “look like” a pre-signature to the adversary, since upon querying the random oracle on $\vk || K^* \cdot \pk_{\bfy^*} || m^*$, \A obtains the value $H [\vk || K^* || m^*]$. 
Game $G_6$ is formally defined in~\Cref{fig:fasig-unf-g6}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_6$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $0$
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$H' = H$
\item
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
$k^* \getr \Z_p$
\item 
$r^* := H(\vk || {\color{blue} g^{k^*}} ||m^*)$
\item 
$\widetilde{s}^* := k^* + r^* \cdot \sk$
\item 
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*)$
\item 
$K^* = g^{\widetilde{s}^*} \cdot \vk^{-r^*}$
\item 
if $H'[\vk||K^*||m^*] \neq \bot$ or $H'[\vk||K^* \cdot \pk_{\bfy^*} || m^*] \neq \bot$: return 0
\item 
{\color{blue} 
$H[\vk || K^* \cdot \pk_{\bfy^*} || m^*] = H[\vk || K^* || m^*]$
% $H[\alpha'] = H[\alpha]$
}
\item 
{\color{blue} 
$H[\vk || K^* || m^*] \getr \Z_p$
% $H[\alpha] \getr \Z_p$
}
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
Parse $\sigma^* = (\cdot, s^*)$
\item 
$z := s^* - \widetilde{s}^*$
\item 
$v := \ipe.\Dec(z, \ct)$
\item 
If $v = {\bfx^*}^T \bfy^*$: return 0
\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$H' = H$
\item
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=H(\vk||g^k||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
\item 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
% \item 
% {\color{blue} 
% $\alpha = \vk || g^k || m$
% }
% \item 
% {\color{blue} 
% $\alpha' = \vk || g^k \cdot \pk_\bfy || m$
% }
\item 
$H[\vk || K \cdot \pk_\bfy || m] = H[\vk || K || m]$
% $H[\alpha'] = H[\alpha]$
\item 
$H[\vk || K || m] \getr \Z_p$
% $H[\alpha] \getr \Z_p$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_6$}
\label{fig:fasig-unf-g6}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g6}
$\Pr[G_5 = 1] = \Pr[G_6 = 1]$.
\end{claim}
\begin{proof}
The adversary can only notice the changes from $G_5$ to $G_6$, in case the random oracle has been previously queried on either $\vk || K^* || m^*$ or $\vk || K^* \cdot \pk_{\bfy^*} || m^*$. This case has been captured in the previous game $G_5$ and hence it holds that $\Pr[G_5 = 1] = \Pr[G_6 = 1]$.
\end{proof}

\begin{claim}
\label{claim:fasig-unf-last}
Suppose $\Sch$ is strongly unforgeable. 
Then, $\Pr[G_6 = 1] \leq \negl(\secparam)$.
\end{claim}
\begin{proof}
We prove the claim using a reduction to the strong unforgeability of the Schnorr signature scheme $\Sch$.
More specifically, we show that if the adversary \A can cause game $G_6$ to return $1$, then, we can use it to construct a reduction \B that breaks the strong unforgeability of $\Sch$.
Let \C be the challenger for the strong unforgeability of $\Sch$. The reduction \B is as follows.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Reduction \B for proof of~\Cref{claim:fasig-unf-last}.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
{\color{blue}
$\vk \gets \C(\pp')$
}
\item 
$(X^*, \bfx^*) \gets \GenR(1^\secparam)$
\item 
$\advt \gets \A^{\mcal{O}_S(\cdot), H(\cdot)}(\pp, \vk, X^*)$
\item 
Parse $\advt = (\mpk, \ct, \pi)$
\item 
If $\nizk.\Verify(\crs, (X^*, \mpk, \ct), \pi) = 0$: return 0
\item 
If $(X^*, \mpk, \ct) \notin L_{NIZK}$: return $0$
\item 
$m^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}()$
\item 
$H' = H$
\item
$\bfy^* \getr \Z_p^\ell, \pk_{\bfy^*} = \ipe.\PubKGen(\mpk, \bfy^*)$
\item 
{\color{blue}
$\widetilde{\sigma}^* = (r^*, \widetilde{s}^*) \gets \mcal{O}_S^\Sch(m^*)$
}
\item 
$K^* = g^{\widetilde{s}^*} \cdot \vk^{-r^*}$
\item 
if $H'[\vk||K^*||m^*] \neq \bot$ or $H'[\vk||K^* \cdot \pk_{\bfy^*} || m^*] \neq \bot$: return 0
\item 
{\color{blue} 
$H[\vk || K^* \cdot \pk_{\bfy^*} || m^*] = H^\Sch[\vk || K^* || m^*]$
% $H[\alpha'] = H[\alpha]$
}
\item 
{\color{blue} 
$H[\vk || K^* || m^*] = H^\Sch[\vk || K^* \cdot \pk_{\bfy^*} || m^*]$
% $H[\alpha] \getr \Z_p$
}
\item 
$\sigma^* \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), H(\cdot)}(\widetilde{\sigma}^*, \bfy^*)$
\item 
Parse $\sigma^* = (\cdot, s^*)$
\item 
$z := s^* - \widetilde{s}^*$
\item 
$v := \ipe.\Dec(z, \ct)$
\item 
If $v = {\bfx^*}^T \bfy^*$: return 0
\item 
return $((m^* \notin \mcal{Q}) \wedge \Verify(\vk, m^*, \sigma^*))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
{\color{blue}
$\sigma = (r, s) \gets \mcal{O}^\Sch_S(m)$
\item 
$K = g^{s} \cdot \vk^{-r}$
\item 
$H[\vk|| K || m] = H^\Sch[\vk || K || m]$
}
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$H' = H$
\item
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
{\color{blue}
$\widetilde{\sigma} = (r, \widetilde{s}) \gets \mcal{O}^\Sch_S(m)$
}
\item 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
\item 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
% \item 
% {\color{blue} 
% $\alpha = \vk || g^k || m$
% }
% \item 
% {\color{blue} 
% $\alpha' = \vk || g^k \cdot \pk_\bfy || m$
% }
\item 
{\color{blue}
$H[\vk || K \cdot \pk_\bfy || m] = H^\Sch[\vk || K || m]$
}
% $H[\alpha'] = H[\alpha]$
\item 
{\color{blue}
$H[\vk || K || m] = H^\Sch[\vk || K \cdot \pk_\bfy || m]$
}
% $H[\alpha] \getr \Z_p$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $H(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
{\color{blue}
$\ \ H[x] = H^\Sch[x]$
}
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Reduction \B for proof of~\Cref{claim:fasig-unf-last}.}
\label{fig:fasig-unf-g6-proof-last}
\end{figure}

In order to prove this claim, it suffices to show that the tuple $(m^*, \sigma^*)$ has not been output by the oracle $\mcal{O}_S^\Sch$ before. Note that the adversary \A has not previously made a query on the challenge message $m^*$ to either oracle $\mcal{O}_S$ or $\mcal{O}_{\fpS}$. Hence, $\mcal{O}_S^\Sch$ is only queried on $m^*$ in the challenge phase in step 15 of the reduction. If \A outputs $\sigma^*$ which is equal to the signature $\widetilde{\sigma}^*$, then, this would result in $\Verify(\vk, m^*, \sigma^*) = 0$ in step 25 of the reduction because of the programmed random oracle in steps 18 and 19 of the reduction. Hence, to win the game, \A must output a valid signature $\sigma^* \neq \widetilde{\sigma}^*$ and $\mcal{O}_S^\Sch$ has never output $\sigma^*$ on query $m^*$ before. Consequently, $(m^*, \sigma^*)$ constitutes a valid forgery and thus the reduction breaks the strong unforgeability of Schnorr signature scheme $\Sch$. This completes the proof.


\end{proof}


\end{proof}


==> fas-proof-unforgeability.tex <==
\section{Unforgeability}

To prove unforgeability of our functional adaptor signature construction in~\Cref{sec:construction}, we need to open up the blackbox of Adaptor Signature scheme $\as$. \nikhil{explain why}

We instantiate the Adaptor Signature scheme to be Schnorr-based as constructed in~\cite{asig}. 
In such a case, $\DS = \Sch$. 
Let $G$ be a cyclic group of prime order $q$, with generator $g$. 
Let $H: \{0,1\}^* \to \Z_p$ be a hash function modelled as a random oracle. 
The resulting functional adaptor signature scheme is as follows. 
We implicitly assume henceforth that all algorithms have access to $(G, q, g, H)$.

\paragraph{$\Setup(1^\secparam, 1^\ell)$:}
\begin{itemize}[itemsep=0.1em]
\item Compute $\crs \gets \nizk.\Setup(1^\secparam)$.
\nikhil{does the nizk setup need to take $1^\ell$ as input too?}
\item Compute $\pp' \gets \ipfe.\Gen(1^\secparam)$.
\item Output $\pp = (\crs, \pp')$.
\end{itemize}

\paragraph{$\AdvertisementGen(1^\ell, \pp, X, \bfx)$:}
\begin{itemize}[itemsep=0.1em]
\item 
Compute the master keys for IPE as $(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$. 
\item 
Sample random coins $r \getr \Z_p$ and compute ciphertext $\ct = \ipe.\Enc(\mpk, \bfx; r)$.
\item 
Compute a proof $\pi \gets \nizk.\Prove(\crs, (X, \mpk, \ct), (\bfx, r))$ attesting that $\ct$ is an IPE encryption of $\bfx$ (which is a witness for statement $X$ w.r.t.\ relation $R$) using master public key $\mpk$ and random coins $r$.
\item 
Output $\advt = (\mpk, \ct, \pi)$, and $\state = \msk$.
\end{itemize}

\paragraph{$\AdvertisementVerify(\pp, X, \advt)$:}
output $\nizk.\Verify(\pp, (X, \mpk, \ct), \pi)$.

\paragraph{$\KGen(1^\secparam, \pp)$:} \nikhil{added crs as input. TODO: update FAS defintion to reflect this change.}
output $(\vk, \sk) \gets \Sch.\KGen(\pp')$, where $\vk$ also contains the hash function $H$. 

\paragraph{$\FPreSign(\advt, \sk, m, X, \bfy \in \mcal{F}^\ell_{IP})$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$. 
\item 
Compute $k \getr \Z_p$, 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$, 
$\widetilde{s}:= k + r \cdot \sk$.
\item 
Output $\widetilde{\sigma} = (r, \widetilde{s})$.
\end{itemize}

\paragraph{$\FPreVerify(\advt, \vk, m, X, \bfy, \widetilde{\sigma})$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$.
\item 
Parse $\widetilde{\sigma} = (r, \widetilde{s})$ and compute $r' := \mcal{H}(\vk || g^{\widetilde{s}} \cdot \vk^{-r} \cdot \pk_\bfy||m)$.
\item 
Output $1$ iff $( r = r' )$, else $0$.
\end{itemize}

\paragraph{$\Adapt(\advt, \state, \widetilde{\sigma}, \bfy, \bfx)$:}
\begin{itemize}[itemsep=0.1em]
\item 
Parse $\advt = (\mpk, \ct, \pi)$, and $\state = \msk$.
\item 
Compute $\sk_\bfy = \ipe.\KGen(\msk, \bfy)$.
\item
Parse $\widetilde{\sigma} = (r, \widetilde{s})$ and compute $s:=\widetilde{s} + \sk_\bfy$.
\item 
Output $\sigma = (r,s)$.
\end{itemize}

\paragraph{$\Verify(\vk, m, \sigma)$:}
output $\Sch.\Verify(\vk, m, \sigma)$.

\paragraph{$\FExt(\advt, \widetilde{\sigma}, \sigma, X, \bfy)$:}
\begin{itemize}[itemsep=0.1em]
\item
Parse $\advt = (\mpk, \ct, \pi)$.
\item 
Compute $\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$.
\item 
Parse $\widetilde{\sigma} = (\widetilde{r}, \widetilde{s})$ and 
$\sigma = (r,s)$. Compute $\sk_\bfy := s - \widetilde{s}$. If $(\pk_\bfy, \sk_\bfy)\notin R_{DL}$, output $\bot$. 
\item 
Output $\bfx^T \bfy = \ipe.\Dec(\sk_\bfy, \ct)$.

\end{itemize}


\begin{lemma}
\label{lemma:fas-unf-old}
Suppose $\Sch$ is strongly unforgeable, 
$R_{DL}$ is a hard relation, and 
 \ipe satisfies the special properties that 
``master public and secret keys satisfy discrete log relation'' and ``$\ipe.\KGen(\msk, \cdot)$ is a linear function in $\msk$''. 
Then, the functional adaptor signature instantiation above is faEUF-CMA secure.
\end{lemma}

\begin{proof}
We prove the lemma by defining a sequence of games.

\paragraph{Game $G_0$:} This game corresponds to the original game $\faSigForge_{\A, \FAS}$, where the adversary \A has to come up with a valid forgery on a message $m$ of his choice, while having access to functional pre-sign oracle $\mcal{O}_{\fpS}$ and sign oracle $\mcal{O}_S$. Since we are in the random oracle model, the adversary additionally has access to a random oracle $H$.
Game $G_0$ is formally defined in~\Cref{fig:fasig-unf-g0-old}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_0$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X, \bfx) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\pp, \vk)$
\item 
$(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$
\item 
$t \getr \Z_p$, $\ct = \ipe.\Enc(\mpk, \bfx; t)$
\item 
$\pi \gets \nizk.\Prove(\pp, (X, \mpk, \ct), (\bfx, t))$
\item 
$\advt = (\mpk, \ct, \pi), \state = \msk$
\item 
$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\advt)$
\item 
$\bfy \getr \Z_p^\ell, \pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\widetilde{\sigma}, \bfy)$
\item 
return $((m \notin \mcal{Q}) \wedge \Verify(\vk, m, \sigma))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $\mcal{H}(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_0$}
\label{fig:fasig-unf-g0-old}
\end{figure}

\paragraph{Game $G_1$:}
same as game $G_0$, except that 
when \A outputs a forgery $\sigma$, 
the game checks if completing the pre-signature $\widetilde{\sigma}$ using the secret value $\sk_\bfy = \ipe.\KGen(\msk, \bfy)$ results in $\sigma$. If yes, the game aborts.
Game $G_1$ is formally defined in~\Cref{fig:fasig-unf-g1-old}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_1$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X, \bfx) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\pp, \vk)$
\item 
$(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$
\item 
$t \getr \Z_p$, $\ct = \ipe.\Enc(\mpk, \bfx; t)$
\item 
$\pi \gets \nizk.\Prove(\pp, (X, \mpk, \ct), (\bfx, t))$
\item 
$\advt = (\mpk, \ct, \pi), \state = \msk$
\item 
$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\advt)$
\item 
$\bfy \getr \Z_p^\ell, \pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\widetilde{\sigma}, \bfy)$
\item 
{\color{blue} if $\sigma = \Adapt(\advt, \state,  \widetilde{\sigma}, \bfy, \bfx)$: abort}
\item 
return $((m \notin \mcal{Q}) \wedge \Verify(\vk, m, \sigma))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $\mcal{H}(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_1$}
\label{fig:fasig-unf-g1-old}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g1-old}
Let ${\sf Bad}_1$ be the event that $G_1$ aborts. 
If $R_{DL}$ is a hard relation and \ipe satisfies the special properties that 
``master public and secret keys satisfy discrete log relation'' and ``$\ipe.\KGen(\msk, \cdot)$ is a linear function in $\msk$'', then, $\Pr[{\sf Bad}_1] \leq \negl(\secparam)$.
\end{claim}

\begin{proof}
We prove the claim using a reduction to the hardness of the discrete log relation $R_{DL}$. 
More specifically, 
we show that if an adversary \A causes game $\G_1$ to abort, then, 
we can use it to construct a reduction \B that breaks 
the hardness of the discrete log relation $R_{DL}$. 
Let \C be the challenger for 
the hardness of the discrete log relation $R_{DL}$. 
Then, the reduction is as follows.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Reduction \B for proof of~\Cref{claim:fasig-unf-g1-old}.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X, \bfx) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\pp, \vk)$
\item 
{\color{blue}
Obtain discrete log challenge $\widetilde{Z} \gets \C(1^\secparam)$
}
\item 
{\color{blue}
$(\mpk', \msk') \gets \ipe.\Setup(\pp', 1^\ell)$. \\
Compute $\mpk = \widetilde{Z}^{\msk'}$. 
}
\item 
$t \getr \Z_p$, $\ct = \ipe.\Enc(\mpk, \bfx; t)$
\item 
$\pi \gets \nizk.\Prove(\pp, (X, \mpk, \ct), (\bfx, t))$
\item 
$\advt = (\mpk, \ct, \pi), \state = \msk$
\item 
$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\advt)$
\item 
$\bfy \getr \Z_p^\ell, \pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\widetilde{\sigma}, \bfy)$
\item 
{\color{blue} 
$\sk_\bfy := \as.\Ext(\widetilde{\sigma}, \sigma, \pk_\bfy)$ 
}
\item 
{\color{blue} 
if $(\pk_\bfy, \sk_\bfy) \notin R_{DL}$: $z' \getr \Z_p$, else, $z' = \sk_\bfy / \ipe.\KGen(\msk', \bfy)$.
}
% \nikhil{this works only if $\ipe.\KGen(\msk', \bfy) \neq 0$. For this reason, \A should not be allowed to choose $\bfy$, as otherwise it can always choose $\bfy = (0, \ldots, 0)$.}
\item 
Output $z'$.
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $\mcal{H}(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Reduction \B for proof of~\Cref{claim:fasig-unf-g1-old}}
\label{fig:fasig-unf-g1-old-proof-old}
\end{figure}

First, note that 
\ipe satisfies the special property that 
``master public and secret keys satisfy discrete log relation''. 
This means that $\mpk' = g^{\msk'}$ 
and thus $\mpk = \widetilde{Z}^{\msk'} = (g^{\widetilde{z}})^{\msk'} = g^{\widetilde{z} \cdot \msk'}$, 
where $\widetilde{z}$ is the witness (unknown to the reduction) of the 
statement $\widetilde{Z}$ w.r.t.\ discrete log relation $R_{DL}$.
Hence, it must be the case that the corresponding $\msk$ (also unknown to the reduction) should be $\msk = \widetilde{z} \cdot \msk'$. 

Next, observe that if \A causes game $G_1$ to abort, then, it must be the case that $\sigma = \Adapt(\advt, \state,  \widetilde{\sigma}, \bfy, \bfx)$. Then, by pre-signature correctness, it follows that $(\pk_\bfy, \sk_\bfy) \in R_{DL}$, where $\sk_\bfy := \as.\Ext(\widetilde{\sigma}, \sigma, \pk_\bfy)$. 
Recall that for any vector $\bfv$, $(\ipe.\PubKGen(\mpk, \bfv), \ipe.\KGen(\msk, \bfv)) \in R_{DL}$. 
% \nikhil{state this assumption about structure of \ipe}.
As $R_{DL}$ is a unique witness relation, it follows that $\sk_\bfy = \ipe.\KGen(\msk, \bfy)$.
Next, recall that $\ipe.\KGen$ is a linear function.
% \nikhil{state this assumption about structure of \ipe}. 
Then, applying this linearity to the equation $\msk = \widetilde{z} \cdot \msk'$, we get that $\ipe.\KGen(\msk, \bfy) = \widetilde{z} \cdot \ipe.\KGen(\msk', \bfy)$. Hence, it follows that $z' = \widetilde{z}$ as long as $\ipe.\KGen(\msk', \bfy) \neq 0$. The latter holds true with overwhelming probability as $\bfy \getr \Z_p^\ell$. Thus, \B breaks the the hardness of discrete log relation $R_{DL}$ in its game against \C.
\end{proof}

\paragraph{Game $G_2$:}
same as game $G_1$, except that 
the behaviour of $\mcal{O}_{\fpS}$ oracle is different.
In this game, $\mcal{O}_{\fpS}$ makes a copy of the list $H$ 
before executing the algorithm $\FPreSign$. 
Afterwards, it extracts the randomness $K$ used during the 
$\FPreSign$ algorithm, and checks if 
befroe the execution of the signing algorithm 
a query of the form $\vk||K||m$ or $\vk||K \cdot \pk_\bfy || m$ 
was made to $H$ by checking if $H'[\vk||K||m] \neq \bot$ or 
$H'[\vk||K \cdot \pk_\bfy ||m] \neq \bot$. If so, the game aborts.
Game $G_2$ is formally defined in~\Cref{fig:fasig-unf-g2-old}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_2$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X, \bfx) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\pp, \vk)$
\item 
$(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$
\item 
$t \getr \Z_p$, $\ct = \ipe.\Enc(\mpk, \bfx; t)$
\item 
$\pi \gets \nizk.\Prove(\pp, (X, \mpk, \ct), (\bfx, t))$
\item 
$\advt = (\mpk, \ct, \pi), \state = \msk$
\item 
$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\advt)$
\item 
$\bfy \getr \Z_p^\ell, \pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\widetilde{\sigma}, \bfy)$
\item 
if $\sigma = \Adapt(\advt, \state,  \widetilde{\sigma}, \bfy, \bfx)$: abort
\item 
return $((m \notin \mcal{Q}) \wedge \Verify(\vk, m, \sigma))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
{\color{blue} $H' = H$}
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
{\color{blue} 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
}
\item 
{\color{blue} 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
}
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $\mcal{H}(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_2$}
\label{fig:fasig-unf-g2-old}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g2-old}
Let ${\sf Bad}_2$ be the event that game $G_2$ aborts in $\mcal{O}_{\fpS}$. Then, $\Pr[{\sf Bad}_2] \leq \negl(\secparam)$.
\end{claim}
\begin{proof}
\nikhil{same as~\cite{asig}. fill details for completeness.}
\end{proof}

\paragraph{Game $G_3$:}
same as game $G_2$ except the behaviour of $\mcal{O}_{\fpS}$ oracle. 
Upon an $\mcal{O}_{\fpS}$ oracle query, the game produces a 
valid full signature $\widetilde{\sigma}$ and adjusts the global list $H$ as follows: 
It assigns the value stored at position 
$\vk || K || m$ to $H[\vk || K \cdot \pk_\bfy || m]$ and 
samples a fresh random value for $H[pk || K || m]$. 
These changes make the full signature  $\widetilde{\sigma}$ “look like” a pre-signature to the adversary, since upon querying the random oracle on $\vk || K \cdot \pk_\bfy || m$, \A obtains the value $H [\vk || K || m]$. 
Game $G_3$ is formally defined in~\Cref{fig:fasig-unf-g3-old}.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_3$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X, \bfx) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\pp, \vk)$
\item 
$(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$
\item 
$t \getr \Z_p$, $\ct = \ipe.\Enc(\mpk, \bfx; t)$
\item 
$\pi \gets \nizk.\Prove(\pp, (X, \mpk, \ct), (\bfx, t))$
\item 
$\advt = (\mpk, \ct, \pi), \state = \msk$
\item 
$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\advt)$
\item 
$\bfy \getr \Z_p^\ell, \pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||g^k \cdot \pk_\bfy||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\widetilde{\sigma}, \bfy)$
\item 
if $\sigma = \Adapt(\advt, \state,  \widetilde{\sigma}, \bfy, \bfx)$: abort
\item 
return $((m \notin \mcal{Q}) \wedge \Verify(\vk, m, \sigma))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$H' = H$
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk||{\color{blue}g^k}||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
\item 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
% \item 
% {\color{blue} 
% $\alpha = \vk || g^k || m$
% }
% \item 
% {\color{blue} 
% $\alpha' = \vk || g^k \cdot \pk_\bfy || m$
% }
\item 
{\color{blue} 
$H[\vk || g^k \cdot \pk_\bfy || m] = H[\vk || g^k || m]$
% $H[\alpha'] = H[\alpha]$
}
\item 
{\color{blue} 
$H[\vk || g^k || m] \getr \Z_p$
% $H[\alpha] \getr \Z_p$
}

\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $\mcal{H}(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_3$}
\label{fig:fasig-unf-g3-old}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g3-old}
$\Pr[G_2 = 1] = \Pr[G_3 = 1]$.
\end{claim}
\begin{proof}
The adversary can only notice the changes from $G_2$ to $G_3$, in case the random oracle has been previously queried on either $\vk || K || m$ or $\vk || K \cdot \pk_\bfy || m$. This case has been captured in the previous game $G_2$ and hence it holds that $\Pr[G_2 = 1] = \Pr[G_3 = 1]$.
\end{proof}

\paragraph{Game $G_4$:}
same as game $G_3$ except the pre-signature generated upon \A outputting the message $m$ is created by modifying a full signature to a pre-signature. 

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Game $G_4$.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
$(\sk, \vk) \gets \Sch.\KGen(\pp')$
\item 
$(X, \bfx) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\pp, \vk)$
\item 
$(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$
\item 
$t \getr \Z_p$, $\ct = \ipe.\Enc(\mpk, \bfx; t)$
\item 
$\pi \gets \nizk.\Prove(\pp, (X, \mpk, \ct), (\bfx, t))$
\item 
$\advt = (\mpk, \ct, \pi), \state = \msk$
\item 
$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\advt)$
\item 
$\bfy \getr \Z_p^\ell, \pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk|| {\color{blue} g^k} ||m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
{\color{blue} 
$\sk_\bfy = \ipe.\KGen(\msk, \bfy)$
}
\item 
$\widetilde{\sigma} = (r, {\color{blue}\widetilde{s} - \sk_\bfy})$
\item 
$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\widetilde{\sigma}, \bfy)$
\item 
if $\sigma = \Adapt(\advt, \state,  \widetilde{\sigma}, \bfy, \bfx)$: abort
\item 
return $((m \notin \mcal{Q}) \wedge \Verify(\vk, m, \sigma))$
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$\sigma \gets \Sch.\Sign(\sk, m)$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$H' = H$
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
$k \getr \Z_p$
\item 
$r:=\mcal{H}(\vk || g^k || m)$
\item 
$\widetilde{s}:= k + r \cdot \sk$
\item 
$\widetilde{\sigma} = (r, \widetilde{s})$
\item 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
\item 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
% \item 
% $\alpha = \vk || g^k || m$
% \item 
% $\alpha' = \vk || g^k \cdot \pk_\bfy || m$
\item 
$H[\vk || g^k \cdot \pk_\bfy || m] = H[\vk || g^k || m]$
% $H[\alpha'] = H[\alpha]$
\item 
$H[\vk || g^k || m] \getr \Z_p$
% $H[\alpha] \getr \Z_p$
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $\mcal{H}(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
$\ \ H[x] \getr \Z_p$
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Unforgeability Proof: Game $G_4$}
\label{fig:fasig-unf-g4-old}
\end{figure}

\begin{claim}
\label{claim:fasig-unf-g4-old}
$\Pr[G_3 = 1] = \Pr[G_4 = 1]$
\end{claim}
\begin{proof}
Since $k$ is chosen uniformly at random, the view of the adversary is identical in games $G_3$ and $G_4$. 
Hence, it follows that $\Pr[G_3 = 1] = \Pr[G_4 = 1]$.
\end{proof}

Having shown the transition form the original game $\faSigForge$ (game $G_0$) to game $G_4$ is indistinguishable, it remains to show that there exists a reduction \B that perfectly simulates $G_4$ and uses \A to win the strong unforgeability game against $\Sch$ challenger. We formally describe this claim and prove it next.

\begin{claim}
\label{claim:fasig-unf-last-old}
Suppose $\Sch$ is strongly unforgeable. 
Then, $\Pr[G_4 = 1] \leq \negl(\secparam)$.
\end{claim}
\begin{proof}
Let \C be the challenger for the strong unforgeability game of $\Sch$. Then reduction \B is as follows.

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
\begin{mdframed}
\begin{multicols}{2}
\paragraph{Reduction \B for proof of~\Cref{claim:fasig-unf-last-old}.} 
\begin{enumerate}[itemsep=0.1em]
\item 
$\mcal{Q} := \emptyset$
\item 
$H := [\bot]$
\item 
$\crs \gets \nizk.\Setup(1^\secparam)$
\item 
$\pp' \gets \ipfe.\Gen(1^\secparam)$
\item 
$\pp = (\crs, \pp')$
\item 
{\color{blue} 
$\vk \gets \C(1^\secparam)$
}
\item 
$(X, \bfx) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\pp, \vk)$
\item 
$(\mpk, \msk) \gets \ipe.\Setup(\pp', 1^\ell)$
\item 
$t \getr \Z_p$, $\ct = \ipe.\Enc(\mpk, \bfx; t)$
\item 
$\pi \gets \nizk.\Prove(\pp, (X, \mpk, \ct), (\bfx, t))$
\item 
$\advt = (\mpk, \ct, \pi), \state = \msk$
\item 
$m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\advt)$
\item 
$\bfy \getr \Z_p^\ell, \pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item 
{\color{blue} 
$\sigma' = (r, \widetilde{s}) \gets \mcal{O}_S^{Sch}(m)$
}
\item 
$\sk_\bfy = \ipe.\KGen(\msk, \bfy)$
\item 
$\widetilde{\sigma} = (r, \widetilde{s} - \sk_\bfy)$
\item 
$\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{\fpS}(\cdot, \cdot, \cdot), \mcal{H}(\cdot)}(\widetilde{\sigma}, \bfy)$
\item 
if $\sigma = {\color{blue} \sigma'}$: abort
\item 
{\color{blue} 
If $((m \in \mcal{Q}) \vee (\Verify(\vk, m, \sigma)=0))$: abort
}
\item 
{\color{blue} 
Output $(m, \sigma)$
}
\end{enumerate}

\vfill\null 
\columnbreak 

\paragraph{Oracle $\mcal{O}_S(m)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
{\color{blue}
$\sigma \gets \mcal{O}_S^{Sch}(m)$
}
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\sigma$
\end{enumerate}

\paragraph{Oracle $\mcal{O}_{\fpS}(m, X, \bfy)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
$H' = H$
\item 
$\pk_\bfy = \ipe.\PubKGen(\mpk, \bfy)$
\item
{\color{blue}
$\widetilde{\sigma} = (r, \widetilde{s}) \gets \mcal{O}_S^{Sch}(m)$
} 
\item 
$K = g^{\widetilde{s}} \cdot \vk^{-r}$
\item 
if $H'[\vk||K||m] \neq \bot$ or $H'[\vk||K \cdot \pk_\bfy || m] \neq \bot$: abort
% \item 
% $\alpha = \vk || g^k || m$
% \item 
% $\alpha' = \vk || g^k \cdot \pk_\bfy || m$
\item 
{\color{blue}
$H[\vk || g^k \cdot \pk_\bfy || m] = \mcal{H}^{Sch}(\vk || g^k || m)$
% $H[\alpha'] = \mcal{H}^{Sch}(\alpha)$
}
\item 
{\color{blue}
$H[\vk || g^k || m] = \mcal{H}^{Sch}(\vk || g^k \cdot \pk_\bfy || m)$
% $H[\alpha] = \mcal{H}^{Sch}(\alpha')$
}
\item 
$\mcal{Q} := \mcal{Q} \vee \{m\}$
\item 
return $\widetilde{\sigma}$
\end{enumerate}

\paragraph{Oracle $\mcal{H}(x)$.}
\begin{enumerate}[itemsep=0.1em]
\item 
if $H[x] = \bot:$
\item 
{\color{blue}
$\ \ H[x] \gets \mcal{H}^{Sch}(x)$
}
\item 
return $H[x]$
\end{enumerate}

\end{multicols}
\end{mdframed}
\caption{Reduction \B for proof of~\Cref{claim:fasig-unf-g4-old}.}
\label{fig:fasig-unf-g4-old-proof-old}
\end{figure}

From the description of reduction \B, we can observe that it differs from game $G_4$ only syntactically in some aspects. In particular, \B does not genate $\Sch$ signing and verification keys on its own and instead interacts with the challenger \C. This change also reflects in  how it replies to queries to each of the three oracles. Therefore, \B perfectly simulates game $G_4$. 

It remains to be shown that the forgery $\sigma$ output by the adversary \A can be used by the reduction \B to win the strong unforgeability game against the challenger \C. For this, we need to show that $(m, \sigma)$ has never been the output of oracle $\mcal{O}_S^{Sch}$. Note that \A has never made a query on the challenge message $m$ to either $\mcal{O}_S$ or $\mcal{O}_{\fpS}$. Hence, $\mcal{O}_S^{Sch}$ is only queried on $m$ in the challenge phase. As shown in game $G_1$, the adversary outputs a forgery $\sigma$ which is the same as $\sigma'$ only with negligible probability. Hence, $\mcal{O}_S^{Sch}$ has never output $\sigma$ on query $m$ before with overwhelming probability and consequently $(m, \sigma)$ constitutes a valid forgery for the strong unforgeability game against the challenger \C.
\end{proof}
Lastly, ~\Cref{lemma:fas-unf-old} follows from~\Cref{claim:fasig-unf-g1-old,claim:fasig-unf-g2-old,claim:fasig-unf-g3-old,claim:fasig-unf-g4-old,claim:fasig-unf-last-old}.
\end{proof}


==> ipe-construction.tex <==
\section{IPFE construction}
\subsection{ALS16 IPFE \nikhil{add cites}}
Let us recall the IPFE construction from ALS16 \nikhil{add cites}. Let $G$ be a group of prime order $q$ and let $g$ and $h$ be generators of $G$. Then, the construction is as follows.

\paragraph{$\KGen(1^\secparam, 1^n, G, q, g, h)$:}
\begin{itemize}
\item Sample $\bfs \getr \Z_q^n$ and $\bft \getr \Z_q^n$.
\item Output $\msk = (\bfs, \bft)$ and $\mpk = g^\bfs h^\bft$.
\end{itemize}

\paragraph{$\Enc(\mpk, \bfx \in \Z_q^n)$:}
\begin{itemize}
\item Sample $r \getr \Z_q$.
\item Compute $C = g^r, D = h^r$, and $\bfE = g^\bfx \cdot \mpk^r$.
\item Output $\ct = (C, D, \bfE)$.
\end{itemize}

\paragraph{$\KGen(\msk, \bfy \in \Z_q^n)$:}
Output $\sk_\bfy = (\bfy, \bfs^T\bfy, \bft^T\bfy)$

\paragraph{$\Dec(\mpk, \sk_\bfy, \ct)$:}
Compute $v:= \bfE^\bfy / (C^{\bfs^T\bfy} \cdot D^{ \bft^T\bfy})$ and output its discrete log.

\begin{fact}[ALS16]
The above construction is a IND-secure IPFE scheme under the DDH assumption.
\end{fact}

\begin{fact}[Wee16]
The above construction is a semi-adaptive simulation secure IPFE scheme under the DDH assumption.
\end{fact}


==> more_prelims.tex <==
\section{More Preliminaries}\label{sec:more-prelims}

\smallskip\noindent\textbf{Notations.}
Suppose $\G$ is a cyclic group of prime-order $p$ and with generator $g$. 
For a scalar $x \in \Z_p$,
$g^x$ denotes its group encoding. 
For a vector $\bfx = (x_1, \ldots, x_n)^T \in \Z_p^n$, 
$g^\bfx$ denotes its group encoding $(g^{x_1}, \ldots, g^{x_n})^T$.
% \pnote{why is there a transpose operation here?}
% \nikhil{transpose operation because it is written like a row vector.}
Similarly, for a matrix $\bfX$, $g^\bfX$ denotes its group encoding.
Given group encoding of a vector $g^\bfx$ and a vector $\bfy$, we can compute $g^{\bfx^T\bfy}$ efficiently as $g^{\bfx^T\bfy} = \Pi_{i \in [n]} (g^{x_i})^{y_i}$. 

\subsection{Hard Relation}

\begin{definition}[Hardness of $R$]
We say that a relation $R$ is hard, if 
(i) there exists a \ppt sampling algorithm $\GenR(1^\secparam)$ that 
outputs a statement/witness pair $(X, x) \in R$,
(ii) the relation is poly-time decidable,
(iii) for every non-uniform PPT adversary $\A$, there exists a negligible function $\negl$ such that for all $\secparam \in \N$,
\begin{equation}
\Pr[\mathsf{G}_{\A,R}( 1^\secparam) = 1] \le \negl(\secparam) \ ,
\end{equation}
where the game $\mathsf{G}_{\A,R}( 1^\secparam)$ is defined as follows:

\begin{pchstack}[boxed, center, space=1em]
\procedure[linenumbering, mode=text]{Game $\mathsf{G}_{\A,R}( 1^\secparam)$}{
$(X,x) \gets \GenR(1^\secparam)$
\\ 
$(x') \gets \A(1^\secparam, X)$
\\ 
If $(X, x') \in R$: \ret $1$
\\ 
\ret $0$	
}
\end{pchstack}

\end{definition}


\begin{definition}[Hardness of $R$ w.r.t.\ function class $\mcal{F}$]
\label{def:f-hard-relation}
We say that a relation $R$ is $\mcal{F}$-hard, if 
(i) there exists a \ppt sampling algorithm $\GenR(1^\secparam)$ that 
outputs a statement/witness pair $(X, x) \in R$,
(ii) for every non-uniform PPT adversary $\A$ there exists a negligible function $\negl$ such that for all $\secparam \in \N$,
\begin{equation}
\Pr[\mathsf{G}_{\A,R, \mcal{F}}( 1^\secparam) = 1] \le \negl(\secparam) \ ,
\end{equation}
where the game $\mathsf{G}_{\A,R, \mcal{F}}( 1^\secparam)$ is defined as follows:
% \pnote{If simpler, we should define hardness w.r.t.\ on linear functions}

\begin{pchstack}[boxed, center, space=1em]
\procedure[linenumbering, mode=text]{Game $\mathsf{G}_{\A,R, \mcal{F}}( 1^\lambda)$}{
$(X,x) \gets \GenR(1^\lambda)$ 
% \pcskipln \\ \nikhil{can we assume that $\GenR$ outputs all witnesses $x$ for $X$?}
\\ 
$(f,z) \gets \A(1^\lambda, X)$
\\ 
If $(f \in \mcal{F}) \wedge \left (z \in \{f(x') : \exists \ x' \text{ such that } (X,x') \in R \} \right )$: \ret $1$
% \pcskipln \\ \pnote{$A$ wins even if $A$ can learn $f(x')$ for another witness $x'$}
\\ 
\ret $0$	
}
\end{pchstack}
\end{definition}

We note that in the above definition we allow the adversary \A to choose $f$ adaptively as this hardness assumption will later be used in proving unforgeability of our functional adaptor signatures construction where the adversary is allowed to choose the challenge function adaptively. This is necessary as functional adaptor signatures are non-trivial to build only in such a setting and become trivial if the challenge function is selectively chosen upfront by the adversary. Further note that we let the adversary \A win even if \A outputs a function evaluation of a witness $x'$ of $X$ that is different from $x$.
% \pnote{Why we allow $A$ to choose $f$ adaptively, and that we let $A$ win even if $A$ learns a function of another witness.}

\begin{definition}[Hard Relation $R_\DL$]
\label{def:dl-relation}
The discrete log language $L_\DL$ is defined with respect 
to a group $G$ with generator $g$ and order $p$ as  
$L_\DL := \{ \ X \ | \ \exists \ x \in  \Z_p, X = g^x \ \}$ 
with the corresponding hard relation $R_\DL = \{ \ (X, x) \ | \ X = g^{x}\ \}$.
\end{definition}

\ignore{
	
		\begin{definition}[Hard Relation $R_\DLstar$]
		The language  $L_\DLstar$ is related to the discrete log language $L_\DL$. It is defined with respect 
		to a group $G$ with generators $g_1, g_2$ and order $p$ as 
		$L_\DLstar := \{ \ X \ | \ \exists \ (x_1,x_2) \in  \Z_p^2, X = g_1^{x_1} \cdot g_2^{x_2} \ \}$ 
		with the corresponding hard relation 
		$R_\DLstar := \{ \ (X, (x_1, x_2)) \ | \ X = g_1^{x_1} \cdot g_2^{x_2} \ \}$.
		\nikhil{there can be multiple witnesses for the statement X. We want the hardness relation to be satisfied only when ``the'' witness is used and not just any witness. Update the hardness relation to reflect this.}
		\end{definition}

		\begin{lemma}
		If $R_\DL$ is a hard relation, then, $R_\DLstar$ is a hard relation.
		\end{lemma}
		\begin{proof}
		Suppose there is a \ppt adversary \A that can break the hardness of the relation $R_\DLstar$. Then, we show how to use it to construct a \ppt reduction \B that can break the hardness of the relation $R_\DL$. This should complete the proof. The reduction \B is as follows.

		The reduction \B obtains as input $(\G, g_1, p, g_1^{x_1})$ from the challenger \C for the relation $R_\DL$. It samples $a \getr \Z_p$, computes the generator $g_2 = g_1^a$, samples $x_2 \getr \Z_p$ and computes $h := (g_1^{x_1}) \cdot g_2^{x_2}$. The reduction \B sends the challenge $(\G, g_1, g_2, p, h)$ to the adversary \A and obtains $(x'_1, x'_2)$ as the response. Then, the reduction computes $x_1 := x'_1 + a (x'_2 - x_2)$ and sends back $x_1$ to the challenger \C.

		Observe that if \A breaks the hardness of $R_\DLstar$, then, it must be the case that $h = g_1^{x'_1} \cdot g_2^{x'_2}$. Therefore we obtain that $g_1^{x_1 + a x_2} = g_1^{x'_1 + a x'_2}$. Thus, it follows that $x_1 = x'_1 + a (x'_2 - x_2)$ and hence, \B breaks the hardness of $R_\DL$.


		\end{proof}

		\begin{definition}[Hard Relation $R_\DLstar$]
		The language  $L_\DLstar$ is related to the discrete log language $L_\DL$. It is defined with respect 
		to a group $G$ with generator $g$, order $p$ and an exponent $a \in \Z_p$ as 
		$L_\DLstar := \{ \ X \ | \ \exists \ (x_1,x_2) \in  \Z_p^2, X = g^{x_1 + a \cdot x_2}\ \}$ 
		with the corresponding hard relation 
		$R_\DLstar := \{ \ (X, (x_1, x_2)) \ | \ X = g^{x_1 + a \cdot x_2} \ \}$.
		\nikhil{there can be multiple witnesses for the statement X. We want the hardness relation to be satisfied only when ``the'' witness is used and not just any witness. Update the hardness relation to reflect this.}
		\end{definition}

		\begin{lemma}
		If $R_\DL$ is a hard relation, then, $R_\DLstar$ is a hard relation.
		\end{lemma}
		\begin{proof}
		Suppose there is a \ppt adversary \A that can break the hardness of the relation $R_\DLstar$. Then, we show how to use it to construct a \ppt reduction \B that can break the hardness of the relation $R_\DL$. This should complete the proof. The reduction \B is as follows.

		The reduction \B obtains as input $(\G, g, p, g^{x_1})$ from the challenger \C for the relation $R_\DL$. It samples $a \getr \Z_p$, $x_2 \getr \Z_p$ and computes $h := (g^{x_1}) \cdot g^{a \cdot x_2}$. The reduction \B sends the challenge $(\G, g, p, a, h)$ to the adversary \A and obtains $(x'_1, x'_2)$ as the response. Then, the reduction computes $x_1 := x'_1 + a (x'_2 - x_2)$ and sends back $x_1$ to the challenger \C.

		Observe that if \A breaks the hardness of $R_\DLstar$, then, it must be the case that $h = g^{x'_1 + a \cdot x'_2}$. Therefore we obtain that $g^{x_1 + a \cdot x_2} = g^{x'_1 + a \cdot x'_2}$. Thus, it follows that $x_1 = x'_1 + a (x'_2 - x_2)$ and hence, \B breaks the hardness of $R_\DL$.


		\end{proof}
}


\subsection{Adaptor Signatures}



\begin{definition}
An adaptor signature scheme 
$\AS_{\DS, R, R'} := (\PreSign, $ $\PreVerify, \Adapt, \Ext)$ 
is defined with respect to a signature scheme $\DS = (\KGen, \Sign, \Verify)$ 
and hard relations $R$ and $R'$ such that $R \subseteq R'$.
Here, $R$ constitutes the relation for the statement-witness pairs generated by $\GenR$ and $R'$ is an extended relation that defines the relation for {\em extracted} witnesses. 
The interfaces are described below.
% \anote{Can we put all interface definitions under definition environment?}


\begin{itemize}[leftmargin=*]
% \item 
% $(\sk, \vk) \gets \KGen(1^\secparam)$:
% The key generation algorithm takes as input the security parameter $1^\secparam$ 
% and outputs a signing key $\sk$ and a verification key $\vk$. 
% This algorithm is the same as in $\DS$. 

\item 
$\widetilde{\sigma} \gets \PreSign(\sk,m,X)$:
The pre-signing algorithm takes as input
a signing key $\sk$,
a message $m$, 
and a statement $X$ for the language $L_R$, 
and outputs a pre-signature $\widetilde{\sigma}$
(we sometimes also refer to this as a partial signature). 

\item 
$0/1 \gets \PreVerify(\vk, m, X, \widetilde{\sigma})$: 
The pre-signature verification algorithm takes as input 
a verification key $\vk$, 
a message $m$, 
a statement $X$ for the language $L_R$, 
and a pre-signature $\widetilde{\sigma}$,
and outputs $0/1$ signifying whether $\widetilde{\sigma}$ 
is correctly generated. 

\item 
$\sigma := \Adapt(\vk, m, X, x, \widetilde{\sigma})$: 
The adapt algorithm transforms 
a pre-signature $\widetilde{\sigma}$ into a valid signature $\sigma$
given the witness $x$ for the instance $X$ of the language $L_R$. 

% \item 
% $\sigma \gets \Sign(\sk, m)$: 
% The signing algorithm takes as input 
% a signing key $\sk$, 
% and a message $m$, 
% and outputs a signature $\sigma$. 
% This algorithm is the same as in $\DS$.

% \item 
% $0/1 \gets \Verify(\vk, m, \sigma)$: 
% The verification algorithm takes as input 
% a verification key $\vk$, 
% a message $m$, 
% and a signature $\sigma$, 
% and outputs $0/1$ signifying whether $\sigma$ 
% is correctly generated. 
% This algorithm is the same as in $\DS$. 

\item 
$x := \Ext(\widetilde{\sigma}, \sigma, X)$: 
The extract algorithm takes as input 
a pre-signature $\widetilde{\sigma}$, 
a signature $\sigma$, 
and an instance $X$, 
and outputs a witness $x'$ such that $(X, x') \in R'$, or $\bot$. 
% This can be formalized as correctness.

\end{itemize}

\end{definition}

Note that an adaptor signature scheme $\AS_{\DS, R, R'}$ also inherits $\KGen, \Sign, \Verify$ algorithms from the signature scheme $\DS$.

Typically, an adaptor signature is run between a buyer and a seller. 
The buyer runs $\KGen, \Sign, \PreSign, \Ext$ algorithms, 
the seller runs $\Adapt$ algorithm, and anyone can run $\PreVerify, \Verify$ algorithms.

\begin{remark}
Looking ahead, in the discrete-log based instantiation, we will have $R'=R$, but in the lattice-based instantiation, we will have $R' \neq R$ and the reason for this extension is the {\em knowledge/soundness gap} inherent in {\em efficient} lattice-based zero-knowledge proofs. 
% \nikhil{explain this more}
\end{remark}

\begin{definition}[Correctness]
\label{def:as-correctness}
% \nikhil{rename to correctness}
An adaptor signature scheme 
$\AS$ satisfies correctness if for every 
$n \in \N$, every message $m \in \{0,1\}^*$, 
and every statement/witness pair $(X, x) \in R$, the following holds:

\[
\Pr \left[
\begin{array}{c}
\PreVerify(\vk, m, X, \widetilde{\sigma}) = 1 \\ 
\wedge \ 
\Verify(\vk, m, \sigma) = 1 \\
\wedge \ 
(X, x') \in R'
\end{array}
:
\begin{array}{l}
(\sk, \vk) \gets \KGen(1^\secparam) \\
\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
\sigma := \Adapt(\vk, m, X, x, \widetilde{\sigma}) \\ 
x' := \Ext(\widetilde{\sigma}, \sigma, X)
\end{array}
\right] = 1
\]


\end{definition}

In terms of security, we want witness extractability against a malicious seller and weak pre-signature adaptability against a malicious seller. We explain these next.

\ignore{

		\begin{definition}[Unforgeability]
		An adaptor signature scheme $\AS$ is aEUF-CMA secure if 
		for every \ppt adversary \A there exists a negligible function $\negl$ such that
		for all $\secparam \in \N$,
		\[
		\Pr[ \aSigForge_{\A,\AS}(1^\secparam) = 1] \leq \negl(\secparam),
		\]
		where the experiment $\aSigForge_{\A,\AS}$ 
		is defined as in~\Cref{fig:asig-unf-exp}.

		\end{definition}

		\begin{figure}[H]
		\centering
		\captionsetup{justification=centering}
		\begin{pchstack}[boxed, space=1em]
		\begin{pcvstack}[space=1em]
		\procedure[linenumbering]{Experiment $\aSigForge_{\A,\AS}$.}{
		\mcal{Q} := \emptyset \\
		(\sk, \vk) \gets \KGen(1^\secparam) \\ 
		m \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{pS}(\cdot, \cdot)}(\vk) \\ 
		(X, x) \gets \GenR(1^\secparam) \\ 
		\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
		\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{pS}(\cdot, \cdot)}(\widetilde{\sigma}, X) \\ 
		\text{\ret \ } ((m \notin \mcal{Q}) \wedge \Verify(\vk, m, \sigma))
		} 

		\end{pcvstack}
		\begin{pcvstack}[space=1em]

		\procedure[linenumbering]{Oracle $\mcal{O}_S(m)$}{
		\sigma \gets \Sign(\sk, m) \\ 
		\mcal{Q} := \mcal{Q} \vee \{m\} \\ 
		\text{\ret \ } \sigma
		}

		\procedure[linenumbering]{Oracle $\mcal{O}_{pS}(m, X)$}{
		\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
		\mcal{Q} := \mcal{Q} \vee \{m\} \\ 
		\text{\ret \ } \widetilde{\sigma}
		}
		\end{pcvstack}

		\end{pchstack}
		\caption{Unforgeability experiment of adaptor signatures}
		\label{fig:asig-unf-exp}
		\end{figure}
}


Witness extractability requires that for an honestly generated pre-signature and a valid signature, one should be able to extract a witness. Intuitively, it tries to capture that an interaction between an honest buyer (i.e., generates valid pre-signature) and a malicious seller trying to get paid (i.e., adapt pre-signature into a valid signature) without revealing a witness (i.e., extraction failure) should be unlikely to occur.

\begin{definition}[Witness Extractability]
\label{def:as-wit-ext}
An adaptor signature scheme $\AS$ is witness extractable if for every PPT adversary \A, there exists a negligible function $\negl$ such that
for all $\secparam \in \N$,
\[
\Pr[ \aWitExt_{\A, \AS}(1^\secparam) = 1] \leq \negl(\secparam),
\]
where the experiment $\aWitExt_{\A, \AS}$ is defined as in~\Cref{fig:asig-wit-ext-exp}.
\end{definition}

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
% \fbox{
\begin{pcvstack}[boxed, space=1em]
\begin{pchstack}[space=1em]
\procedure[linenumbering]{Experiment $\aWitExt_{\A,\AS}$.}{
\mcal{Q} := \emptyset \\
(\sk, \vk) \gets \KGen(1^\secparam) \\ 
(m, X) \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{pS}(\cdot, \cdot)}(\vk) \\ 
\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
\sigma \gets \A^{\mcal{O}_S(\cdot), \mcal{O}_{pS}(\cdot, \cdot)}(\widetilde{\sigma}) \\ 
x' := \Ext(\widetilde{\sigma}, \sigma, X) \\ 
\text{\ret \ } ((m \notin \mcal{Q}) \wedge ((X, x') \notin R') \wedge \Verify(\vk, m, \sigma))
}
\end{pchstack}
\begin{pchstack}[space=1em]
\procedure[linenumbering]{Oracle $\mcal{O}_S(m)$}{
\sigma \gets \Sign(\sk, m) \\ 
\mcal{Q} := \mcal{Q} \vee \{m\} \\ 
\text{\ret \ } \sigma
}

\procedure[linenumbering]{Oracle $\mcal{O}_{pS}(m, X)$}{
\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
\mcal{Q} := \mcal{Q} \vee \{m\} \\ 
\text{\ret \ } \widetilde{\sigma}
}
\end{pchstack}
\end{pcvstack}
% }
\caption{Witness Extractability experiment of adaptor signatures}
\label{fig:asig-wit-ext-exp}
\end{figure}

Note that, in the above witness extractability definition, the adversary's winning condition is restricted to the extracted witness not being in $R'$.
Since $R \subseteq R'$, $(X, x') \notin R'$ implies $(X, x') \notin R$. Therefore, it is sufficient to ensure that $R'$ is a hard relation, which itself implies that $R$ is also a hard relation. As a result, in our security assumptions, we make sure that $R'$ is a hard relation. 

Weak pre-signature adaptability requires that given a valid pre-signature and a witness for the instance, 
one can always adapt the pre-signature into a valid signature.
Intuitively, this tries to capture that it should be impossible for a malicious buyer to learn the witness without doing the payment. 

\begin{definition}[Weak Pre-signature Adaptability]
\label{def:as-pre-sig-adaptability}
An adaptor signature scheme $\AS$ satisfies weak pre-signature adaptability 
if for any $\secparam \in \N$, 
any message $m \in \{0,1\}^*$, 
any key pair $(\sk, \vk) \gets \KGen(1^\secparam)$, 
any statement/witness pair $(X, x) \in R$, 
and any pre-signature $\widetilde{\sigma} \in \{0,1\}^*$ 
with $\PreVerify(\vk, m, X, \widetilde{\sigma}) = 1$, we have:
\[
\Pr[\Verify(\vk, m, \Adapt(\vk, m, X, x, \widetilde{\sigma})) = 1] = 1.
\]
\end{definition}

Note that the above pre-signature adaptability is called {\em weak} because only statement-witness pairs satisfying $R$ are guaranteed to be adaptable, and not those satisfying $R'$. Therefore, weak pre-signature adaptability does not guarantee, for example, that an {\em extracted} witness can be used to adapt a pre-signature successfully. This is however guaranteed whenever $R=R'$.

We have several constructions of adaptor signatures compatible with ECDSA~\cite{asig}, lattice-based signatures~\cite{pq-as,albrecht2022lattice}, and dichotomic signature schemes~\cite{as-foundations} which is a recently introduced abstraction that captures many popular schemes like Schnorr, CL, BBS, etc. The group-based schemes are constructed w.r.t.\ the discrete logarithm NP language in the respective groups, while the lattice-based schemes are constructed w.r.t.\ the SIS NP language.


\ignore {
	
		In terms of security, we want extractability and unique extractability against a malicious seller, weak pre-signature adaptability and pre-verify soundness against a malicious buyer, and unlinkability against a malicious observer. We explain these next.

		Extractability, proposed by Dai, Okamoto, and Yamamoto~\cite{as-stronger}, combines and extends the security properties of witness extractability and adaptor unforgeability (as described in~\cite{asig}) to the so-called multiple query setting. In partic- ular, the adversary is allowed to see multiple pre-signatures on the challenge message as well as pre-signatures on multiple honestly sampled statements. In contrast, in prior definitions, the adversary was restricted to seeing only one pre-signature on the challenge message and an honestly sampled statement. In the multiple query setting, the adversary’s task is to output a special forgery $(m^*, \sigma^*)$ for which $\sigma^*$ cannot be used to successfully extract a witness (breaking extractability). We formally state the definition below:

		\begin{definition}[Extractability]
		An adaptor signature scheme $\AS$ is extractable if for every \ppt adversary \A, there exists a negligible function $\negl$ such that
		for all $\secparam \in \N$,
		\[
		\Pr[ \aExt_{\A, \AS}(1^\secparam) = 1] \leq \negl(\secparam),
		\]
		where the experiment $\aExt_{\A, \AS}$ is defined as in~\Cref{fig:asig-ext-exp} and the probability is taken over the random choices of all probabilistic algorithms.
		\end{definition}

		\begin{figure}[H]
		\centering
		\captionsetup{justification=centering}
		\begin{pcvstack}[boxed, space=1em]
		\procedure[linenumbering,mode=text]{Experiment $\aExt_{\A,\AS}$.}{
		$(\sk, \vk) \gets \KGen(1^\secparam)$; $b=1$;
		$\mcal{S}, \mcal{C}, \mcal{T} := \emptyset$ \\
		$(m^*, \sigma^*) \gets \A^{\mcal{O}_{\sf NewX}(\cdot),\mcal{O}_{\sf S}(\cdot), \mcal{O}_{\sf pS}(\cdot, \cdot)}(\vk)$ \\ 
		If $\Verify(\vk, m^*, \sigma^*) = 0$: $b=0$ \\
		If $m^* \notin \mcal{S}$: $b=0$\\ 
		For $(X, \widetilde{\sigma})\in \mcal{T}[m^*]$ s.t.\ $X \notin \mcal{C}$: \\ 
		\quad If $(X, \Ext(\widetilde{\sigma}, \sigma, X)) \in R'$: $b=0$ \\ 
		\ret $b$
		}

		\procedure[linenumbering,mode=text]{Oracle $\mcal{O}_{\sf NewX}(1^\secparam)$.}{
		$(X, x) \gets R.\GenR(1^\secparam)$; $\mcal{C} := \mcal{C} \cup \{X\}$; \ret $X$	
		}
		\begin{pchstack}[space=1em]
		\procedure[linenumbering]{Oracle $\mcal{O}_{\sf S}(m)$}{
		\sigma \gets \Sign(\sk, m) \\ 
		\mcal{S} := \mcal{S} \cup \{m\} \\ 
		\text{\ret \ } \sigma
		}

		\procedure[linenumbering]{Oracle $\mcal{O}_{\sf pS}(m, X)$}{
		\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
		\mcal{T}[m] := \mcal{T}[n] \cup \{(X, \widetilde{\sigma})\} \\ 
		\text{\ret \ } \widetilde{\sigma}
		}
		\end{pchstack}
		\end{pcvstack}
		\caption{Extractability of adaptor signatures}
		\label{fig:asig-ext-exp}
		\end{figure}

		\begin{remark}
		The above extractability definition generalizes extractability as defined in~\cite{as-stronger,as-foundations} in the following way: the adversary's winning condition is restricted to the extracted witness not being in $R'$.
		Since $R \subseteq R'$, $(X, x') \notin R'$ implies $(X, x') \notin R$. Therefore, it is sufficient to ensure that $R'$ is a hard relation, which itself implies that $R$ is also a hard relation. As a result, in our security assumptions, we make sure that $R'$ is a hard relation. 
		\end{remark}

		Next, we describe unique extractability. 
		Unique extractability guarantees that any verifying pre-signature can be viewed as a commitment to both a single valid signature and a single witness. This means that no efficient adversary can compute a pre-signature $\widetilde{\sigma}$ on a message $m$ and a statement $X$ , such that there exist two different signatures on $m$ that both extract to a valid witness with $\widetilde{\sigma}$. More formally:

		\begin{definition}[Unique Extractability]
		An adaptor signature scheme $\AS$ is unique extractable if for every \ppt adversary \A, there exists a negligible function $\negl$ such that
		for all $\secparam \in \N$,
		\[
		\Pr[ \aUniqueExt_{\A, \AS}(1^\secparam) = 1] \leq \negl(\secparam),
		\]
		where the experiment $\aUniqueExt_{\A, \AS}$ is defined as in~\Cref{fig:asig-unique-ext-exp} and the probability is taken over the random choices of all probabilistic algorithms.
		\end{definition}

		\begin{figure}[H]
		\centering
		\captionsetup{justification=centering}
		\begin{pcvstack}[boxed, space=1em]
		\procedure[linenumbering,mode=text]{Experiment $\aUniqueExt_{\A,\AS}$.}{
		$(\sk, \vk) \gets \KGen(1^\secparam)$; $b=1$ \\
		$(m, X, \widetilde{\sigma}, \sigma, \sigma') \gets \A^{\mcal{O}_{\sf S}(\cdot), \mcal{O}_{\sf pS}(\cdot, \cdot)}(\vk)$ \\ 
		If $(\sigma=\sigma') \cup (\Verify(\vk, m, \sigma) = 0) \cup (\Verify(\vk, m, \sigma') = 0)$: $b=0$ \\
		If $\PreVerify(\vk, m, X, \widetilde{\sigma}) = 0$: $b=0$\\ 
		$x = \Ext(\widetilde{\sigma}, \sigma, X)$, 
		$x' = \Ext(\widetilde{\sigma}, \sigma', X)$ \\
		If $((X, x) \notin R') \cup ((X, x') \notin R')$: $b=0$\\
		\ret $b$
		}

		\begin{pchstack}[space=1em]
		\procedure[linenumbering]{Oracle $\mcal{O}_{\sf S}(m)$}{
		\sigma \gets \Sign(\sk, m) \\ 
		\text{\ret \ } \sigma
		}

		\procedure[linenumbering]{Oracle $\mcal{O}_{\sf pS}(m, X)$}{
		\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
		\text{\ret \ } \widetilde{\sigma}
		}
		\end{pchstack}
		\end{pcvstack}
		\caption{Unique Extractability of adaptor signatures}
		\label{fig:asig-unique-ext-exp}
		\end{figure}

		\begin{remark}
		The above unique extractability definition is a weakening of unique extractability as defined in~\cite{as-stronger,as-foundations} in the following way: the adversary's winning condition is restricted to the extracted witnesses being in $R'$.
		Since $R \subseteq R'$, $(X, x') \in R'$ does not necessarily imply $(X, x') \in R$ and hence this definition is weaker. Note that it is not a weakening if $R=R'$ (which is the typical case for non-lattice based constructions). 
		\end{remark}

		Next, we describe weak pre-signature adaptability. 
		It requires that given a valid pre-signature and a witness for an honestly generated the instance, 
		one can always adapt the pre-signature into a valid signature.

		\begin{definition}[Weak Pre-signature Adaptability]
		An adaptor signature scheme $\AS$ satisfies weak pre-signature adaptability 
		if for any $\secparam \in \N$, 
		any message $m \in \{0,1\}^*$, 
		any key pair $(\sk, \vk) \gets \KGen(1^\secparam)$, 
		any statement/witness pair $(X, x) \in R$, 
		and any pre-signature $\widetilde{\sigma} \in \{0,1\}^*$ 
		with $\PreVerify(\vk, m, X, \widetilde{\sigma}) = 1$, we have:
		\[
		\Pr[\Verify(\vk, m, \Adapt(\vk, m, X, x, \widetilde{\sigma})) = 1] = 1.
		\]
		\end{definition}

		Note that the above pre-signature adaptability is called {\em weak} because only statement-witness pairs satisfying $R$ are guaranteed to be adaptable, and not those satisfying $R'$. Therefore, it weak pre-signature adaptability does not guarantee, for example, that an {\em extracted} witness can be used to adapt a pre-signature successfully. This is however guaranteed whenever $R=R'$.

		Next, we describe pre-verify soundness. It was introduced by~\cite{as-foundations} and it ensures that the pre-verification algorithm satisfies computational soundness w.r.t.\ the relation $R$. In particular, $\PreVerify$ should reject pre-signatures computed using statements $X \notin R$. Intuitively, pre-verify soundness ensures that every valid pre-signature can be adapted to a full signature and one can extract a witness from it. This strengthens the property of weak pre-signature adaptability which is restricted to honestly generated pre-signatures on statements in the relation. 

		\begin{definition}[Pre-verify Soundness]
		An adaptor signature scheme $\AS$ satisfies computational pre-verify soundness if for every \ppt adversary \A, there exists a negligible function $\negl$ such that for every $\secparam \in \N$ and polynomially-bounded $X \notin L_R$,

		\[
		\Pr\left[ 
		\PreVerify(\vk, m, X, \widetilde{\sigma}) = 1: 
		\begin{matrix}
		(\sk, \vk) \gets \KGen(1^\secparam) \\ 
		(m, \widetilde{\sigma}) \gets \A(\sk)
		\end{matrix}
		\right] \leq \negl(\secparam)
		\]
		\end{definition}

		Next, we describe unlinkability.
		It was introduced by~\cite{as-foundations} and
		it guarantees that an adversary cannot distinguish standard signa- tures from adapted pre-signatures, even when the pre-signatures are adapted using adversarially generated witnesses.

		\begin{definition}[Unlinkability]
		An adaptor signature scheme $\AS$ is unlinkable if for every \ppt adversary \A, there exists a negligible function $\negl$ such that for every $\secparam \in \N$,

		\[ 
		\mid \Pr[\aUnlink_{\A, \AS}^0 (1^\secparam) = 1] - 
		\Pr[\aUnlink_{\A, \AS}^1 (1^\secparam) = 1] \mid 
		\leq \negl(\secparam),
		\]

		where experiment $\aUnlink_{\A, \AS}^b$ for $b \in \{0,1\}$ is described in~\Cref{fig:asig-unlink-exp}, and the probability is
		taken over the random choices of all probabilistic algorithms.
		\end{definition}

		\begin{figure}[H]
		\centering
		\captionsetup{justification=centering}
		\begin{pcvstack}[boxed, space=1em]
		\procedure[linenumbering,mode=text]{Experiment $\aUnlink_{\A,\AS}^b$.}{
		$(\sk, \vk) \gets \KGen(1^\secparam)$\\
		$b' \gets \A^{\mcal{O}_{\sf Chal}(\cdot, \cdot), \mcal{O}_{\sf pS}(\cdot, \cdot)}(\vk)$ \\ 
		\ret $b'$
		}

		\procedure[linenumbering,mode=text]{Oracle $\mcal{O}_{\sf Chal}(m, (X, x))$}{
		If $(X, x) \notin R$: \ret $\bot$\\ 
		$\widetilde{\sigma} \gets \PreSign(\sk, m, X)$ \\ 
		$\sigma_0 := \Adapt(\vk, m, X, x, \widetilde{\sigma})$ \\
		$\sigma_1 \gets \Sign(\sk, m)$ \\ 
		\ret  $\sigma_b$
		}

		\begin{pchstack}[space=1em]
		\procedure[linenumbering]{Oracle $\mcal{O}_{\sf S}(m)$}{
		\sigma \gets \Sign(\sk, m) \\ 
		\text{\ret \ } \sigma
		}

		\procedure[linenumbering]{Oracle $\mcal{O}_{\sf pS}(m, X)$}{
		\widetilde{\sigma} \gets \PreSign(\sk, m, X) \\ 
		\text{\ret \ } \widetilde{\sigma}
		}
		\end{pchstack}
		\end{pcvstack}
		\caption{Unlinkability of adaptor signatures}
		\label{fig:asig-unlink-exp}
		\end{figure}
}

\subsection{Non-Interactive Zero-Knowledge Arguments}\label{sec:nizk}

\begin{definition}[Secure NIZK Argument System]
\label{def:nizk}
A $\NIZK$ for language $L_R$ in the CRS model consists of the following possibly randomized algorithms.

\begin{itemize}[itemsep=1pt,leftmargin=*]
\item 
$\crs \gets \Setup(1^\secparam)$:
it takes in a security parameter $\secparam$ 
and outputs the common reference string $\crs$ which is publicly known to everyone.

\item 
$\pi \gets \Prove(\crs, \stmt, \wit)$:
it takes in the common reference string $\crs$, 
a statement $\stmt$, 
and a witness $\wit$, 
outputs a proof $\pi$.

\item 
$0/1 \gets \Verify(\crs, \stmt, \pi)$:
it takes in the common reference string $\crs$, 
a statement $\stmt$, 
and a proof $\pi$, 
and either accepts (with output $1$) the proof, or rejects (with output $0$) it.
\end{itemize}
A secure $\nizk$ argument system must satisfy the following properties:
\begin{itemize}[itemsep=1pt,leftmargin=*]
\item 
{\bf Completeness:}
For all $\stmt, \wit$ where $R(\stmt, \wit) = 1$, 
if $\crs \gets \Setup(1^\secparam)$ and 
$\pi \gets \Prove(\crs, \stmt, \wit)$, then, 
\[
\Pr[\Verify(\crs, \stmt, \pi) = 1] = 1.
\]
\item 
% \pnote{why are we defining statistical soundness?}
{\bf Adaptive Soundness:}
For all non-uniform \ppt provers $\mcal{P}^*$, 
there exists a negligible function $\negl$ such that 
for all $\secparam \in \N$,
if $\crs \gets \Setup(1^\secparam)$ and 
$(\stmt, \pi) \gets \mcal{P}^*(\crs)$, then,
\[
\Pr[\stmt \notin L_R \wedge \Verify(\crs, \stmt, \pi) = 1] \leq \negl(\secparam).
\]
% \pnote{$\cap$ is set intersection, you probably want $\wedge$ which is the logical-and operation}
\item 
{\bf Zero-Knowledge:}
% For all \ppt verifiers $\mcal{V}^*$,
There exists a 
% \pnote{NIZK simulators are strict polytime} 
\ppt simulator $\Sim = (\Setup^*, \allowbreak \Prove^*)$ 
and there exists a negligible function $\negl$ such that 
for all \ppt distinguishers \D, 
for all $\secparam \in \N$,
for all $(\stmt, \wit) \in R$, 
% \pnote{verifier shouldn't be choosing the witness}
% \pnote{what is adaptive about this definition?}
% \pnote{better to define two games: REAL and IDEAL played with the verifier where games output views, and then ask views to be indistinguishbable}
% \pnote{It is better to avoid the notation $\approx_c$ and spell it out completely using a distinguisher.}
\[
| 
\Pr[\D(\crs, \pi) = 1] 
-
\Pr[\D(\crs^*, \pi^*) = 1]
| \leq \negl(\secparam),
\]
where
$\crs \gets \Setup(1^\secparam)$,
% $\crs^* \gets \Setup^*(1^\secparam)$,
$\pi \gets \Prove(\crs, \stmt,$ $ \wit)$, 
$(\crs^*, \td) \allowbreak \gets \Setup^*(1^\secparam)$,
$\pi^* \allowbreak \gets \Prove^*(\crs^*, \td, \stmt)$ and 
$\td$ is a trapdoor used by $\Sim$ to come up with proof $\pi^*$ for a statement $\stmt$ without knowing its witness.
% $\pi^* \gets \Prove^*(\crs^*, \stmt)$.
% \nikhil{check with Pratik if these definitions are alright.}
\end{itemize}

\end{definition}

\subsection{Inner Product Functional Encryption}
\label{sec:ipeprelim}
% \anote{Compress this into short paragraph}
We will need a inner-product functional encryption scheme (IPFE). 
Let $\ell$ be an integer. 
We define IPFE for computing inner products of vectors of length $\ell$. Let the message space be $\mcal{M} \subseteq \Z^\ell$ and function space $\mcal{F}_{{\sf IP}, \ell}$. Messages are denoted by $\bfx \in \mcal{M}$, functions are denoted by $\bfy \in \mcal{F}_{{\sf IP}, \ell}$ and the function evaluation is denoted by $f_\bfy(\bfx)$ (all three of them are parameterized by the prime $p \in \pp$ as output by $\Gen$ below).
% \pnote{maybe emph that we define IPE scheme for message space $\mathbb{Z}_p^n$ and hence our functions are described by a $\mathbb{Z}_p^n$ element.}
% However, we will need our underlying IPE to satisfy a few nice properties, including
% the fact that $\Enc$ and $\KGen$ 
% should still work when taking in the group encoding
% of the plaintext or key vector; moreover, we want that the scheme
% computes the ``inner-product in the exponent''.
Formally, IPFE consists of the 
following algorithms:

\begin{itemize}[itemsep=1pt,leftmargin=*]
\item 
$\pp \leftarrow \Gen(1^\secparam)$: 
it is a {\em randomized} algorithm that 
takes in a security parameter $\secparam$ 
and samples public parameters $\pp$.
We assume that $\pp$ contains a prime number $p$.
% We will assume that $\pp$ contains
% the description of a cyclic group $\G$ 
% of prime order $p$, and
% a random generator $g \in \G$.

\item 
$(\mpk, \msk) \leftarrow \Setup(\pp, \ell)$:
it is a {\em randomized} algorithm that 
takes in the public parameters $\pp$ and the vector length $\ell$,
outputs a master public key $\mpk$ and 
a master secret key $\msk$. 

\item 
$\sk_\bfy := \KGen(\msk, \bfy \in \mcal{F}_{{\sf IP}, \ell})$:
it is a {\em deterministic} algorithm that 
takes in the master secret key $\msk$, and 
a vector $\bfy \in \mcal{F}_{{\sf IP}, \ell}$,
outputs a functional secret key $\sk_\bfy$.

\item 
$\ct \leftarrow \Enc(\mpk, \bfx \in \mcal{M})$:
it is a {\em randomized} algorithm that 
takes in the master public key $\mpk$, 
a plaintext vector $\bfx \in \mcal{M}$, 
and outputs a ciphertext $\ct$.

\item 
$v := \Dec(\sk_\bfy, \ct)$:
it is a {\em deterministic} algorithm that 
takes in the functional secret key $\sk_\bfy$ 
%the group encoding $\grp\bfy$ of $\bfy$, 
and a ciphertext $\ct$, and outputs a decrypted outcome $v$.
\end{itemize}

Further, we augment the IPFE scheme with an additional algorithm $\PubKGen$ defined as follows. 
\begin{itemize}[itemsep=1pt,leftmargin=*]
\item $\pk_\bfy := \PubKGen(\mpk, \bfy \in \mcal{F}_{{\sf IP}, \ell})$:
it is a {\em deterministic} algorithm that 
takes in the master public key $\mpk$, and 
a vector $\bfy \in \mcal{F}_{{\sf IP}, \ell}$,
outputs a functional public key $\pk_\bfy$. 
\end{itemize}

Next, we describe the correctness of IPFE.
\begin{definition}[IPFE Correctness]
\label{def:ipfe-correctness}
For any $\secparam \in \N$,
let $\pp \gets \Gen(1^\secparam)$, 
then for any 
$ \ell \in \N, \bfx \in \mcal{M}, \bfy \in \mcal{F}_{{\sf IP}, \ell}$, 
the following holds:
\[
\Pr\left[
v = f_\bfy(\bfx): 
\begin{array}{l}
(\mpk, \msk) \leftarrow  \Setup(\pp, \ell),\\ 
\sk_\bfy = \KGen(\msk, \bfy),\\ 
\ct \leftarrow \Enc(\mpk, \bfx),\\ 
v = \Dec(\sk_\bfy, \ct)
\end{array}
\right] = 1.
\]
\end{definition}

% \anote{Introduce $\PubKGen$ here.}

% \pnote{we now want to modify this definition be selective in the challenge message.}
Next, we describe the security of IPFE.
\begin{definition}[Selective, IND-security]
\label{def:ipfe-sel-ind-sec}
We say that the \ipe scheme satisfies selective,  IND-security, 
iff for any non-uniform \ppt admissible adversary \A, 
there exists a negligible function $\negl$ 
such that for all $\secparam \in \N, \ell \in \N$,
\begin{align*}
& |
\Pr[\ipfeIND^0(1^\secparam, \ell) = 1] \\
& \quad - \Pr[\ipfeIND^1(1^\secparam, \ell) = 1]
| \leq \negl(\secparam),
\end{align*}
where experiments $\ipfeIND^b(1^\secparam)$ for $b \in \{0,1\}$ are described in~\Cref{fig:ipfe-sel-ind-sec}.
Here, an adversary \algA is said to be {\it admissible} iff the following
holds with probability $1$:
for any $\bfy$
submitted in a $\mcal{O}_\KGen$ oracle query, 
it must be that 
$f_\bfy(\bfx^*_0) = f_\bfy(\bfx^*_1)$.
\end{definition}

\begin{figure}[H]
\centering
\captionsetup{justification=centering}
% \fbox{
\begin{pcvstack}[boxed, space=1em]
\procedure[linenumbering, mode=text]{Experiment $\ipfeIND^b(1^\secparam, \ell)$}{
$\pp \gets \Gen(1^\secparam)$
\\ 
$(\bfx^*_0, \bfx^*_1) \gets \A(\pp)$
\\ 
$(\mpk, \msk) \gets \Setup(\pp, \ell)$
\\ 
$\ct^* \gets \Enc(\mpk, \bfx^*_b)$
\\ 
$b' \gets \A^{\mcal{O}_\KGen(\cdot)}(\mpk, \ct^*)$
\\ 
\ret $b'$
}
\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_\KGen(\bfy)$}{
\ret $\sk_\bfy = \KGen(\msk, \bfy)$
}
\end{pcvstack}
% }
\caption{Selective, IND-security experiment of Inner Product Functional Encryption
% \pnote{To be consistent with the literature, I would just call it WI and WH instead of WitInd and WitHid.}
% \nikhil{done}
}
\label{fig:ipfe-sel-ind-sec}
\end{figure}

The above IND-security level is called selective because it requires the adversary to commit to the challenge message pair even before it sees $\mpk$. Stronger security models exist such as (i) semi-adaptive, IND-security where the adversary can commit to the challenge message pair after seeing $\mpk$ but before gaining access to the oracle $\mcal{O}_\KGen$ and (ii) adaptive, IND-security where the adversary can commit to the challenge message pair after seeing $\mpk$ and the power to make queries to the oracle $\mcal{O}_\KGen$ before and after committing to the challenge message pair. But, we only consider selective, IND-security as it suffices for the scope of this work.
We also note that any adaptive, IND-secure IPFE is also selective, IND-secure.

\begin{remark}
We note that $\pk_\bfy$ does not enable decryption by any means, so it will not change the correctness requirement. It will also not affect security of IPFE in any way. To see this, note that $\PubKGen$ is deterministic. So, an adversary can always compute $\pk_\bfy$ on its own. Given that $\KGen$ is also deterministic, one way to think of $\pk_\bfy$ is as a statistically binding and computationally hiding commitment to $\sk_\bfy$. Typically, $\mpk$ also has this property w.r.t.\ $\msk$ and it is always implicit in the security definitions of IPFE. We make this explicit below for $\pk_\bfy$ and $\sk_\bfy$ because our functional adaptor signatures will rely on it. 
We formalize this compliance requirement below.
\end{remark}

\begin{definition}[$R_\ipfe$-Compliant IPFE]
\label{def:ipfe-compliant-appendix}
For a hard relation $R_\ipfe$, we say that an IPFE scheme is $R_\ipfe$ compliant if
for any $\secparam \in \N$,
for any $\pp \gets \ipe.\Gen(1^\secparam)$,
for any $(\mpk, \msk) \gets \ipe.\Setup(\pp, 1^\ell)$, 
for any $\bfy \in \mcal{F}_{{\sf IP}, \ell}$,
let $\pk_\bfy := \PubKGen(\mpk, \bfy)$, and 
$\sk_\bfy := \KGen(\msk, \bfy)$.
Then, it must be the case that $(\pk_\bfy, \sk_\bfy) \in R_\ipe$.
\end{definition}

Next, we describe an additional correctness property of IPFE that is tailored specifically to make IPFE compatible with adaptor signatures when the two are used in tandem in our functional adaptor signature construction. Looking ahead, we need this property because in our functional adaptor signature construction, we will use a standard adaptor signature to sell functional secret keys. Recall that adaptor signatures are defined w.r.t.\ two relations $R$ and $R'$. In this case, $R$ will be $R_\ipfe$ as defined in~\Cref{def:ipfe-compliant-appendix} and let us denote the corresponding extended relation $R'$ by $R'_\ipfe$. Then, the $\as.\Ext$ algorithm of adaptor signature scheme $\as$ will extract a functional secret key $\sk'_\bfy$ as the witness for the adaptor statement $\pk_\bfy$. While $\sk'_\bfy$ will be a witness of $R'_\ipfe$, it may not be a witness of the base relation $R_\ipfe$ since  $R_\ipfe \subseteq R'_\ipfe$, and we still want that $\sk'_\bfy$ should enable meaningful decryption. 
We formalize this robustness requirement below.

\begin{definition}[$R'_\ipfe$-Robust IPFE]
\label{def:ipfe-robust-appendix}
Let $R_\ipfe$ be the hard relation as defined in~\Cref{def:ipfe-compliant-appendix}. 
Let $R'_\ipfe$ such that $R_\ipfe \subseteq R'_\ipfe$ be an 
an extended relation of $R_\ipfe$. 
We say that an IPFE scheme is $R'_\ipfe$ robust if 
IPFE correctness holds even w.r.t.\ a functional secret key satisfying $R'_\ipfe$. More formally, 
for any $\secparam \in \N$,
let $\pp \gets \ipfe.\Gen(1^\secparam)$,
then for any $\ell \in \N$, 
$\bfx \in \mcal{M}, \bfy \in \mcal{F}_{{\sf IP}, \ell}$, the following holds: 
\[
\Pr\left[
v = f_\bfy(\bfx): 
\begin{array}{l}
(\mpk, \msk) \leftarrow  \Setup(\pp, \ell),\\ 
\pk_\bfy = \PubKGen(\msk, \bfy),\\ 
\sk'_\bfy \ s.t.\ (\pk_\bfy, \sk'_\bfy) \in R'_\ipfe,\\
\ct \leftarrow \Enc(\mpk, \bfx),\\ 
v = \Dec(\sk'_\bfy, \ct)
\end{array}
\right] = 1.
\]
\end{definition}

\begin{remark}
One can think of decryption correctness (\Cref{def:ipfe-correctness}) as being implicitly defined with respect to $\sk_\bfy$ that is witness to $\pk_\bfy$ for the relation $R_\ipfe$. And one can think of the $R'_\ipfe$-robustness as decryption correctness with respect to $\sk'_\bfy$ that is witness to $\pk_\bfy$ for the relation $R'_\ipfe$. 
% Note that here $R_\ipfe \subseteq R'_\ipfe$. 
% Thus, if $(\pk_\bfy, \sk_\bfy) \in R_\ipfe$, then, $(\pk_\bfy, \sk_\bfy) \in R'_\ipfe$. But, $(\pk_\bfy, \sk'_\bfy) \in R'_\ipfe$ does not necessarily imply $(\pk_\bfy, \sk'_\bfy) \in R_\ipfe$. It is for this reason that we need IPFE special property 2 beyond just IPFE correctness.
\end{remark}

% Lastly, we require a compatability property from our IPFE as follows. This will be useful for proving zero-knowledge witness privacy of our functional adaptor signature scheme.

% \begin{definition}[$(\mcal{M},\mcal{F}_{{\sf IP}, \ell})$- Compatible IPFE]
% \label{def:ipfe-compatible}
% We say that an IPFE scheme for message space $\mcal{M}$ and function space $\mcal{F}_{{\sf IP}, \ell}$ is $(\mcal{M},\mcal{F}_{{\sf IP}, \ell})$-compatible if for any $\bfx \in \mcal{M}$ and any $\bfy \in \mcal{F}_{{\sf IP}, \ell}$, it is the case that $f_\bfy(\bfx) \in \mcal{F}_{{\sf IP}, 1}$.
% \end{definition}

Abdalla et al.~\cite{ipe} constructed selective, IND-secure IPFE schemes from DDH and LWE. Subsequently, Agrawal et al.~\cite{ipe01} constructed adaptive, IND-secure IPFE schemes from DDH, DCR, and LWE. 
Within the scope of this work, we will use the following two IPFE schemes:
\begin{itemize}[leftmargin=*]
\item 
The DDH based IPFE by Abdalla et al.~\cite{ipe}. 
This scheme computes inner products with output values polynomially bounded by $B \ll p$. 
Specifically, the message space is $\mcal{M} = \Z_p^\ell$ and the function class is $\mcal{F}_{{\sf IP}, \ell, p, B} = \{ f_\bfy : \bfy \in \Z_p^\ell\} \subseteq \mcal{F}_{{\sf IP}, \ell}$, where $f_\bfy: \Z_p^\ell \to \{0, \ldots, B\}$ is defined as $f_\bfy(\bfx) = \bfx^T \bfy \in \{0, \ldots, B\}$. 
% \nikhil{add reference to where it is described}
\item 
The LWE based IPFE by Agrawal et al.~\cite[Section 4.2]{ipe01}.
This scheme computes inner products modulo $p$. 
Specifically, the message space is $\mcal{M} = \Z_p^\ell$ and the function class is $\mcal{F}_{{\sf IP}, \ell, p} = \{ f_\bfy : \bfy \in \Z_p^\ell\} \subseteq \mcal{F}_{{\sf IP}, \ell}$, where $f_\bfy: \Z_p^\ell \to \Z_p$ is defined as $f_\bfy(\bfx) = \bfx^T \bfy \bmod{p} \in \Z_p$.
% \nikhil{add reference to where it is described}
\end{itemize}

\subsection{Lattice Preliminaries}

We denote by $\S_c = \{ \bfx \in \Z_q^n : ||\bfx||_\infty \leq c\}$ the set of vectors in $\Z_q^n$ whose maximum absolute coefficient is at most $c \in \Z^+$. 

\begin{definition}[$\sis_{n, m,q,\beta}$]
Let $\bfA \getr \Z_q^{n \times m}$.
Given $\bfA$, \sis problem with parameters $m>1$ and $0 < \beta < q$ asks to find a short non-zero $\bfv \in \Z^m$ such that $\bfA \bfv = 0 \bmod{q}$ and $||\bfv||_\infty \leq \beta$.
\end{definition}

Next, we define $\sis$ in Hermite Normal Form (HNF).
\begin{definition}[$\hnfsis_{n, m,q,\beta}$]
Let $\bfA' \getr \Z_q^{n \times (m-1)}$ and $\bfA = (\bfnum{1} || {\bfA'}) \in \Z_q^{n \times m}$.
Given $\bfA$, \hnfsis problem with parameters $m>1$ and $0 < \beta < q$ asks to find a short non-zero $\bfv \in \Z^m$ such that $\bfA \bfv = 0 \bmod{q}$ and $||\bfv||_\infty \leq \beta$.
\end{definition}

\begin{definition}[$\isis_{n, m, q, \beta}$]
\label{def:isis}
It is the inhomogeneous version of \hnfsis. 
Let $\bfA' \getr \Z_q^{n \times (m-1)}$ and $\bfA = (\bfnum{1} || {\bfA'}) \in \Z_q^{n \times m}$ and
let $\bfu \getr \Z^m$ s.t. $||\bfu||_\infty \leq \beta$. 
Let $\bfb = \bfA \bfu \in \Z_q^n$. 
Given $(\bfA, \bfb)$, the problem with parameters $m>1$ and $0 < \beta < q$ asks to find a short non-zero $\bfv \in \Z^m$ such that $\bfA \bfv = \bfb \bmod{q}$ and $||\bfv||_\infty \leq \beta$. 
\end{definition}

\begin{definition}[$\lwe_{n, m, q, \Psi}$]
\lwe problem with parameters $n, m>0$ and distribution $\Psi$ over $\Z_q$ asks to distinguish between the following two cases with non-negligible advantage: 1) $(\bfA, \bfb) \getr \Z_q^{m \times n} \times \Z_q^m$, and 2) $(\bfA, \bfA \bfs + \bfe)$ for $\bfA \getr \Z_q^{m \times n}$, a secret $\bfs \getr \Z_q^n$ and an error vector $\bfe \gets \Psi^m$.
\end{definition}

\begin{definition}[Multi-hint extended-LWE]
\label{def:mhe-lwe}
Let $q, m, t$ be integers, $\alpha$ be a real and $\tau$ be a distribution over $\Z^{t \times m}$, all of them functions of a parameter $n$. The multi-hint extended-LWE problem $\mheLWE_{n, m, q, \alpha, t, \tau}$ is to distinguish between the distributions of the tuples 
\[
(\bfA, \bfb, \bfZ, \bfZ \bfe) \text{ and }
(\bfA, \bfA \bfs + \bfe, \bfZ, \bfZ \bfe), 
\]
where $\bfA \getr \Z_q^{m \times n}$, $\bfs \getr \Z_q^n$, $\bfb \getr \Z_q^m$, $\bfe \gets D_{\Z, \alpha q}^m$, $\bfZ \gets \tau$.
\end{definition}

\begin{lemma}[\cite{ipe01}, Theorem 4]
Let $n \geq 100$, $q \geq 2$, $t < n$ and $m$ with $m = \Omega(n \log n)$ and $m \leq n^{O(1)}$. 
There exists $\xi \leq O(n^4 m^2 \log^{5/2} n)$ and a distribution $\tau$ over $\Z^{t \times m}$ such that the following statements hold:
\begin{itemize}[leftmargin=*]
\item 
There is a reduction from $\LWE_{n-t, m, q, D_{\Z, \alpha q}}$ to $\mheLWE_{n, m, q, \alpha, t, \tau}$.
\item 
It is possible to sample from $\tau$ in polynomial time in $n$.
\item 
Each entry of matrix $\tau$ is an independent discrete Gaussian $\tau_{i,j} = D_{\Z,\sigma_{i,j},c_{i,j}}$ for some $c_{i,j} \in \{0,1\}$ and $\sigma_{i,j} \geq \Omega(\sqrt{mn \log m})$.
\item 
With probability at least  $1 - n^{-\omega(1)}$, all rows from a sample from $\tau$ have norms at most $\xi$.

\end{itemize}
\end{lemma}

\begin{definition}[Discrete Gaussian distribution]
A discrete gaussian distribution $D_{\Lambda, \sqrt{\Sigma}, \bfc}$, for $\bfc \in \R^n$, $\Sigma$ a positive semi-definite matrix in $\R^{n \times n}$, and a lattice $\Lambda \subset \Z^n$, is a distribution with values in $\Lambda$ and probabilities
\[
\Pr[X = \bfx] \propto \exp{\left(-\frac12 (\bfx - \bfc)^T\Sigma^+(\bfx-\bfc)\right)}.
\]
\end{definition}
Note that $\Sigma^+$ denotes the pseudoinverse of a matrix. If $\Lambda = \Z^n$, we shall just write $D_{\sqrt{\Sigma}, \bfc}$. Further, if $\bfc = 0$, then we shall just write $D_{\sqrt{\Sigma}}$, and if $\sqrt{\Sigma} = \sigma I_n$ for $\sigma \in \R^+$ and $I_n$ an identity matrix, we shall just write $D_\sigma$.

% \nikhil{describe discrete gaussian over $\Z_q$: $\D_{\Z_q, \sigma, 0}$}


==> old-overview.tex <==
\section{Technical Overview}

We first present two strawman approaches ``Compiler Approach'' and ``Direct Approach'' for building functional adaptor signatures. 
While these approaches will have some  shortcomings that we will discuss, more importantly they also motivate our main construction which we present subsequently.

\pnote{from here}
\subsection{Compiler Approach}
% \pnote{I view this as a compiler not because of BB use of components, but because it "compiles" adaptors for dlog to adaptors for NP.}
\pnote{I forgot the shortcomings of the compiler approach, can you message on slack?}

We first present a construction of adaptor signatures w.r.t.\ the Schnorr signature scheme $\Sch$ and any hard relation $R_L$. 
We obtain this from three building blocks:
\begin{itemize}
\item 
Adaptor Signature $\Pi'_{ADP}$ w.r.t.\ the Schnorr signature scheme $\Sch$ and the discrete log hard relation $R_{DL}$
\item 
NIZKs for NP 
\item 
Secret Key Encryption 
\end{itemize}
The construction can be viewed as a compiler from adaptor signatures w.r.t.\ a specific hard relation $R_{DL}$ to one w.r.t.\ any hard relation $R_L$.

Next, we will present a construction of functional adaptor signatures w.r.t.\ the Schnorr signature scheme $\Sch$, any hard relation $R_L$, and any function class $\mcal{F}$. 
This construction will essentially be an extension of the previous construction. 

\subsubsection{Adaptor Signatures w.r.t.\ $\Sch$ and any hard relation $R_L$}

Suppose that a seller wants to sell a witness $x$ for a statement $X$ where $(X, x)\in R_L$. 
Suppose that the schnorr signature scheme $\Sch$ is defined for a group $\G$ of prime order $q$ and with generator $g$. 
Suppose that everyone knows the common reference string $\crs$ of the NIZK proof system. Then, we describe the adaptor signature scheme next. Recall that an adaptor signature scheme comprises of three stages: (i) seller advertisement, (ii) buyer proposal, (iii) sale.

\paragraph{Seller Advertisement.}
The seller first samples a $\ske$ key $k \getr \Z_q$, computes $\ct = \ske.\Enc(k, x; r)$ where $r$ are the random coins consumed by the encryption algorithm, and generates a proof $\pi \gets \nizk.\Prove(\crs, (g^k, X, \ct), (k, x, r))$ attesting that the ciphertext $\ct$ encrypts $x$ (which is a witness for $X$ w.r.t.\ relation $R_L$) using key $k$ (which is a witness for $g^k$ w.r.t.\ relation $R_{DL}$) and random coins $r$. Then, the seller advertises $\advt = (X, g^k, \ct, \pi)$ to everyone. 

\paragraph{Buyer Proposal.}
Suppose a buyer sees the advertisement $\advt$ and wants to buy the witness. 
Suppose the buyer has the key pair $(\sk, \vk)$ for the adaptor signature scheme $\Pi'_{ADP}$.
Then, the buyer does the following. It first verifies the proof $\pi$ by running $\nizk.\Verify(\crs, (g^k, X, \ct), \pi)$. If the verification fails, the buyer aborts. Else, it chooses some message $m$ and computes pre-signature w.r.t.\ statement $g^k$ as $\widetilde{\sigma} = \Pi'_{ADP}.\PreSign(\sk, m, g^k)$ and sends the buyer proposal $m, \widetilde{\sigma}$ to the seller. 

\paragraph{Sale.}
On receiving the proposal $m, \widetilde{\sigma}$ from a buyer with verification key $\vk$, the seller first checks if pre-signature verifies as $\Pi'_{ADP}.\PreVerify(\vk, m, g^k, \widetilde{\sigma})$. If the check fails, then, the seller rejects the proposal. Else, the seller executes the sale by computing signature $\sigma = \Pi'_{ADP}.\Adapt(\widetilde{\sigma}, k)$ and publishing $\sigma$ to the blockchain.

Note that the signatures $\sigma$ gets published to the blockchain only if it satisfies $\Sch.\Verify(\vk, m, \sigma)$. In such a case, the buyer can extract the SKE key $k = \Pi'_{ADP}.\Ext(\widetilde{\sigma}, \sigma)$ and obtain the witness by decrypting the ciphertext as $x = \ske.\Dec(k, \ct)$.

\subsubsection{Functional Adaptor Signatures w.r.t.\ $\Sch$, any hard relation $R_L$, and any function class $\mcal{F}$.}

Suppose that a seller wants to sell function evaluations of witness $x$ for a statement $X$ where $(X, x)\in R_L$. 
Suppose that the schnorr signature scheme $\Sch$ is defined for a group $\G$ of prime order $q$ and with generator $g$. 
Suppose that everyone knows the common reference string $\crs$ of the NIZK proof system. 
Suppose $\mcal{F} = \{f_1, \ldots, f_{|\mcal{F}|} \}$.
Then, we describe the functional adaptor signature scheme next. Recall that a functional adaptor signature scheme comprises of three stages: (i) seller advertisement, (ii) buyer proposal, (iii) sale.

\paragraph{Seller Advertisement.}
This is same as the seller advertisement in the previous construction except that we encrypt $f_i(x)$ instead of $x$ for all $f_i \in \mcal{F}$. More concretely, for all $i \in [|\mcal{F}|]$, the seller samples a $\ske$ key $k_i \getr \Z_q$, computes $\ct_i = \ske.\Enc(k_i, f_i(x); r_i)$ where $r_i$ are the random coins consumed by the encryption algorithm, and generates a proof $\pi \gets \nizk.\Prove(\crs, (g^{k_i}, X, f_i, \ct), (k_i, x, r))$ attesting that the ciphertext $\ct$ encrypts $f_i(x)$ (where $x$ is a witness for $X$ w.r.t.\ relation $R_L$) using key $k_i$ (which is a witness for $g^{k_i}$ w.r.t.\ relation $R_{DL}$) and random coins $r_i$. Then, the seller advertises $\advt = (X, \{g^{k_i}, \ct_i, \pi_i\}_{i \in [|\mcal{F}|]})$ to everyone. 

\paragraph{Buyer Proposal.}
Suppose a buyer sees the advertisement $\advt$ and wants to buy the function $f_i$ evaluated on the witness. 
Suppose the buyer has the key pair $(\sk, \vk)$ for the adaptor signature scheme $\Pi'_{ADP}$.
Then, the buyer does the following. It first verifies the proof $\pi_i$ by running $\nizk.\Verify(\crs, (g^{k_i}, X, \ct_i), \pi_i)$. If the verification fails, the buyer aborts. Else, it chooses some message $m$ and computes pre-signature w.r.t.\ statement $g^{k_i}$ as $\widetilde{\sigma} = \Pi'_{ADP}.\PreSign(\sk, m, g^k)$ and sends the buyer proposal $m, f_i, \widetilde{\sigma}$ to the seller. 

\paragraph{Sale.}
On receiving the proposal $m, f_i, \widetilde{\sigma}$ from a buyer with verification key $\vk$, the seller first checks if pre-signature verifies as $\Pi'_{ADP}.\PreVerify(\vk, m, g^{k_i}, \widetilde{\sigma})$. If the check fails, then, the seller rejects the proposal. Else, the seller executes the sale by computing signature $\sigma = \Pi'_{ADP}.\Adapt(\widetilde{\sigma}, k_i)$ and publishing $\sigma$ to the blockchain.

Note that the signatures $\sigma$ gets published to the blockchain only if it satisfies $\Sch.\Verify(\vk, m, \sigma)$. In such a case, the buyer can extract the SKE key $k_i = \Pi'_{ADP}.\Ext(\widetilde{\sigma}, \sigma)$ and obtain the function $f_i$ evaluated on the witness by decrypting the ciphertext $ct_i$ as $f_i(x) = \ske.\Dec(k_i, \ct_i)$.

\paragraph{Problem: Large Advertisement size.}
Note that in the above strawman construction, the size of the advertisement $\advt$ grows linearly with the size of the function class $\mcal{F}$. This is problematic and we want to avoid it. To illustrate this point, consider the simple function class of linear functions represented as inner product computation. Here, $f_\bfy(\bfx) = \bfx^T \bfy$, where $\bfx, \bfy \in \Z_q^n$. Thus, $\mcal{F}_{IP, \Z_q^n} = \{\bfy \in \Z_q^n\}$ and $|\mcal{F}_{IP, \Z_q^n}| = q^n$. Note here that $q$ is the prime order of the group $G$. Thus, $q$ is at least super-polynomial in the security parameter $\secparam$ and hence, so is the $|\mcal{F}_{IP, \Z_q^n}|$. This is always going to be impractical to realize and thus, we would ideally like the advertisement size to be independent of the size of the function class $|\mcal{F}|$.

\subsection{Direct Approach}
Here, we present a direct approach which avoid using $\ske$ altogether in an attempt to achieve the advertisement size to be independent of the size of the function class $|\mcal{F}|$. 
We present the direct approach to build functional adaptor signatures w.r.t.\ the Schnorr signature scheme $\Sch$, any hard relation $R_L$ whose witnesses belong to $\Z_q^n$, and the inner-products  function class $\mcal{F}_{IP, \Z_q^n}$. 

\paragraph{Seller Advertisement.}
Suppose the seller wants to sell function evaluations of witness $\bfx \in \Z_q^n$ of statement $X$. Then, the seller considers another statement $g^\bfx$ and generates a proof $\pi \gets \nizk.\Prove(\crs, (X, g^\bfx), \bfx)$ attesting that $\bfx$ is a witness for $X$ w.r.t.\ relation $R_L$ and a witness for $g^\bfx$ w.r.t.\ relation $R_{DL}$. Then, the seller advertises $\advt = (X, g^\bfx, \pi)$ to everyone. 

\paragraph{Buyer Proposal.}
Suppose a buyer sees the advertisement $\advt$ and wants to buy the function $\bfy$ evaluated on the witness. 
Suppose the buyer has the key pair $(\sk, \vk)$ for the adaptor signature scheme $\Pi'_{ADP}$.
Then, the buyer does the following. It first verifies the proof $\pi$ by running $\nizk.\Verify(\crs, (X, g^\bfx), \pi)$. If the verification fails, the buyer aborts. Else, it chooses some message $m$ and computes pre-signature w.r.t.\ statement $g^{\bfx^T\bfy} := \Pi_{i \in [n]} (g^{x_i})^{y_i}$ as $\widetilde{\sigma} = \Pi'_{ADP}.\PreSign(\sk, m, g^{\bfx^T\bfy})$ and sends the buyer proposal $m, \bfy, \widetilde{\sigma}$ to the seller. 

\paragraph{Sale.}
On receiving the proposal $m, \bfy, \widetilde{\sigma}$ from a buyer with verification key $\vk$, the seller first checks if pre-signature verifies as $\Pi'_{ADP}.\PreVerify(\vk, m, g^{\bfx^T\bfy}, \widetilde{\sigma})$. If the check fails, then, the seller rejects the proposal. Else, the seller executes the sale by computing signature $\sigma = \Pi'_{ADP}.\Adapt(\widetilde{\sigma}, \bfx^T\bfy)$ and publishing $\sigma$ to the blockchain.

Note that the signatures $\sigma$ gets published to the blockchain only if it satisfies $\Sch.\Verify(\vk, m, \sigma)$. In such a case, the buyer can extract the function evaluation $\bfy$ on the witness as $ \bfx^T\bfy = \Pi'_{ADP}.\Ext(\widetilde{\sigma}, \sigma)$.

\paragraph{Correctness.} Note that this approach satisfies correctness because given the group encoding of the witness as $g^\bfx$ and the function description $\bfy$, it is possible to efficiently compute the group encoding of the function evaluation as $g^{\bfx^T\bfy} := \Pi_{i \in [n]} (g^{x_i})^{y_i}$. This approach can work more generally for other function classes $\mcal{F}$ which satisfy a similar property: ``Given any $f \in \mcal{F}$ and group encoding of the witness $g^{\bfx}$, it is possible to efficiently compute the group encoding of the function evaluation $g^{f(\bfx)}$.''. Such an approach may not work for other function classes where this computation is inefficient.

\paragraph{Additional security assumption.}
For the hard relation $R_L$, let the corresponding set of witnesses be $W_L$.
Then, the hardness of the relation $R_L$ implies that given $X$, it is computationally infeasible to find $\bfx \in W_L$. But to prove security of the above construction, we additionally need to assume that for any $\bfx \in W_L$, given $g^\bfx$, it is still computationally infeasible to find $\bfx$. 

\paragraph{Problem: additional security assumption does not always hold.}
We note that this additional security assumption often does not hold true. Note that if $\bfx = (x_1, \ldots, x_n)$, then, $g^\bfx = (g^{x_1}, \ldots, g^{x_n})$. So, intuitively, given $X$, it could be  computationally infeasible to find $\bfx = (x_1, \ldots, x_n)$ if there is sufficient entropy in $\bfx$ left. But, given $g^\bfx = (g^{x_1}, \ldots, g^{x_n})$, it will be computationally infeasible to find $\bfx = (x_1, \ldots, x_n)$ if there is sufficient entropy left in each entry of $\bfx$. This assumption does not hold if each entry of $\bfx$ is in a small range space.
For instance, in medical data, consider $X = $ ``In database $\bfx$ of 1000 cancer patients, 150 had a malignant tumor'', where $\bfx = (x_1, \ldots, x_{1000})$ and each $x_i \in \{0,1\}$. Here, given $X$ there are $\binom{1000}{150}$ possibilities of $\bfx$ where each is equally likely, but, given $g^\bfx$, it is easy to recover $\bfx$.

\subsection{Our Approach: Functional Encryption}
\nikhil{we describe this section for a general function class $\mcal{F}$. If necessary, change it to inner-products specifically.}
Suppose that the schnorr signature scheme $\Sch$ is defined for a group $\G$ of prime order $q$ and with generator $g$. 
Suppose that a seller wants to sell function evaluations of witness $\bfx \in \Z_q^n$ for a statement $X$ where $(X, \bfx)\in R_L$. 
Suppose that everyone knows the common reference string $\crs$ of the NIZK proof system. 
Suppose $\mcal{F} = \{f_1, \ldots, f_{|\mcal{F}|} \}$ and let $\fe$ be a functional encryption scheme for computing function in the class $\mcal{F}$. Looking ahead, we will need an additional algorithm for the $\fe$ scheme which we will describe below.

For constructing our functional adaptor signature scheme, we need two main ideas that we discuss next.
\begin{itemize}
\item {\bf Idea 1:} $\advt$ will now contain a single FE encryption of $\bfx$ instead of containing encryptions of all possible function evaluations on $\bfx$. 
This ensures that size of $\advt$ is sub-linear in $|\mcal{F}|$ because for any non-trivial functional encryption scheme, the ciphertext size is sub-linear in $|\mcal{F}|$.  
For instance, when we consider the class of inner-product functions $f: \Z_q^n \times \Z_q^n \to \Z_q$, $\advt$ is linear in $q$ and $n$ instead of linear in $|\mcal{F}|$, where $|\mcal{F}| = q^n$. 
\item {\bf Idea 2:} we will use the adaptor signature scheme to sell the functional secret key $\sk_f$ which will enable decrypting the FE ciphertext to $f(\bfx)$. The main challenge in enabling this approach is that we need the buyer to pre-sign w.r.t.\ a statement corresponding to the witness $\sk_f$. While the buyer can request the seller to provide such a statement, this additional round of interaction actually trivializes the problem. So, we crucially are interested in overcoming this challenging without additional rounds of interaction. To address this challenge, we augment the $\fe$ scheme with an additional public keygen algorithm $\PubKGen$ as described next.
\end{itemize}

\paragraph{Additional public keygen algorithm for $\fe$.}
Suppose that $\fe$ has an additional {\em deterministic} public keygen algorithm that computes $\pk_f := \fe.\PubKGen(\mpk, f)$ such that $(\pk_f, \sk_f) \in R_{DL}$, where $\sk_f = \fe.\KGen(\msk, f)$. Then, the buyer can pre-sign w.r.t.\ the statement $\pk_f$ for its choice of function $f \in \mcal{F}$. Note that the algorithm $\PubKGen$ does not affect the FE security game as the algorithm is deterministic and thus the adversary does not learn any new information in the FE security game.

More concretely, our construction then is as follows.

\paragraph{Seller Advertisement.}
The seller samples a $\fe$ master key pair $(\mpk, \msk)$, computes FE ciphertext $\ct = \fe.\Enc(\mpk, x; r)$ where $r$ are the random coins consumed by the encryption algorithm, and generates a proof $\pi \gets \nizk.\Prove(\crs, (X, \mpk, \ct), (x, r))$ attesting that the ciphertext $\ct$ encrypts $\bfx$ (which is a witness for $X$ w.r.t.\ relation $R_L$) using master public key $\mpk$ and random coins $r$. Then, the seller advertises $\advt = (X, \mpk, \ct, \pi)$ to everyone. 

\paragraph{Buyer Proposal.}
Suppose a buyer sees the advertisement $\advt$ and wants to buy the function $f \in \mcal{F}$ evaluated on the witness. 
Suppose the buyer has the key pair $(\sk, \vk)$ for the adaptor signature scheme $\Pi'_{ADP}$.
Then, the buyer does the following. It first verifies the proof $\pi$ by running $\nizk.\Verify(\crs, (X, \mpk, \ct), \pi)$. If the verification fails, the buyer aborts. Else, it chooses some message $m$ and computes pre-signature w.r.t.\ statement $\pk_f := \fe.\PubKGen(\mpk, f)$ as $\widetilde{\sigma} = \Pi'_{ADP}.\PreSign(\sk, m, \pk_f)$ and sends the buyer proposal $m, f, \widetilde{\sigma}$ to the seller. 

\paragraph{Sale.}
On receiving the proposal $m, f, \widetilde{\sigma}$ from a buyer with verification key $\vk$, the seller first checks if pre-signature verifies as $\Pi'_{ADP}.\PreVerify(\vk, m, \pk_f, \widetilde{\sigma})$, where $\pk_f$ can be locally computed by the seller. If the check fails, then, the seller rejects the proposal. Else, the seller executes the sale by computing the witness $\sk_f := \fe.\KGen(\msk, f)$, adapting the pre-signature to obtain the signature $\sigma = \Pi'_{ADP}.\Adapt(\widetilde{\sigma}, \sk_f)$ and publishing $m, \vk, \sigma$ to the blockchain.

Note that the signatures $\sigma$ gets published to the blockchain only if it satisfies $\Sch.\Verify(\vk, m, \sigma)$. In such a case, the buyer can extract the functional secret key $\sk_f = \Pi'_{ADP}.\Ext(\widetilde{\sigma}, \sigma)$ and obtain the function $f$ evaluated on the witness by decrypting the FE ciphertext $ct$ as $f(x) = \fe.\Dec(\sk_f, \ct)$.


==> prelims.tex <==
\section{Preliminaries}
\label{sec:prelims}\label{sec:notations}

We briefly recall the cryptographic tools needed in this work.

% \anote{Keep only the notations we need for group-based construction. The lattice one, push to the lattice section in the appendix.}

\smallskip\noindent\textbf{Notations.}
We denote by $x \gets S$ the experiment of sampling $x$ from a probability distribution $S$. 
We denote by $[A(\cdot)]$ the range of an algorithm $A(\cdot)$. 
If $p(\cdot, \cdot)$ denotes a predicate, then $\Pr[p(y, z): x \gets S, (y, z) \gets A(x)]$ is the probability that the predicate $p(y, z)$ is true after the ordered sequence of events $x \gets S$ followed by $(y, z) \gets A(x)$.
 We denote scalars by lower-case alphabets such as $x$, 
vectors by bold-face lower-case alphabets such as $\bfx$, 
matrices by bold-face upper-case alphabets such as $\bfX$. 
$\bfx = (x_1, x_2)^T$ denotes a column-vector with elements $x_1$ and $x_2$.
$\bfx^T$ denotes a row-vector.

\noindent\textbf{Linear Functions.}
We denote linear functions as inner product computation. 
Let $\mcal{F}_{{\sf IP}, \ell}$ denote the family of inner products of vectors of length $\ell$.
For a prime $p$, in this work we study two restrictions of inner product computations as follows:
\begin{itemize}[leftmargin=*]
\item \emph{Inner products modulo $p$.} 
The function class $\mcal{F}_{{\sf IP}, \ell, p} = \{ f_\bfy : \bfy \in \Z_p^\ell\}$, where $f_\bfy: \Z_p^\ell \to \Z_p$ is defined as $f_\bfy(\bfx) = \bfx^T \bfy \bmod{p}$.

\item \emph{Inner products with output values polynomially bounded by $B \ll p$.}
The function class $\mcal{F}_{{\sf IP}, \ell, p, B} = \{ f_\bfy : \bfy \in \Z_p^\ell\}$, where $f_\bfy: \Z_p^\ell \to \{0, \ldots, B\}$ is defined as $f_\bfy(\bfx) = \bfx^T \bfy \in \{0, \ldots, B\}$.

\end{itemize}
Often we will use $\bfy$ instead of $f_\bfy$ to denote the function. 

\smallskip\noindent\textbf{Digital Signature.}
A digital signature scheme 
$\DS := (\KGen, \Sign, \allowbreak \Verify)$ 
has a key generation algorithm $(\vk, \sk) \gets \KGen(1^\secparam)$ 
that outputs a verification-signing key pair. 
Using signing key $\sk$ we can compute signatures on a message $m$ 
by running $\sigma \gets \Sign(\sk, m)$, 
which can be publicly verified using the corresponding verification key $\vk$ 
by running $\Verify(\vk, m, \sigma)$. 
We require the digital signature scheme to satisfy strong existential unforgeability~\cite{sig}. 

\smallskip\noindent\textbf{Hard Relations.}
We recall the notion of a hard relation $R$ with statement/witness pairs 
$(X, x)$. We denote by $L_R$ the associated language defined as 
$L_R := \{ \ X \ | \ \exists \ x, (X , x) \in R \ \}$. 
We want the following properties from the hard relation: (1) Statement-witness pairs $(X , x) \in R$ can be efficiently sampled using a  sampling algorithm $\mathsf{GenR}(1^\secpar)$, (2) for all PPT adversaries  $\adv$ the
probability of $\adv$ on input $X$ outputting a witness $x'$ such that $(X, x') \in R$ is negligible, and 
(3) for a given function class $\mcal{F}$, for any PPT adversaries $\adv$ that is given input $X$, and returns $(f,z)$, it must be the case that $(f \in \mcal{F}) \wedge \left (z \in \{f(x') : \exists \ x' \text{ such that } (X,x') \in R \} \right )$ only with negligible probability.
If a relation satisfies only the first two properties, we call it \emph{hard}, and if it satisfies all three, it we call it \emph{$\mcal{F}$-hard}.
The formal definitions are described 
\ifcameraready
in the full version.
\else 
in~\cref{sec:more-prelims}. 
\fi
In this work, we use the discrete log language $L_\DL$ defined with respect to a group $\GG$ with generator $g$ and order $p$. The language is defined as $L_\DL := \{ Y \mid \exists y \in \ZZ_p,\ Y = g^y \}$ with corresponding hard relation $R_\DL = \{ (X,x)| X = g^x\}$.




\smallskip\noindent\textbf{Adaptor Signatures (AS).}
Adaptor Signatures were first formally defined in~\cite{asig}.
% and were used to enable one-time fair exchange of a coin for a witness. 
%Two different lines of work have improved the syntax and security subsequently. 
~\cite{pq-as} generalized the syntax in~\cite{asig} to enable constructing adaptor signatures from lattices. 
More concretely, ~\cite{asig} defined adaptor signatures w.r.t.\ a digital signature scheme and a hard relation $R$.
~\cite{pq-as} generalized it to be w.r.t.\  two hard relations $R$ and $R'$ such that such that $R \subseteq R'$. For the group-based constructions, typically we have $R=R'$, but for the lattice based constructions, typically we have $R \neq R'$.
In this work, one of our constructions will be from lattices, hence, we follow this generalized syntax. 


In a different vein, ~\cite{as-stronger,as-foundations} have strengthened the security properties of adaptor signatures, with notions like \emph{unforgeability}, \emph{pre-signature extractability}, and \emph{witness extractability}.
~\cite{as-stronger} further added \emph{unique extractability} and \emph{unlinkability} as security properties and unified \emph{unforgeability} and \emph{witness extractability} under a single security property called \emph{extractability}. ~\cite{as-foundations} further added \emph{pre-verify soundness} as a security property. We note that not all security properties are needed always. Within the scope of this work, we will use adaptor signatures as a building block for the construction of FAS and we only need \emph{pre-signature adaptability} and \emph{witness extractability} security properties of adaptor signatures. 
Intuitively, pre-signature adaptability ensures that 
given a valid pre-signature and a witness for the statement, one can always adapt the pre-signature into a valid signature.
Witness extractability requires that given an honestly generated pre-signature and a valid signature, one should be able to extract a witness.
The formal definitions of the properties are deferred 
\ifcameraready
to the full version.
\else
to~\cref{sec:more-prelims}.
\fi

%, thus enabling secure constructions of diverse applications of adaptor signatures such as private coin mixing~\cite{coin-mixing,qin2023blindhub} and oracle-based payments protocol~\cite{madathil2022cryptographic}. 
%More concretely, ~\cite{asig} introduced three security properties for adaptor signatures, namely, \emph{unforgeability}, \emph{pre-signature extractability}, and \emph{witness extractability}. 




% \nikhil{say surprisingly, we don't need unforgeability of adaptor signatures?}





% Combining the five properties described above, we can define a secure adaptor signature scheme as follows.

% \begin{definition}[Secure Adaptor Signature Scheme]
% An adaptor signature scheme $\AS$ is secure if it is extractable, unique extractable, weak pre-signature adaptable, pre-verify sound and unlinkable.
% \end{definition}

\smallskip\noindent\textbf{Non-Interactive Zero-Knowledge (NIZK) Arguments.}
A $\NIZK$ for the NP language $L_R$ in the {\em common reference string (CRS)} model consists of algorithms $(\Setup, \Prove, \Verify)$. $\Setup(1^\secparam)$ outputs the common reference string $\crs$.
$\Prove(\crs, \stmt, \wit)$ outputs a proof $\pi$ that statement $\stmt \in L_R$ using a witness $\wit$.
The validity of the proof can be checked by $\Verify(\crs, \stmt, \pi)$.
We require the $\NIZK$ argument system to be (1) \emph{complete}, where honestly generated proofs for $(\stmt, \wit) \in R$ verify successfully, (2) \emph{zero-knowledge}, where a malicious verifier does not learn more than the validity of the statement $\stmt$, i.e., there exists a  simulator $\Sim$ that without any information of the witness, can create an ideal-world view that the verifier can't distringuish from its real-world view, and (3) \emph{adaptive soundness}, where it is hard for any \ppt prover to convince a verifier of an invalid statement that is chosen by the prover after receiving $\crs$.
For formal definitions, we refer the reader 
\ifcameraready
to the full version.
\else
to~\cref{sec:more-prelims}.
\fi
Such NIZK arguments are known from 
factoring~\cite{feige1990multiple}, 
and standard assumptions on 
pairings~\cite{canetti2003forward,groth2006non} and 
lattices~\cite{peikert2019noninteractive,canetti2019fiat}.
% \nikhil{check with pratik for more cites}

\smallskip\noindent\textbf{Inner Product Functional Encryption (IPFE)}
% \anote{Compress this into short paragraph}
We will need a functional encryption scheme for computing inner products of vectors of length $\ell$. Let the message space be $\mcal{M} \subseteq \Z^\ell$ and function space $\mcal{F}_{{\sf IP}, \ell}$. Messages are denoted by $\bfx \in \mcal{M}$, functions are denoted by $\bfy \in \mcal{F}_{{\sf IP}, \ell}$ and the function evaluation is denoted by $f_\bfy(\bfx)$. 
An IPFE scheme is a tuple of five algorithms $(\Gen, \Setup, \KGen, \Enc,$ $\Dec)$: 
$\Gen(1^\secparam)$ algorithm samples public parameters $\pp$.
$\Setup(\pp, \ell)$ algorithm samples master public key $\mpk$ and master secret key $\msk$. 
$\KGen(\msk, \bfy)$ is a deterministic algorithm that outputs a functional secret key $\sk_\bfy$ for function vector $\bfy$.
$\Enc(\mpk, \bfx)$ algorithm outputs a ciphertext $\ct$ encrypting message vector $\bfx$.
$\Dec(\sk_\bfy, \ct)$ algorithm can be used to decrypt ciphertext $\ct$ to  reveal a value $v$ using functional secret key $\sk_\bfy$.
We require $\ipfe$ to satisfy 
(1) \emph{correctness}, where $v=f_\bfy(\bfx)$ if everything was honestly computed, 
(2) \emph{selective, IND-security}, where the adversary commits to challenge messages $(\bfx^*_0, \bfx^*_1)$ at the beginning of the game and obtains $\mpk, \ct^*$, where $\ct^*$ encrypts $\bfx^*_b$ for $b \in \{0,1\}$ unknown to adversary. 
Then, the adversary can make polynomially many $\KGen$ queries for functions $\bfy$ satisfying $f_\bfy(\bfx^*_0) = f_\bfy(\bfx^*_1)$. At the end of the game, the adversary wins if it can correctly guess the bit $b$. 
We defer the formal definitions
\ifcameraready
to the full version.
\else
to~\Cref{sec:ipeprelim}.
\fi 

Further, we augment the IPFE scheme with an additional algorithm $\PubKGen$ defined as follows. $\PubKGen(\mpk, \bfy \in \mcal{F}_{{\sf IP}, \ell})$ is a {\em deterministic} algorithm that takes in the master public key $\mpk$, and 
a vector $\bfy \in \mcal{F}_{{\sf IP}, \ell}$, and outputs a functional public key $\pk_\bfy$. 

\begin{remark}
We note that $\pk_\bfy$ does not enable decryption, so it does not change the correctness requirement. It also does not affect security of IPFE. To see this, note that $\PubKGen$ is deterministic. So, an adversary can always compute $\pk_\bfy$ on its own. Given that $\KGen$ is also deterministic, one way to think of $\pk_\bfy$ is as a commitment to $\sk_\bfy$. Typically, $\mpk$ also has this property w.r.t.\ $\msk$ and it is always implicit in the security definitions of IPFE. We formalize this compliance requirement for $\pk_\bfy$ and $\sk_\bfy$ below since FAS will use it. 
\end{remark}

\begin{definition}[$R_\ipfe$-Compliant IPFE]
\label{def:ipfe-compliant}
For a hard relation $R_\ipfe$, we say that an IPFE scheme is $R_\ipfe$ compliant if
for any $\secparam \in \N$,
for any $\pp \gets \ipe.\Gen(1^\secparam)$,
for any $(\mpk, \msk) \gets \ipe.\Setup(\pp, $ $1^\ell)$, 
for any $\bfy \in \mcal{F}_{{\sf IP}, \ell}$,
let $\pk_\bfy := \PubKGen(\mpk, \bfy)$, and 
$\sk_\bfy := \KGen(\msk, \bfy)$.
Then, it must be the case that $(\pk_\bfy, \sk_\bfy) \in R_\ipe$.
\end{definition}

Next, we describe an additional correctness property of IPFE that is tailored to make IPFE compatible with adaptor signatures (AS) when the two are used in tandem in our FAS construction. Looking ahead, we need this property because in our FAS construction, we will use an AS to sell functional secret keys. Recall that AS are defined w.r.t.\ two relations $R$ and $R'$. In this case, $R$ will be $R_\ipfe$ as defined in~\Cref{def:ipfe-compliant} and we  denote the extended relation $R'$ by $R'_\ipfe$. Then, the $\as.\Ext$ algorithm will extract a functional secret key $\sk'_\bfy$ as the witness for $\pk_\bfy$. While $\sk'_\bfy$ will be a witness of $R'_\ipfe$, it may not be a witness of the base relation $R_\ipfe$ since  $R_\ipfe \subseteq R'_\ipfe$, and we still want that $\sk'_\bfy$ should enable meaningful decryption. 
We formalize this robustness requirement below.

\begin{definition}[$R'_\ipfe$-Robust IPFE]
\label{def:ipfe-robust}
Let $R_\ipfe$ be the hard relation as defined in~\Cref{def:ipfe-compliant}. 
Let $R'_\ipfe$ such that $R_\ipfe \subseteq R'_\ipfe$ be an 
an extended relation of $R_\ipfe$. 
We say that an IPFE scheme is $R'_\ipfe$ robust if 
IPFE correctness holds even w.r.t.\ a functional secret key satisfying $R'_\ipfe$. More formally, 
for any $\secparam \in \N$,
let $\pp \gets \ipfe.\Gen(1^\secparam)$,
for any $\ell \in \N$, 
$\bfx \in \mcal{M}, \bfy \in \mcal{F}_{{\sf IP}, \ell}$, 
let $(\mpk, \msk) \leftarrow  \Setup(\pp, \ell)$, 
$\pk_\bfy := \PubKGen(\msk, \bfy)$,
$\ct \leftarrow \Enc(\mpk, \bfx)$.
For any $\sk'_\bfy$, if $(\pk_\bfy, \sk'_\bfy) \in R'_\ipfe$, then,  
$\Dec(\sk'_\bfy, \ct)$ outputs $f_\bfy(\bfx)$.
% \[
% \Pr\left[
% v = f_\bfy(\bfx): 
% \begin{array}{l}
% (\mpk, \msk) \leftarrow  \Setup(\pp, \ell),\\ 
% \pk_\bfy = \PubKGen(\msk, \bfy),\\ 
% \sk'_\bfy \ s.t.\ (\pk_\bfy, \sk'_\bfy) \in R'_\ipfe,\\
% \ct \leftarrow \Enc(\mpk, \bfx),\\ 
% v = \Dec(\sk'_\bfy, \ct)
% \end{array}
% \right] = 1.
% \]
\end{definition}

% \begin{remark}
% One can think of decryption correctness (\Cref{def:ipfe-correctness}) as being implictly defined with respect to $\sk_\bfy$ that is witness to $\pk_\bfy$ for the relation $R_\ipfe$. And one can think of the $R'_\ipfe$-robustness as decryption correctness with respect to $\sk'_\bfy$ that is witness to $\pk_\bfy$ for the relation $R'_\ipfe$. 
% % Note that here $R_\ipfe \subseteq R'_\ipfe$. 
% % Thus, if $(\pk_\bfy, \sk_\bfy) \in R_\ipfe$, then, $(\pk_\bfy, \sk_\bfy) \in R'_\ipfe$. But, $(\pk_\bfy, \sk'_\bfy) \in R'_\ipfe$ does not necessarily imply $(\pk_\bfy, \sk'_\bfy) \in R_\ipfe$. It is for this reason that we need IPFE special property 2 beyond just IPFE correctness.
% \end{remark}

% Lastly, we require a compatability property from our IPFE as follows. This will be useful for proving zero-knowledge witness privacy of our FAS scheme.

% \begin{definition}[$(\mcal{M},\mcal{F}_{{\sf IP}, \ell})$- Compatible IPFE]
% \label{def:ipfe-compatible}
% We say that an IPFE scheme for message space $\mcal{M}$ and function space $\mcal{F}_{{\sf IP}, \ell}$ is $(\mcal{M},\mcal{F}_{{\sf IP}, \ell})$-compatible if for any $\bfx \in \mcal{M}$ and any $\bfy \in \mcal{F}_{{\sf IP}, \ell}$, it is the case that $f_\bfy(\bfx) \in \mcal{F}_{{\sf IP}, 1}$.
% \end{definition}

\ignore{
	
	\nikhil{once the sim secure fas construction proof is successfully shown starting with ind secure ipfe and applying ind-to-sim compiler manually, delete the selective, sim-secure definition.}
	\begin{definition}[Selective, SIM-security]
	We say that the \ipe scheme satisfies selective, SIM-security, 
	iff for any non-uniform \ppt adversary \A, 
	there exists a stateful \ppt simulator $\Sim=(\Setup^*, \Enc^*, \KGen^*)$ and 
	there exists a negligible function $\negl$ 
	such that for all $\secparam \in \N, \ell \in \N$,
	\begin{align*}
	& |
	\Pr[\ipfeSimReal(1^\secparam, \ell) = 1] \\
	& \quad - \Pr[\ipfeSimIdeal(1^\secparam, \ell) = 1]
	| \leq \negl(\secparam),
	\end{align*}
	where $\ipfeSimReal(1^\secparam, \ell)$ and $\ipfeSimIdeal(1^\secparam, \ell)$ 
	are described in~\Cref{fig:ipfe-sel-sim-sec}. 
	\end{definition}

	\begin{figure*}[t]
	\centering
	\captionsetup{justification=centering}
	\begin{pchstack}[boxed, space=1em]
	\begin{pcvstack}
	\procedure[linenumbering, mode=text]{Experiment $\ipfeSimReal(1^\secparam, \ell)$}{
	$\pp \gets \Gen(1^\secparam)$
	\\ 
	$\bfx^* \gets \A(\pp)$
	\\ 
	$(\mpk, \msk) \gets \Setup(\pp, \ell)$
	\\ 
	$\ct^* \gets \Enc(\mpk, \bfx^*)$
	\\ 
	$b \gets \A^{\mcal{O}_\KGen(\cdot)}(\mpk, \ct^*)$ 
	\\ 
	\ret $b \in \{0,1\}$
	}
	\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_\KGen(\bfy)$}{
	\ret $\sk_\bfy = \KGen(\msk, \bfy)$
	}
	\end{pcvstack}
	\begin{pcvstack}
	\procedure[linenumbering, mode=text]{Experiment $\ipfeSimIdeal(1^\secparam, \ell)$}{
	$\pp \gets \Gen(1^\secparam)$
	\\ 
	$\bfx^* \gets \A(\pp)$
	\\ 
	$(\mpk^*, \msk^*) \gets \Setup^*(\pp, \ell)$
	\\ 
	$\ct^* \gets \Enc^*(\msk^*)$
	\\ 
	$b \gets \A^{\mcal{O}_\KGen^*(\cdot, \cdot)}(\mpk^*, \ct^*)$
	\\ 
	\ret $b \in \{0,1\}$
	}
	\procedure[linenumbering, mode=text]{Oracle $\mcal{O}_\KGen^*(\bfy, z)$}{
	\ret $\sk_\bfy \gets \KGen^*(\msk^*, \bfy, z)$
	}
	\end{pcvstack}

	\end{pchstack}
	\caption{Selective, SIM-security experiments of Inner Product Functional Encryption
	% \pnote{To be consistent with the literature, I would just call it WI and WH instead of WitInd and WitHid.}
	% \nikhil{done}
	}
	\label{fig:ipfe-sel-sim-sec}
	\end{figure*}
}



\ignore{
			\begin{mdframed}
			\textbf{Experiment} $\ipfeIND^b(1^\secparam)$:

			\begin{itemize}[leftmargin=5mm]
			\item {\bf Setup.}
			The challenger $\algC$ runs $\pp
			\leftarrow \Gen(1^\secparam)$, 
			and 
			gives $\pp$ to \algA.
			\algA submits its single encryption query $(\bfx_0,  \bfx_1)$ to the challenger \algC.
			The challenger computes $(\mpk, \msk) \leftarrow \Setup(\pp, n)$, $\ct \gets \Enc(\mpk, \bfx_b)$
			and 
			gives $\mpk, \ct$ to \algA.

			\item {\bf Query.}
			\algA makes the following types of queries to \algC: 
			\begin{itemize}[leftmargin=5mm,itemsep=1pt]
			\item $\KGen$ queries:
			the adversary \algA submits $\bfy$; 
			the challenger \algC computes $\sk_\bfy 
			\leftarrow \KGen(\msk, \bfy)$
			and returns to \algA the resulting $\sk_\bfy$.
			\end{itemize}
			\end{itemize}
			\end{mdframed}

			\begin{mdframed}
			\textbf{Experiment} ${\sf IPFE\text{-}Expt}^b(1^\secparam)$:

			\begin{itemize}[leftmargin=5mm]
			\item {\bf Setup.}
			The challenger $\algC$ runs $\pp
			\leftarrow \Gen(1^\secparam)$, and $(\mpk, \msk) \leftarrow \Setup(\pp, n)$, and 
			gives $\pp, \mpk$ to \algA.

			\item {\bf Query.}
			\algA makes the following types of queries to \algC: 
			\begin{itemize}[leftmargin=5mm,itemsep=1pt]
			\item $\KGen$ queries:
			the adversary \algA submits $\bfy$; 
			the challenger \algC computes $\sk_\bfy 
			\leftarrow \KGen(\msk, \bfy)$
			and returns to \algA the resulting $\sk_\bfy$.

			\item $\Enc$ queries:
			the adversary $\algA$ submits $(\bfx^{(0)},  \bfx^{(1)})$; 
			the challenger \algC computes $\ct \leftarrow \Enc(\mpk, \bfx^{(b)})$,
			and returns $\ct$ to \algA.
			\end{itemize}
			\end{itemize}
			\end{mdframed}



			\begin{definition}[Adaptive, IND-security of \ipe]
			We say that the \ipe scheme satisfies adaptive, IND-security, 
			iff for any non-uniform probabilistic polynomial-time (\ppt) admissible adversary, 
			its views in 
			${\sf IPFE\text{-}Expt}^0$
			and ${\sf IPFE\text{-}Expt}^1$
			are computationally indistinguishable.\pnote{better tos spell this out using the notion of a distinguisher}
			\label{defn:ipesec-ad}
			\end{definition}
			\nikhil{TODO: cite papers that construct this}
}




